Higher-Order Program Verification via HFL Model Checking

There are two kinds of higher-order extensions of model checking: HORS model checking and HFL model checking. Whilst the former has been applied to automated verification of higher-order functional programs, applications of the latter have not been well studied. In the present paper, we show that various verification problems for functional programs, including may/must-reachability, trace properties, and linear-time temporal properties (and their negations), can be naturally reduced to (extended) HFL model checking. The reductions yield a sound and complete logical characterization of those program properties. Compared with the previous approaches based on HORS model checking, our approach provides a more uniform, streamlined method for higher-order program verification.

==> appx-liveness-effective-selection-draft.tex <==
   \subsubsection{Overview of Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}}
  \wtnb{This subsection is a draft for Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete} and will be deleted in the final version.}

\begin{proof}[draft]
 Suppose that \(\TopEnv \pInter \prog \ESRel (\prog_0', \Pfun_0)\),
 \(\TopEnv \pInter \prog \eESRel (\prog_1', \Pfun_1)\),
 and \(\prog'_1 = (\progd, \mainfun)\).

 Proof proceeds in the following steps:
 \begin{align}
  &\InfTraces(\prog) \cap \Lang(\PWA) = \emptyset \\
  \Leftrightarrow&\InfTraces(\prog'_1) \cap \Lang(\PWA) = \emptyset \\
  \Leftrightarrow&
  \forall \seq{\ell} \in \InfTraces(\prog'_1). \forall \runseq \COL \text{run of \(\PWA\) over \(\seq{\ell}\).} \notag\\
  & \MAX\mathbf{Inf}(\Omega(\runseq)) \text{ is \emph{odd}}. \\
  \Leftrightarrow&
  \forall \RTyPath \COL \text{valid infinite choice sequence w.r.t }\prog'_1. \notag \\
  & \MAX\mathbf{Inf}(\Omega(\Run_{D,\PWA}(\RTyPath))) \text{ is \emph{odd}}. \\
  \Leftrightarrow &\forall \RTyPath \COL \text{valid infinite choice sequence w.r.t }
  \prog'_1. \notag \\
  & \text{If } \RTyPath \Vdash \mainfun \CallSeq_{\progd} g_1\,\seq{u}_1 \CallSeq_{\progd} g_2\,\seq{u}_2 \dots \text{, then }
  \MAX \mathbf{Inf}(\Omega_1(g_1) \Omega_1(g_2) \dots) \text{ is \emph{even}}. \\
  \Leftrightarrow& \models_\CSA (P'_1, \Pfun_1) \\
  \Leftrightarrow& \models_\CSA (P'_0, \Pfun_0)
 \end{align}

 Justifications for each step are the following:
\begin{itemize}
 \item \((1) \Leftrightarrow (2)\)
       By Lemma~\ref{lem:liveness:trace-coincidence},
       which follows from the simulation relation between \(\prog\) and \(\prog'\).
 \item \((2) \Leftrightarrow (3)\)
       By the definition.
 \item \((3) \Leftrightarrow (4)\) \\
       \((\Rightarrow)\) By the definition of \(\Run_{D, \PWA}(\RTyPath)\). \\
       \((\Leftarrow)\)
       I will prove the following lemma:
       \begin{lemma}
        Let \(D\) be a program and \(\PWA\) be a parity automaton.
        Suppose \(\seq{\ell} \in \InfTraces(\progd)\) and \(\runseq\) be a run of \(\PWA\) over \(\seq{\ell}\).
        There exists a choice sequence \(\RTyPath\) such that
        \(\EvSeq_{D, \PWA}(\RTyPath) = \seq{\ell}\) and
        \(\Run_{D, \PWA}(\RTyPath) = \runseq\).
       \end{lemma}
 \item \((4) \Leftrightarrow (5)\)
       This step follows from the following Corollary~\ref{cor:liveness:summarising-priority}.
       The next lemma is used to prove the corollary.
       \begin{lemma}
        Assume that \(\TopEnv\) is simple.
        Assume also:
        \begin{align*}
         \TopEnv \pInter D \qquad
         \ITE_0 \EnvRel \TopEnv \qquad
         \ITE_0 \pInter f\,\seq{s} : q \\
         (f\,\seq{s}; \RTyPath_0\RTyPath_1)  \mathrel{\stackrel{\seq{\ell}}{\red}\!\!{}_{\progd}^{N}} (g\,\seq{u}; \RTyPath_1) \qquad
         \RTyPath_0\RTyPath_1 \Vdash f\,\seq{s} \mathrel{\stackrel{\seq{\ell}}{\red}\!\!{}_{\progd}^{N}} g\,\seq{u} \qquad
         \RTyPath_0\RTyPath_1 \Vdash f\,\seq{s} \CallSeqN{N}_{D} g\,\seq{u}
        \end{align*}
        Then,
        \( \SUMMARY(\Run_{D, \PWA}(q, \seq{\ell}, \RTyPath_0)) + 1 = \Pfun_{\TopEnv}(g)\) holds.
       \end{lemma}
       \begin{corollary}\label{cor:liveness:summarising-priority}
        Assume \( \TopEnv \pInter (D, \mainfun) \) and \( \TopEnv \) is simple.
        Let \(\ell_1 \ell_2 \dots \in \InfTraces((D, \mainfun))\) and \(\runseq\) be
        an infinite run of \(\PWA\) over \(\ell_1 \ell_2 \dots\).
        Then there exists a choice sequence \(\RTyPath\) such that
        \begin{align*}
         \RTyPath \Vdash \mainfun \Pred{\ell_1}{D} \term_1 \Pred{\ell_2}{D} \term_2 \Pred{\ell_3}{D}\cdots \qquad
         \RTyPath \Vdash \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots
        \end{align*}
        and
        \( \MAX \mathbf{Inf}(\Omega(\Run_{D, \PWA}(\RTyPath))) + 1 = \MAX \mathbf{Inf}(\Omega_{\TopEnv}(g_1) \Omega_{\TopEnv}(g_2) \dots) \) hold.
       \end{corollary}
 \item \((5) \Leftrightarrow (6)\)
       By the definition of \(\models_\CSA\).
 \item \((6) \Leftrightarrow (7)\)
       Obvious, maybe. \wtnb{need to prove?}
\end{itemize}
\end{proof}

\wtnb{Below, I will prove the theorem in the way I described here.}

==> appx-liveness-effective-selection-old.tex <==
\subsection{Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}}
\wtnb{Deterministic automata version}
\subsubsection{Notations}
Given an intersection type \( \Itype = \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \) and a variable \( x \), we abbreviate the sequence \( x_{\Atype_1, m_1} x_{\Atype_2, m_2} \dots x_{\Atype_k, m_k} \) as \( \dup{x,\Itype} \).
For \( \Itype = \INT \), we write \( \dup{x,\Itype} \) for \( x_{\INT} \).

For an intersection type \( \Itype = \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \), we write \( \ZEnv{x : \Itype} \) for the intersection type environment \( \{ x : (\Atype_i, m_i, 0) \mid 1 \le i \le k \} \).
If \(\Itype = \Tint\), \(\ZEnv{x \COL \Itype}\) means \(\{x \COL \Tint\}\).
Similarly, for a top-level environment \( \TopEnv \), we write \( \TopEnvZ \) to mean \( \{ x : (\Atype, m, 0) \mid x : (\Atype, m) \in \TopEnv \} \).

Given an intersection type environment \( \ITE \), we write \( \ITE^{\Mark} \) for \( \{ x^{\Mark} : (\Atype, m, m') \mid x : (\Atype, m, m') \in \ITE \} \cup \{ x^{\Mark} : \INT \mid x : \INT \in \ITE \} \).
Similarly, for a top-level environment \( \TopEnv \), we write \( \TopEnv^{\Mark} \) for \( \{ x^{\Mark} : (\Atype, m) \mid x : (\Atype, m) \in \TopEnv \} \).

For an intersection type environment \( \ITE \) and a top-level environment \( \TopEnv \), we write \(\ITE \EnvRel \TopEnv\) if
\(f \COL (\Atype, m) \in \TopEnv\) for each \((f \COL (\Atype, m, m')) \in \ITE\).
%%it satisfies the following conditions: if \((f \COL (\Atype, m, m')) \in \ITE\), then \(f \COL (\Atype, m) \in \TopEnv\).


\subsubsection{Basic properties of the type system and transformation}

\begin{lemma}[Weakening]
 \label{appx:es:lem:weakening}
 If \(\ITE \pInter \term \COL \Atype \ESRel \term'\) and \(\ITE \subseteq \ITE'\),
 then \(\ITE' \pInter \term \COL \Atype \ESRel \term'\).
\end{lemma}
\begin{proof}
  Straightforward induction on structure of the derivations.
  We discuss only one case below.
  \begin{itemize}
  \item Case for \rn{IT-Event}:
    Then
    \begin{align*}
      \Atype = q \qquad
      \term = \evexp{\lab}{\termalt} \qquad
      \term' = \evexp{\lab}{\termalt'} \qquad
      \ITE \RaiseP \Omega(\delta(q, \lab)) \pInter \termalt \COL \Atype \ESRel \termalt'.
    \end{align*}
    Since \(\ITE \subseteq \ITE'\), we have \(\ITE \RaiseP \Omega(\delta(q, \lab)) \subseteq \ITE' \RaiseP \Omega(\delta(q, \lab))\).
    By the induction hypothesis,
    \[
    \ITE' \RaiseP \Omega(\delta(q, \lab)) \pInter \termalt \COL \Atype \ESRel \termalt'.
    \]
    By using \rn{IT-Event}, we obtain
    \(\ITE' \pInter \term \COL \Atype \ESRel \term'\).
  \end{itemize}
\end{proof}


\begin{lemma}[Substitution (Integer)]
 \label{appx:es:lem:subst:integer}
 Assume \(\ITE, x \COL \Tint \pInter \term \COL \Atype \ESRel \term'\) and
 \(\ITE \pInter u \COL \Tint \ESRel u'\).
 Then, \(\ITE \pInter [u/x] \term \COL \Atype \ESRel [u'/\xint]\term'\) holds.
\end{lemma}
\begin{proof}
 By straightforward induction.
\end{proof}



\begin{lemma}[Substitution (Intersection Type)]
 \label{appx:es:lem:subst:inter}
 Assume:
 \begin{align*}
  \Itype = \bigwedge_{1 \le i \le l} (\Atype_i, m_i) \qquad
  &x \notin dom(\ITE) \\
  ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' \pInter \term \COL \Atype \ESRel \term' \qquad
  &\forall i \in \{1,\dots,l\}.\ \ITE \RaiseP m_i \pInter u \COL \Atype_i \ESRel u'_i.
 \end{align*}
 Then,
 \[
 (\ITE \RaiseP n) \cup \ITE' \pInter [u/x] \term \COL \Atype \ESRel [\seq{u}'/\dup{x,\Itype}]t'.
 \]
 % Then, \(\ITE \RaiseP n \pInter [u/x] \term \COL \Atype \ESRel [u'_1/x_{\Atype_1, m_1}]\dots[u'_l/x_{\Atype_l, m_l}] t'\) holds.
\end{lemma}
\begin{proof}
 The proof proceeds by induction on the derivation of
 \((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \pInter \term \COL \Atype \ESRel \term'\),
 with case analysis on the last rule used.

 \begin{itemize}
  \item Case for \rn{IT-Var}:
        The case where \(\term \neq x\) is trivial.
        Assume that \(\term = x\).
        Then there exists \(k \in \{1, \dots, l\}\) such that \( \theta = \theta_k \), \( t' = x_{\theta_k,m_k} \) and \( n = m_k \).
        %% \begin{align*}
        %%   (\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n &\pInter x \COL \Atype_k \ESRel x_{\Atype_k, m_k} \\
        %%  n &= m_k \tag{Since \(x \COL (\Atype_k, m_k, m_k) \in (\ITE \cup \ZEnv{x \COL \Itype})\RaiseP n\)}
        %% \end{align*}
        By the assumption, we have \(\ITE \RaiseP m_k \pInter u \COL \Atype_k \ESRel u'_k\).
        Since \([u/x]x = u\) and \([\seq{u'}/\dup{x,\Itype}]x_{\Atype_k, m_k} = u'_k\), we have
        \begin{align*}
         \ITE \RaiseP m_k &\pInter [u/x]x \COL \Atype_k \ESRel [\seq{u'}/\dup{x,\Itype}] x_{\Atype_k, m_k}.
        \end{align*}
        By Lemma~\ref{appx:es:lem:subst:inter}, we have
        \begin{align*}
         (\ITE \RaiseP m_k) \cup \ITE' &\pInter [u/x]x \COL \Atype_k \ESRel [\seq{u'}/\dup{x,\Itype}] x_{\Atype_k, m_k}.
        \end{align*}
        as required.
  \item Case for \rn{IT-Event}:
        Then \(\term = \evexp{\lab}{\term_1}\) and we have
        \begin{align*}
         \term'=\evexp{\lab}{\term'_1} \qquad
         \Atype = q \\
         (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) &\pInter \term_1 \COL \delta(q, \lab) \ESRel \term'_1.
        \end{align*}
        Since
        \begin{align*}
          & (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) \\
          & = ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \RaiseP \Omega(\delta(q,\lab))) \cup (\ITE' \RaiseP \Omega(\delta(q, \lab))),
        \end{align*}
        one can apply the induction hypothesis, obtaining
        \begin{align*}
         ((\ITE  \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) &\pInter [u/x] \term_1 \COL \delta(q, \lab) \ESRel  [\seq{u'}/\dup{x,\Itype}] \term'_1.
        \end{align*}
        By using \rn{IT-Event}, we have the following as required:
        \begin{align*}
         \ITE \RaiseP n &\pInter [u/x] (\evexp{\lab}{\term_1}) \COL q \ESRel  [\seq{u'}/\dup{x,\Itype}] (\evexp{\lab}{\term'_1}).
        \end{align*}
  \item Case for \rn{IT-App}:
        Then \(\term=\term_1\;\term_2\) and we have
        \begin{align*}
         \term'=\term'_1\;\term'_{2,1}\dots \term'_{2,k} \qquad
         ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' &\pInter \term_1 \COL \bigwedge_{1 \le j \le k}(\Atype'_{j}, m'_{j}) \to \Atype
         \ESRel \term'_1 \\
         \forall j \in \{1,\dots,k\}. (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP m'_{j} &\pInter \term_2 \COL \Atype'_{j} \ESRel \term'_{2,j}.
        \end{align*}
        By the induction hypothesis, we have
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' \pInter [u/x]\term_1 \COL \bigwedge_{1 \le j \le k}(\Atype'_{j}, m'_{j}) \to \Atype
         \ESRel [\seq{u'}/\dup{x,\Itype}]\term'_1 \\
         \forall j \in \{1,\dots,k\}. ((\ITE \RaiseP n) \cup \ITE') \RaiseP m'_{j} \pInter [u/x]\term_2 \COL \Atype'_{j} \ESRel [\seq{u'}/\dup{x,\Itype}] \term'_{2,j}.
        \end{align*}
        By using \rn{IT-App}, we obtain:
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' &\pInter [u/x](\term_1\;\term_2) \COL \Atype
         \ESRel [\seq{u'}/\dup{x,\Itype}](\term'_1\;\term'_{2,1}\dots\term'_{2,k})
        \end{align*}
        as required.
  \item Case for \rn{IT-Abs}:
        Then \(\term=\lambda y.\termalt\) and we have
        \begin{align*}
         \Atype = \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j) \to \Atype'_0 \qquad
         &\term'=\lambda y_{\Atype'_1,m'_1}\dots y_{\Atype'_k,m'_k}. s' \\
         y \not\in dom((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \qquad
         &((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)} \pInter \termalt \COL \Atype'_0
         \ESRel \termalt'
        \end{align*}
        %% Since
        %% \[
        %% ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n, \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)}) \RaiseP 0 = (\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)},
        %% \]
        By the induction hypothesis, we have
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)} &\pInter [u/x]\termalt \COL \Atype'_0
         \ESRel [\seq{u'}/\dup{x,\Itype}] \termalt'.
        \end{align*}
        By using \rn{IT-Abs}, we obtain:
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE'
         &\pInter [u/x]\lambda y.\termalt \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j) \to \Atype'_0
         \ESRel [\seq{u'}/\dup{x,\Itype}]
         \lambda y_{\Atype'_1,m'_1}\dots y_{\Atype'_k,m'_k}. \termalt'
        \end{align*}
        as required.
 \end{itemize}
\end{proof}




\subsubsection{Translation preserves traces}
The next lemma shows that the reduction of the original program can be simulated by the result of translation.
(It also proves an additional result on types, which shall be used.)
\begin{lemma}
  \label{appx:es:lem:sim1}
  Assume
  \begin{itemize}
  \item \( \TopEnv \pInter D \ESRel D' \),
  \item \( \ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt \),
  \item \( \ITE \EnvRel \TopEnv \) and  \( \ITE' \EnvRel \TopEnv^\Mark \), and
  \item \(\RTyPath \Vdash \term \Pred{\ell}{D^\Mark} \term' \).
  \end{itemize}
  Then there exists \(\termalt'\) such that
  \[
  \RTyPath \Vdash \termalt \Pred{\ell}{D'^\Mark} \termalt'
  \]
  and
  \[
  \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) \pInter \term' \COL \delta(q,\ell) \ESRel \termalt'.
  \]
\end{lemma}
\begin{proof}
 The proof proceeds by case analysis on the shape of \(\term\).
 \begin{itemize}
  \item Case \(\term = \evexp{\lab}{\term_1}\):
        By definition, we have \(\term' = \term_1\) and \(\ell = \lab\).
        Since the last rule used to derive \( \ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt \) is \rn{IT-Event}, we have:
        \begin{align*}
         (\ITE \cup \ITE') \RaiseP \Omega(\delta(q, a)) \pInter \term_1 \COL \delta(q,\lab) \ESRel \termalt_1 \qquad
         \termalt = \evexp{\lab}{\termalt_1}
        \end{align*}
        By the definition of \(\SUMMARY\), \(\SUMMARY(q, \lab) = \Omega(\delta(q, \lab))\).
        In addition, \(\evexp{\lab}{\termalt_1} \Pred{\lab}{D'^\Mark} \termalt_1\) holds.
        Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \[
        \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \lab)) \pInter \term_1 \COL \delta(q, \lab) \ESRel \termalt_1.
        \]
        Hence, the required result holds for \(\termalt' = \termalt_1\).
  \item Case \(\term = \term_1 \nondet \term_2\):
        Suppose \(\RTyPath\) is of the form \(\PLeft\RTyPath'\); the case that \( \RTyPath = \PRight\RTyPath' \) can be proved similarly.
        By definition, \(\ell = \epsilon\) and \(\term' = \term_1\).
        Since the last rule used to derive \( \ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt \) is \rn{IT-NonDet}, we have:
        \begin{align*}
         \termalt = \termalt_{1} \nondet \termalt_{2} \qquad
         (\ITE \cup \ITE') \pInter \term_{1} \COL q \ESRel \termalt_{1} \qquad
         (\ITE \cup \ITE') \pInter \term_{2} \COL q \ESRel \termalt_{2}
        \end{align*}
        We have \(\SUMMARY(q, \ell) = 0\).
        Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \begin{align*}
         \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) &\pInter \term_1 \COL q
         \ESRel \termalt_1.
        \end{align*}
        In addition, \(\RTyPath \Vdash \termalt \Pred{\epsilon}{D'^\Mark} \termalt_1\).
         Hence, the required result holds for \(\termalt' = \termalt_1\).
        %% Similarly, in the case where \(\RTyPath = \PRight\RTyPath'\), we obtain \(\termalt' = \termalt_2\).
  \item Case \(\term = \ifexp{p(\term_{1}, \dots, \term_{n})}{\term_{n+1}}{\term_{n+2}}\):
        Suppose \((\sem{\term_{1}}, \dots, \sem{\term_{n}}) \in \sem{p}\).
        In this case, we have \(\ell = \epsilon\), \(\term' = \term_{n+1}\).
        Since the last rule used to derive \( \ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt \) is \rn{IT-IF}, we have:
        \begin{align*}
         \termalt &= \ifexp{p(\termalt_{1}, \dots, \termalt_{n})}{\termalt_{n+1}}{\termalt_{n+2}} \qquad
         \forall i \in \{1,\dots, n\}.
         \ITE \cup \ITE' \pInter \term_{i} \COL \Tint \ESRel \termalt_{i} \\
         \ITE \cup \ITE' &\pInter \term_{n+1} \COL q \ESRel \termalt_{n+1} \qquad
         \ITE \cup \ITE' \pInter \term_{n+2} \COL q \ESRel \termalt_{n+2}
        \end{align*}
        By the well-typedness of the program,
        for every \(i \in \{1,\dots,n\}\), \(\term_{i}\) consists of only integers and integer operations.
        Thus, we have \(\sem{\term_i} = \sem{\termalt_i}\) for each \(i \in \{1,\dots,n\}\) and
        \(\termalt \Pred{\epsilon}{D'^\Mark} \termalt_{n+1}\).

        In addition, we have \(\SUMMARY(q, \ell) = 0\).
        Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \begin{align*}
         \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) &\pInter \term' \COL q
         \ESRel \termalt_{n+1}.
        \end{align*}
        Hence, the required result holds for \(\termalt' = \termalt_{n+1}\).

        The case where
        \((\sem{\term_{1}}, \dots, \sem{\term_{n}}) \notin \sem{p}\) is similar.
%%        we obtain \(\termalt' = \termalt_{n+2}\) in similar way.
  \item Case \(\term = f\;\term_1\dots \term_n\):
        Suppose \(D^\Mark(f) = \lambda x_1\dots x_n. \term_0\).
        In this case, \(\term' = [\term_1/x_1]\dots[\term_n/x_n]\term_0\) and \(\ell = \epsilon\).

        Then we have
        \begin{align}
         \ITE \cup \ITE' &\pInter f \COL \Atype \ESRel f_{\Atype, m} \nonumber\\
         \Atype = \Itype_1 \to \dots \Itype_n \to q \qquad
         I &\subseteq \{1, \dots, n\} \qquad
         \bar{I} = \{1,\dots,n\}\setminus I \nonumber\\
         \forall i \in I. \Itype_i = \bigwedge_{1 \le j \le \ell_i} (\Atype'_{i,j}, m'_{i,j}) \qquad
         &\forall i \in \bar{I}. \Itype_i = \Tint \nonumber\\
         \forall i \in I. \forall j \in \{1, \dots, \ell_i\}.
         (\ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j}
         \ESRel \termalt_{i, j}
         \label{appx:es:lem:sim1:1} \\
         \forall i \in \bar{I}.
         \ITE \cup \ITE' &\pInter \term_{i} \COL \Tint
         \ESRel \termalt_{i, 1}
         \label{appx:es:lem:sim1:2} \\
         \forall i \in \{1,\dots,n\}. \seq{\termalt_{i}} &=
         \begin{cases}
          \termalt_{i,1} \dots \termalt_{i,\ell_i} & (i \in I) \\
          \termalt_{i,1} & (\text{otherwise})
         \end{cases} \nonumber\\
         \termalt &= f_{\Atype, m}\;\seq{\termalt_{1}}\dots\seq{\termalt_{n}} \nonumber
        \end{align}

        Since \(\TopEnv \pInter D\),
        we have
        \begin{align}
         \TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
         &\pInter \term_0 \COL q
         \ESRel \termalt_0
         \label{appx:es:lem:sim1:4}
        \end{align}


        By using Lemma~\ref{appx:es:lem:weakening} with
        \eqref{appx:es:lem:sim1:1}, \eqref{appx:es:lem:sim1:2} and \eqref{appx:es:lem:sim1:4},
        we have
        \begin{align}
         (\TopEnvZ \cup \ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j} \ESRel s_{i,j} \label{appx:es:lem:sim1:5} \\
         \forall i \in \bar{I}.
         (\TopEnvZ \cup \ITE \cup \ITE') &\pInter \term_{i} \COL \Tint \label{appx:es:lem:sim1:6} \ESRel s_{i,1} \\
         \TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
         &\pInter \term_0 \COL q
         \ESRel \termalt_0
         \label{appx:es:lem:sim1:7}
        \end{align}

        Since
        \[
        (\TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}) \RaiseP 0 =
        \TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n},
        \]
        by using Lemma~\ref{appx:es:lem:subst:inter} and Lemma~\ref{appx:es:lem:subst:integer} repeatedly
        with \eqref{appx:es:lem:sim1:5}, \eqref{appx:es:lem:sim1:6} and \eqref{appx:es:lem:sim1:7},
        we have
        \begin{align*}
         \TopEnvZ \cup \ITE \cup \ITE' &\pInter [\term_{1}/x_1] \dots [\term_{n}/x_n] \term_0 \COL q
         \ESRel [\seq{\termalt_1}/\dup{x_1, \Itype_1}]\dots [\seq{\termalt_n}/\dup{x_n, \Itype_n}] \termalt_0.
        \end{align*}
        In addition, \(\SUMMARY(q, \ell) = 0\) and \(\termalt \Pred{\epsilon}{D'^\Mark} [\seq{\termalt_1}/\dup{x_1, \Itype_1}]\dots [\seq{\termalt_n}/\dup{x_n, \Itype_n}] \termalt_0\).
        Thus, the required result holds for \(\termalt' = [\seq{\termalt_1}/\dup{x_1, \Itype_1}]\dots [\seq{\termalt_n}/\dup{x_n, \Itype_n}] \termalt_0\).
 \end{itemize}
\end{proof}

The next lemma shows the simulation in the other direction.
\begin{lemma}
 \label{appx:es:lem:sim2}
 Assume
 \begin{align*}
  \TopEnv \pInter D \ESRel D' \qquad
  \ITE \EnvRel \TopEnv \qquad
  \ITE' \EnvRel \TopEnv^\Mark \qquad
  \ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt \qquad
  \RTyPath \Vdash \termalt \Pred{\ell}{D'^\Mark} \termalt'.
 \end{align*}
 Then, there exists \(\term'\) such that
 \begin{align*}
  \RTyPath \Vdash \term \Pred{\ell}{D^\Mark} \term' \qquad
  \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) \pInter \term' \COL \delta(q,\ell) \ESRel \termalt'
 \end{align*}
\end{lemma}
\begin{proof}
  The proof proceeds by case analysis on the shape of \(\termalt\).
  By the assumption
  \(\RTyPath \Vdash \termalt \Pred{\ell}{D'^\Mark} \termalt'\), it suffices to consider
  only the cases where the shape of \(\termalt\) mathces the lefthand side of a transition rule.,
 \begin{itemize}
  \item Case \(\termalt = \evexp{\lab}{\termalt_1}\):
        By the shape of \(\termalt\),
        the last rule used on the derivation of \(\ITE \cup \ITE' \pInter \term \COL q \ESRel \termalt\) is
        either \rn{IT-Event} or \rn{IT-App}.
        By induction on the derivation, one can prove that \( \term = (\evexp{\lab}{\term_0})\,\term_1\,\dots\,\term_k \) for some \( k \).
        By the simple-type system, one cannot apply \( \evexp{\lab}{\term_0} \) to a term; hence \( k = 0 \) and the last rule used on the derivation is \rm{IT-Event}.
        %% Even if the last rule is \rn{IT-App}, \rn{IT-Event} must be used before finite steps.
        %% However, \rn{IT-Event} can not be used for a term with a function type.
        %% Thus, the last rule used on the derivation is \rn{IT-Event}.

        %By rule \rn{IT-Event}, we have:
        Then we have
        \begin{align*}
         (\ITE \cup \ITE') \RaiseP \Omega(\delta(q, a)) \pInter \term_1 \COL \delta(q,\lab) \ESRel \termalt_1 \qquad
         \term = \evexp{\lab}{\term_1}
        \end{align*}
        By the transition semantics, \(\termalt' = \termalt_1\) and \(\ell = \lab\).
        Since \(\SUMMARY(q, \lab) = \Omega(\delta(q, \lab))\),
        by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \[
        \TopEnvZ \cup (\ITE \cup \ITE') \RaiseP \SUMMARY(q, \lab) \pInter \term_1 \COL \delta(q, \lab) \ESRel \termalt_1.
        \]
        In addition, \(\evexp{\lab}{\term_1} \Pred{\lab}{D^\Mark} \term_1\) holds.
        Hence, the required result holds for \(\term' = \term_1\).
  \item Case \(\termalt = \termalt_1 \nondet \termalt_2\):
        As with the previous case,
        the last rule used on the derivation is \rn{IT-NonDet}.
        %
        %By rule \rn{IT-NonDet}, we have:
        Then we have
        \begin{align*}
         (\ITE \cup \ITE') \pInter \term_{1} \COL q \ESRel \termalt_{1} \qquad
         (\ITE \cup \ITE') \pInter \term_{2} \COL q \ESRel \termalt_{2} \qquad
         \term = \term_{1} \nondet \term_{2}
        \end{align*}
        Suppose \(\RTyPath\) is of the form \(\PLeft\RTyPath'\).
        By the transition semantics, \(\ell = \epsilon\) and
        \(\termalt' = \termalt_1\).
        We have \(\SUMMARY(q, \ell) = 0\).
        Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \begin{align*}
         \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) &\pInter \term_1 \COL q
         \ESRel \termalt_1.
        \end{align*}
        In addition, \(\PLeft\RTyPath' \Vdash \term \Pred{\epsilon}{D^\Mark} \term_i\).
        Hence, the required result holds for \(\term' = \term_1\).
        Similarly, in the case where \(\RTyPath = \PRight\RTyPath'\),
        we obtain \(\term' = \term_2\).
  \item Case \(\termalt = \ifexp{p(\termalt_{1}, \dots, \termalt_{n})}{\termalt_{n+1}}{\termalt_{n+2}}\):
        As with the previous cases,
        the last rule used on the derivation is \rn{IT-If}.
        %
        %By rule \rn{IT-IF}, we have:
        Hence we have
        \begin{align*}
      &   \term = \ifexp{p(\term_{1}, \dots, \term_{n})}{\term_{n+1}}{\term_{n+2}} \qquad
         \forall i \in \{1,\dots, n\}.
         \ITE \cup \ITE' \pInter \term_{i} \COL \Tint \ESRel \termalt_{i} \\&
         \ITE \cup \ITE' \pInter \term_{n+1} \COL q \ESRel \termalt_{n+1} \qquad
         \ITE \cup \ITE' \pInter \term_{n+2} \COL q \ESRel \termalt_{n+2}
        \end{align*}
        Suppose \((\sem{\termalt_{1}}, \dots, \sem{\termalt_{n}}) \in \sem{p}\).
        In this case, we have \(\ell = \epsilon\) and \(\termalt' = \termalt_{n+1}\).
        By the well-typedness of the program,
        for every \(i \in \{1,\dots,n\}\), \(\term_{i}\) consists of only integers and integer operations.
        Thus, we have \(\sem{\term_i} = \sem{\termalt_i}\) for each \(i \in \{1,\dots,n\}\) and
        \(\term \Pred{\epsilon}{D^\Mark} \term_{n+1}\).

        In addition, we have \(\SUMMARY(q, \ell) = 0\).
        Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        \begin{align*}
         \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(q, \ell)) &\pInter \term' \COL q
         \ESRel \termalt_{n+1}.
        \end{align*}
        Hence, the required result holds for \(\term' = \term_{n+1}\).

        In the case where
        \((\sem{\termalt_{1}}, \dots, \sem{\termalt_{n}}) \notin \sem{p}\),
        we obtain \(\term' = \term_{n+2}\) in a similar way.
  \item Case \(\termalt = g\;\termalt_1\dots \termalt_n\) with \(g\in\dom(D')\):
        \newcommand\bdy{\mathit{body}}
        By the shape of \(\termalt\),
        the last rule used on the derivation is \rn{IT-App} or \rn{IT-AppInt}.

%%        Since \(\termalt\) has a reduction,
%%        \(\termalt_0 \in dom(D')\) holds.
        By induction on the derivation,
        we have \(\term = f \term_1 \dots \term_k\) for some \(k\).

        Then, we have
        \begin{align}
         g = f_{\Atype, m} \qquad
         \ITE \cup \ITE' \pInter f \COL \Atype \ESRel f_{\Atype, m} \nonumber\\
         D(f) = \lambda x_1\dots x_k. \term_\bdy \qquad
         D'(f_{\Atype, m}) = \lambda y_1\dots y_n. \termalt_\bdy \nonumber\\
         \TopEnvZ \pInter \lambda x_1\dots x_k. \term_\bdy \COL \Atype
         \ESRel
         \lambda y_1\dots y_n. \termalt_\bdy. \label{appx:es:lem:sim2:app:0}
        \end{align}

        %By \rn{IT-App} and \rn{IT-AppInt},
        Furthermore, we have
        \begin{align}
         \Atype = \Itype_1 \to \dots \Itype_{k} \to q \qquad
         I &\subseteq \{1, \dots, k\} \qquad
         \bar{I} = \{1,\dots,k\}\setminus I \nonumber\\
         \forall i \in I. \Itype_i = \bigwedge_{1 \le j \le \ell_i} (\Atype'_{i,j}, m'_{i,j}) \qquad
         &\forall i \in \bar{I}. \Itype_i = \Tint \nonumber\\
         \forall i \in I. \forall j \in \{1, \dots, \ell_i\}.
         (\ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j}
         \ESRel u_{i, j}
         \label{appx:es:lem:sim2:1} \\
         \forall i \in \bar{I}.
         \ITE \cup \ITE' &\pInter \term_{i} \COL \Tint
         \ESRel u_{i, 1}
         \label{appx:es:lem:sim2:2} \\
         \forall i \in \{1,\dots,k\}. \seq{u_{i}} &=
         \begin{cases}
          u_{i,1} \dots u_{i,\ell_i} & (i \in I) \\
          u_{i,1} & (\text{otherwise})
         \end{cases} \nonumber\\
         \seq{u_1} \dots \seq{u_k} &= \termalt_1 \dots \termalt_n \nonumber\\
         \dup{x_1,\Itype_1} \dots \dup{x_k,\Itype_k} &= y_1\dots y_n\nonumber\\
        \end{align}

        Thus, \(\termalt' =  [\seq{u_1}/\dup{x_1, \Itype_1}]\dots [\seq{u_k}/\dup{x_k, \Itype_k}] \termalt_\bdy\) and \(\ell = \epsilon\).

        %By \eqref{appx:es:lem:sim2:app:0}, \rn{IT-Abs} and \rn{IT-AbsInt},
        By \eqref{appx:es:lem:sim2:app:0},
        we have
        \begin{align}
         \TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}
         &\pInter \term_{\bdy} \COL q
         \ESRel \termalt_{\bdy}
         \label{appx:es:lem:sim2:4}
        \end{align}

        By using Lemma~\ref{appx:es:lem:weakening} with
        \eqref{appx:es:lem:sim2:1}, \eqref{appx:es:lem:sim2:2} and \eqref{appx:es:lem:sim2:4},
        we have
        \begin{align}
         (\TopEnvZ \cup \ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j} \ESRel u_{i,j} \label{appx:es:lem:sim2:5} \\
         \forall i \in \bar{I}.
         (\TopEnvZ \cup \ITE \cup \ITE') &\pInter \term_{i} \COL \Tint \label{appx:es:lem:sim2:6} \ESRel u_{i,1} \\
         \TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k} &\pInter \term_{\bdy} \COL q
         \ESRel \termalt_{\bdy}
         \label{appx:es:lem:sim2:7}
        \end{align}

        %Since
        %\[
        %(\TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}) \RaiseP 0 =
        %\TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}
        %\]
        By using Lemma~\ref{appx:es:lem:subst:inter} and Lemma~\ref{appx:es:lem:subst:integer} repeatedly
        with \eqref{appx:es:lem:sim2:5}, \eqref{appx:es:lem:sim2:6} and \eqref{appx:es:lem:sim2:7},
        we have
        \begin{align*}
         \TopEnvZ \cup \ITE \cup \ITE' &\pInter [\term_{1}/x_1] \dots [\term_{k}/x_k] \term_\bdy \COL q
         \ESRel [\seq{u_1}/\dup{x_1, \Itype_1}]\dots [\seq{u_k}/\dup{x_k, \Itype_k}] \termalt_{\bdy}.
        \end{align*}
        In addition, \(\SUMMARY(q, \ell) = 0\) and \(\term \Pred{\epsilon}{D} [\term_1/x_1]\dots [\term_k/x_k] \term_{\bdy}\).
        Thus, the required result holds for \(\term' = [\term_1/x_1]\dots [\term_k/x_k] \term_{\bdy}\).
 \end{itemize}
\end{proof}

\begin{lemma}\label{lem:liveness:trace-coincidence}
  If \( \TopEnv \pInter P \Rightarrow (P', \Pfun) \), then \( \InfTraces(P) = \InfTraces(P') \).
\end{lemma}
\begin{proof}
%%  \tk{to do}\wtnb{I tried to fill out the proof}\nk{I am afraid the following is sufficient.}
  This follows immediately from
  Lemmas~\ref{appx:es:lem:sim1} and \ref{appx:es:lem:sim2}.
%% Let \(P = (D, \term_0)\) and \(P' = (D', \termalt_0)\).
%%
%% (\(\InfTraces(P) \subseteq \InfTraces(P')\))
%% Let \(\ell_0 \ell_1 \dots \in \InfTraces(P)\).
%% For every \(i \in \omega\), we have \(\RTyPath_i \Vdash \term_i \Pred{\ell_i}{D} \term_{i+1}\) and
%% \(\RTyPath_i\) is \(\PLeft\RTyPath_{i+1}\), \(\PRight\RTyPath_{i+1}\) or \(\RTyPath_{i+1}\).
%% By Lemma~\ref{appx:es:lem:sim1}, for every \(i \in \omega\),
%% we have
%% \(\RTyPath_i \Vdash \termalt_i \Pred{\ell_i}{D'} \termalt_{i+1}\) and
%% \(\ITE_i \pInter \term_i \COL q_i \ESRel \termalt_i\) for some \(\ITE_i\) and \(q_i\).
%% Hence, \(\ell_0 \ell_1 \dots \in \InfTraces(P').\)
%%
%% (\(\InfTraces(P') \subseteq \InfTraces(P)\))
%% Similarly, by using Lemma~\ref{appx:es:lem:sim2},
%% we can prove this side.
\end{proof}


\subsubsection{Analysis of the result of the translation}
\label{sec:appx:liveness:analysis-of-result}
By the translation, an intersection type \( \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \) is transformed into the product type \( \prod_{1 \le i \le k} (\Atype_i, m_i) \).
Formally the translation on types is defined by:
\begin{align*}
  \EffTypeTrans{q} &:= q \\
  \EffTypeTrans{(\INT \to \Atype)} &:= \INT \to (\EffTypeTrans{\Atype}) \\
  \EffTypeTrans{\left(\bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype_0\right)} &:= (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to \EffTypeTrans{\Atype_0}.
\end{align*}
For an intersection type environment \(\ITE\), we define \( \EffTypeTrans{\ITE} := \{ x_{\Atype,m} : (\Atype,m, m') \mid x : (\Atype,m, m') \in \ITE \} \).
Similarly, for a top-level type environment \( \TopEnv \), we define \( \EffTypeTrans{\TopEnv} := \{ x_{\Atype,m} : (\Atype,m) \mid x : (\Atype,m) \in \TopEnv \} \).

We say that a top-level environment \( \TopEnv \) is \emph{simple} if, for every \( x \), there exists at most one binding \( x : (\Atype, m) \in \TopEnv \).
Given a simple top-level environment \( \TopEnv \), if \( x : (\Atype, m) \in \TopEnv \), then we write \( \Pfun_{\TopEnv}(x) = m \).
Since \( \TopEnv \) is simple, \( \Pfun_{\TopEnv} \) is a partial mapping.

\changed{Below, we write
\(\ITE \pInter \term \COL \Atype \) if
\(\ITE \pInter \term \COL \Atype \ESRel \termalt\) for some \(\termalt\).}
\nk{Has this been mentioned elsewhere?}

\begin{lemma}\label{lem:appx:liveness:translation-typable:pre}
 If \(\ITE \pInter \term \COL \Atype \ESRel \termalt\),
 then \(\EffTypeTrans{\ITE} \pInter \termalt \COL \EffTypeTrans{\Atype}\).
\end{lemma}
\begin{proof}
 The proof proceeds by induction on the derivation of \(\ITE \pInter \term \COL \Atype \ESRel \termalt\),
 with case analysis on the last rule used.
 We prove only interesting cases.
 \begin{itemize}
  \item Case for \rn{IT-App}:
    %%        Let \(\term = \term_1 \term_2\).
    By \rn{IT-App}, we have:
        \begin{align*}
          &   \term=\term_1\term_2 \qquad
                   \termalt = \term'_1 \term'_{2,1} \dots \term'_{2,k}\\
      &   \ITE \pInter \term_1 \COL \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype \ESRel \term'_1 \qquad
         \forall i \in \{1,\dots, k\}.\;\ITE \RaiseP m_i \pInter \term_2 \COL \Atype_i \ESRel \term'_{2,i} \qquad
        \end{align*}
        By the induction hypothesis, we have
        \begin{align*}
         \EffTypeTrans{\ITE} \pInter \term'_1 \COL (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to (\EffTypeTrans{\Atype}) \qquad
         \forall i \in \{1,\dots, k\}.\;\EffTypeTrans{(\ITE \RaiseP m_i)} &\pInter \term'_{2,i} \COL \EffTypeTrans{\Atype_i}.
        \end{align*}
        Since
        \(\EffTypeTrans{(\ITE \RaiseP m_i)} = (\EffTypeTrans{\ITE}) \RaiseP m_i\),
        by using \rn{IT-App} \(k\) times,
        we obtain \(\EffTypeTrans{\ITE} \pInter \term'_1 \term'_{2,1}\dots \term'_{2,k} \COL \EffTypeTrans{\Atype}\) as required.
  \item Case for \rn{IT-Abs}:
        By \rn{IT-Abs}, we have:
        \begin{align*}
      &  \term = \lambda x. \term' \qquad \termalt = \lambda x_{\Atype_1,m_1}\dots x_{\Atype_k,m_k}.\;\termalt'\qquad
        \Atype = \bigwedge_{1 \le i \le k} (\Atype_i,m_i)\to \Atype'\\
       &  \ITE, x \COL (\Atype_1, m_1, 0), \dots, x \COL (\Atype_k, m_k, 0)
         \pInter \term' \COL \Atype' \ESRel \termalt' \qquad
         x \notin dom(\ITE)
        \end{align*}
        By the induction hypothesis, we have
        \begin{align*}
         \EffTypeTrans{\ITE} \cup \{x_{\Atype_1, m_1} \COL (\Atype_1, m_1, 0), \dots, x_{\Atype_k, m_k} \COL (\Atype_k, m_k, 0) \} \pInter \termalt' \COL \EffTypeTrans{\Atype'}.
        \end{align*}
        In addition, \(x_{\Atype_i, m_i} \notin dom(\EffTypeTrans{\ITE})\) for each \(i\),
         since \(x \notin dom(\ITE)\).
        Thus, by using \rn{IT-Abs} \(k\) times, we obtain the following as required:
        \[
        \EffTypeTrans{\ITE} \pInter \lambda x_{\Atype_1,m_1}\dots x_{\Atype_k,m_k}.\;\termalt'
        \COL (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to \EffTypeTrans{\Atype'}.
        \]
 \end{itemize}
\end{proof}

\begin{lemma}\label{lem:appx:liveness:translation-typable}
  If \( \TopEnv \pInter P \Rightarrow (P', \Pfun) \), then \( \EffTypeTrans{\TopEnv} \pInter P' \).
  Furthermore \( \EffTypeTrans{\TopEnv} \) is simple and \( \Pfun = \Pfun_{\EffTypeTrans{\TopEnv}} \).
\end{lemma}
\begin{proof}
 The former condition follows immediately from Lemma~\ref{lem:appx:liveness:translation-typable:pre}. \tk{to do}\wtnb{done}
 The latter condition follows immediately from the definition of
 \( \TopEnv \pInter P \Rightarrow (P', \Pfun) \).
\end{proof}

%% This is a simpler version of simulation relation lemma, but unused
%\begin{lemma}
% Assume \(\TopEnv \pInter D\),
% \(\ITE_1 \EnvRel \TopEnv\),
% \(\ITE_1 \pInter \term \COL q\) and
% \(\term_1 \Pred{\ell}{D} \term_2\).
% Then, there exists \(\ITE_2\) such that
% \(\ITE_2 \EnvRel \TopEnv\) and
% \(\ITE_2 \pInter \term_2 \COL \delta(q, \ell)\) hold.
%\end{lemma}
%\begin{proof}
% By Lemma~\ref{appx:es:lem:sim1}, we obtain \(\ITE_2 = \TopEnvZ \cup (\ITE_1 \RaiseP \SUMMARY(q, \lab))\).
%\end{proof}

\begin{lemma}
 \label{appx:es:lem:summary}
 Assume:
 \begin{align*}
  \TopEnv \pInter D \qquad
  \ITE_1 \EnvRel \TopEnv \qquad
  \ITE_2 \EnvRel \TopEnv^\Mark \qquad
  \ITE_1 \cup \ITE_2 &\pInter \term \COL q \qquad
  \term \Preds{\seq{\ell}}{D^\Mark} \term'.
 \end{align*}
 Then, there exist \(\ITE'_1\) and \(\ITE'_2\) that satisfy the following conditions.
 \begin{itemize}
  \item \(
        \ITE'_1 \EnvRel \TopEnv \qquad
        \ITE'_2 \EnvRel \TopEnv^\Mark \qquad
        \ITE'_1 \cup \ITE'_2 \pInter \term' \COL \hat{\delta}(q, \seq{\ell})
        \)
  \item  If \(f^{\Mark} : (\Atype, m, m') \in \ITE'_2\),
         there exists \(f^{\Mark} : (\Atype, m, m'') \in \ITE_2\) such that
         \(
         \MAX(m'', \SUMMARY(q, \seq{\ell})) = m'.
         \)
 \end{itemize}
\end{lemma}
\begin{proof}
 The proof proceeds by induction on the length of reduction
 \(\term \Preds{\seq{\ell}}{D^\Mark} \term'\).

 For the base case, \(\term' = \term\).
 In this case, \(\seq{\ell} = \epsilon\) and \(\SUMMARY(q, \seq{\ell}) = 0\).
 Hence, the required result holds for \(\ITE'_1 = \ITE_1\) and \(\ITE'_2 = \ITE_2\).

 For the induction step,
 suppose \(\term \Pred{\ell_1}{D^\Mark} \term_1 \Preds{\seq{\ell'}}{D^\Mark} \term'\) and \(\seq{\ell} = \ell_1 \seq{\ell'}\).

 By Lemma~\ref{appx:es:lem:sim1},
 we have
 \begin{align*}
  \TopEnvZ \cup ((\ITE_1 \cup \ITE_2) \RaiseP \SUMMARY(q, \ell_1))
  &\pInter \term_1 \COL \delta(q, \ell_1).
 \end{align*}
 Now, let \(\ITE_3 = \TopEnvZ \cup (\ITE_1 \RaiseP \SUMMARY(q, \ell_1))\) and
 \(\ITE_4 = (\ITE_2 \RaiseP \SUMMARY(q, \ell_1))\).
 Then, \(\ITE_3 \EnvRel \TopEnv\) and \(\ITE_4 \EnvRel \TopEnv^\Mark\).
 Thus, by the induction hypothesis, we have \(\ITE'_3\) and \(\ITE'_4\) such that
 \begin{itemize}
  \item   \(
          \ITE'_3 \EnvRel \TopEnv \qquad
          \ITE'_4 \EnvRel \TopEnv^\Mark \qquad
          \ITE'_3 \cup \ITE'_4 \pInter \term' \COL \hat{\delta}(\delta(q, \ell_1), \seq{\ell'})
          \)
  \item \(
         \forall f^{\Mark} : (\Atype, m, m') \in \ITE'_4.
         \exists f^{\Mark} : (\Atype, m, m'') \in \ITE_4.
        \MAX(m'', \SUMMARY(\delta(q, \ell_1), \seq{\ell'})) = m'.
        \)
 \end{itemize}
 Suppose \(f^\Mark \COL (\Atype, m, m') \in \ITE'_4\).
 In this case, we have \(f^{\Mark} : (\Atype, m, m'') \in \ITE_4\) such that
 \(\MAX(m'', \SUMMARY(\delta(q, \ell_1), \seq{\ell'})) = m'\).
 Since \(\ITE_4 = (\ITE_2 \RaiseP \SUMMARY(q, \ell_1))\),
 there exists \(f^{\Mark} : (\Atype, m, n) \in \ITE_2\) such that
 \begin{align*}
  m'
  = \MAX\{n, \SUMMARY(q, \ell_1), \SUMMARY(\delta(q, \ell_1), \seq{\ell'})\}
  = \MAX(n, \SUMMARY(q, \seq{\ell})).
 \end{align*}
 Hence, the required result holds for \(\ITE'_1 = \ITE'_3\) and \(\ITE'_2 = \ITE'_4\).
\end{proof}

\begin{lemma}
 \label{appx:es:lem:mark-type}
 Assume \(\ITE \pInter \term \COL q\).
 Then, \(\ITE \cup \ITE^\Mark \pInter \term^\Mark \COL q\) holds.
\end{lemma}
\begin{proof}
 By straightforward induction.
\end{proof}

\begin{lemma}
  \label{appx:es:lem:typeenv:summary}
  \changed{Assume that \(\TopEnv\) is simple.} \nk{Otherwise \( \Pfun_{\TopEnv}\) is undefined.}
 Assume also \( \TopEnv \pInter D \),
 \(\ITE_0 \EnvRel \TopEnv\) and
 \( \ITE_0 \pInter f\,\seq{s} : q \).
 If \( \RTyPath \Vdash f\,\seq{s} \mathrel{\stackrel{\seq{\ell}}{\red}\!\!{}_{\progd}^{N}} g\,\seq{u} \) and
 \( \RTyPath \Vdash f\,\seq{s} \CallSeqN{N}_{D} g\,\seq{u} \),
 then \( \Pfun_{\TopEnv}(g) = \SUMMARY(q, \seq{\ell}) \).
 %% then there exists \(\ITE\) such that
 %% \begin{align*}
 %%  \ITE \EnvRel \TopEnv \qquad
 %%  \ITE \pInter g\,\seq{u} : \hat{\delta}(q,\seq{\ell}) \qquad
 %%  \exists \Atype. g : (\Atype, \SUMMARY(q, \seq{\ell}), \SUMMARY(q, \seq{\ell}))) \in \ITE.
 %% \end{align*}
\end{lemma}
\begin{proof}
 Let \(n = |\seq{\termalt}|\).
 %
 %By \(\ITE_0 \pInter f\;\seq{s} \COL q\), \rn{IT-App} and \rn{IT-AppInt},
 Since \(\ITE_0 \pInter f\;\seq{s} \COL q\),
 there exist \( \Atype_0 \) and \( m_0 \) such that
 \begin{align}
   & f \COL (\Atype_0, m_0, m_0) \in \ITE_0 \nonumber\\
   & \Atype_0 = \Itype_1 \to \dots \to \Itype_n \to q \nonumber\\
   %% &I \subseteq \{1,\dots,n\} \qquad
   %% \bar{I} = \{1,\dots,n\} \setminus I \nonumber\\
   %% \forall i \in I. \Itype_i = \bigwedge_{1 \le j \le l_i} (\Atype'_{i, j}, m'_{i,j}) \qquad
   %%&\forall i \in \bar{I}. \Itype_i = \Tint \nonumber\\
   %% \forall i \in I. \forall j \in \{1,\dots,l_i\}.
   %% \ITE_0 \RaiseP m'_{i,j} &\pInter \termalt_i \COL \Atype'_{i,j} \label{eq:appx:lem:summary1}\\
   %% \forall i \in \bar{I}.
   %% \ITE_0 &\pInter \termalt_i \COL \Tint. \label{eq:appx:lem:summary2}
   & \forall i \in \{ 1,\dots,n \}.\; \ITE_0 \pInter s_i \COL \Itype_i
   \label{eq:appx:lem:summary2}
 \end{align}
 where \( \ITE_0 \pInter s \COL \bigwedge_{1 \le j \le k} (\Atype'_{j}, m_j) \) means \( \forall j \in \{1,\dots\,k\}.\, \ITE_0 \RaiseP m_j \pInter s_i : \Atype'_j \).

 Suppose \(D(f) = \lambda x_1\dots x_n. \term\).
 Since \( \TopEnv \pInter D \), %\rn{IT-Abs} and \rn{IT-AbsInt},
 we have
 \begin{align*}
  \TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
  &\pInter \term \COL q.
 \end{align*}
 By Lemma~\ref{appx:es:lem:mark-type}, we have
 \begin{align}
  \TopEnvZ \cup \TopEnvZM \cup \ITE_0 \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
  &\pInter \term^\Mark \COL q. \label{eq:appx:lem:summary:lambda}
 \end{align}

 %% By \eqref{eq:appx:lem:summary1},
 %% \eqref{eq:appx:lem:summary2},
 %% \eqref{eq:appx:lem:summary:lambda} and
 %% Lemma~\ref{appx:es:lem:weakening},
 %% \begin{align}
 %%  \forall i \in I. \forall j \in \{1,\dots,l_i\}.
 %%  (\TopEnvZ \cup \TopEnvZM \cup \ITE_0) \RaiseP m'_{i,j} &\pInter \termalt_i \COL \Atype'_{i,j} \label{eq:appx:lem:summary3:1} \\
 %%  \forall i \in \bar{I}.
 %%  (\TopEnvZ \cup \TopEnvZM \cup \ITE_0) &\pInter \termalt_i \COL \Tint. \label{eq:appx:lem:summary3:2} \\
 %%  \TopEnvZ \cup \TopEnvZM \cup \ITE_0 \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n} \label{eq:appx:lem:summary3:3}
 %%  &\pInter \term^\Mark \COL q.
 %% \end{align}

 % By \eqref{eq:appx:lem:summary3:1}, \eqref{eq:appx:lem:summary3:2}, \eqref{eq:appx:lem:summary3:3},
 %Lemma~\ref{appx:es:lem:subst:inter} and Lemma~\ref{appx:es:lem:subst:integer},
 By using Weakening (Lemma~\ref{appx:es:lem:weakening}) and Substitution Lemmas (Lemmas~\ref{appx:es:lem:subst:inter} and \ref{appx:es:lem:subst:integer}), from \eqref{eq:appx:lem:summary2} and \eqref{eq:appx:lem:summary:lambda},
 we have
 \begin{align}
  \TopEnvZ \cup \TopEnvZM \cup \ITE_0
  &\pInter [\termalt_1/x_1]\dots[\termalt_n/x_n] \term^\Mark \COL q. \label{eq:appx:lem:summary4:1}
 \end{align}

 Now, by the definition of call sequence, we have
 \begin{align}
  \RTyPath \Vdash [\termalt_1/x_1]\dots[\termalt_n/x_n] \term^\Mark \Predk{}{N-1}{D^\Mark} g^\Mark\;\seq{u'}. \label{eq:appx:lem:summary4:2}
 \end{align}

 Since \((\TopEnvZ \cup \ITE_0) \EnvRel \TopEnv\),
 \(\TopEnvZM \EnvRel \TopEnv^\Mark\),
 \eqref{eq:appx:lem:summary4:1} and
 \eqref{eq:appx:lem:summary4:2},
 by using Lemma~\ref{appx:es:lem:summary},
 we obtain \(\ITE_1\) and \(\ITE_2\) such that:
 \begin{align}
  \ITE_1 \EnvRel \TopEnv \qquad
  \ITE_2 \EnvRel \TopEnv^\Mark \qquad
  \ITE_1 \cup \ITE_2 \pInter g^\Mark\;\seq{u'} \COL \hat{\delta}(q, \seq{\ell}) \label{eq:appx:lem:summary6}\\
  \forall f^\Mark \COL (\Atype, m, m') \in \ITE_2.
  \exists f^\Mark \COL (\Atype, m, m'') \in \TopEnvZM.
  \MAX(m'', \SUMMARY(q, \seq{\ell})) = m'. \label{eq:appx:lem:summary7:0}
 \end{align}
 %% Since for every \(f^\Mark \COL (\Atype, m, m'') \in \TopEnvZM\), \(m'' = 0\) holds,
 %% by \eqref{eq:appx:lem:summary7:0},
 %% we have
 %% \begin{align}
 %%  \forall f^\Mark \COL (\Atype, m, m') \in \ITE_2.
 %%  m' = \SUMMARY(q, \seq{\ell}). \label{eq:appx:lem:summary7}
 %% \end{align}

 By \eqref{eq:appx:lem:summary6}, % and \rn{IT-App}, \rn{IT-AppInt} and \rn{IT-Var}, we have
 \(g^\Mark \COL (\Atype_1, m_1, m_1) \in \ITE_2\) for some \(\Atype_1\) and \(m_1\).
 Thus, by \eqref{eq:appx:lem:summary7:0}, there exists \( g^{\Mark} : (\Atype, m_1, m_1') \in \TopEnvZM. \) such that \( m_1 = \max \{ m_1', \SUMMARY(q,\seq{\ell}) \} \).
 By definition of \( \TopEnvZM \), \( m_1' = 0 \) and thus \( \SUMMARY(q,\seq{\ell}) = m_1 = \Pfun_{\TopEnv}(g) \).
 %% \begin{align}
 %%  g^\Mark \COL (\Atype_1, \SUMMARY(q, \seq{\ell}), \SUMMARY(q, \seq{\ell}) ) \in \ITE_2. \nonumber
 %% \end{align}

 %% Now, let \(\ITE'_2 = \{f\COL (\Atype, m, m') \mid f^\Mark \COL (\Atype, m, m') \in \ITE_2\}\).
 %% We have
 %% \(\ITE'_2 \EnvRel \TopEnv\) and
 %% \(g \COL (\Atype_1, \SUMMARY(q, \seq{\ell}), \SUMMARY(q, \seq{\ell}) ) \in \ITE'_2\).

 %% In addition, by using Lemma~\ref{appx:es:lem:sim1} repeatedly,
 %% there exists \(\ITE_3\) such that
 %% \(\ITE_3 \EnvRel \TopEnv\) and
 %% \(\ITE_3 \pInter g\;\seq{u} \COL \hat{\delta}(q, \seq{\ell})\).
 %% Thus, by Lemma~\ref{appx:es:lem:weakening}, \(\ITE'_2 \cup \ITE_3 \pInter g\;\seq{u} \COL \hat{\delta}(q, \seq{\ell})\) holds.

 %% Hence, the required result holds for \(\ITE = \ITE'_2 \cup \ITE_3\).
\end{proof}

\begin{corollary}\label{cor:liveness:summarising-priority}
 Assume \( \TopEnv \pInter (D, \mainfun) \) and \( \TopEnv \) is simple.
  %Let
  %\[
  %\RTyPath \Vdash f\,\seq{s} \stackrel{\ell_1}{\red}_D t_1 \stackrel{\ell_2}{\red}_D \cdots
  %\]
  %be the infinite reduction sequence following \( \RTyPath \) and \( \runseq \) be the run of \( \PWA \) over \( \ell_1 \ell_2 \cdots \).
  %Let
  %\[
  %\RTyPath \Vdash f\,\seq{s} \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots
  %\]
  Let
  \[
  \RTyPath \Vdash \mainfun \stackrel{\ell_1}{\red}_D t_1 \stackrel{\ell_2}{\red}_D \cdots
  \]
  be the infinite reduction sequence following \( \RTyPath \) and \( \runseq \) be the run of \( \PWA \) over \( \ell_1 \ell_2 \cdots \).
  Let
  \[
  \RTyPath \Vdash \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots
  \]
  be an infinite call-sequence following \( \RTyPath \).
  Let \( m_i \) (\( i \ge 1 \)) be the unique priority such that \( g_i : (\Atype_i, m_i) \in \TopEnv \) for some \( \Atype_i \).
  Then \( \MAX \mathbf{Inf}(\Omega(R)) = \MAX \mathbf{Inf}(m_1 m_2 \dots) \).
\end{corollary}
\begin{proof}
  Let \( \ell_1 \ell_2 \dots \) be the infinite sequence of events generated by the reduction sequence.
  Here \( \ell_i \) may be the empty sequence.
  By the definition of call-sequence,
  we have a infinite sequence \( 0 = j_0 < j_1 < j_2 < \dots \) such that
 %% \(j_0 = 0\),
 %% \(\lim_{i \to \infty} j_i = \infty\),
  \begin{align*}
  %% \RTyPath \Vdash \mainfun \Preds{\ell_1\dots \ell_{j_1}}{D} g_1\,\seq{u}_1 \Preds{\ell_{j_1 + 1}\dots\ell_{j_2}}{D} g_2\,\seq{u}_2 \Preds{\ell_{j_2 + 1}\dots\ell_{j_3}}{D} \dots \\
    \RTyPath \Vdash \mainfun  \CallSeqN{j_1}_\progd g_1\,\seq{u}_1 \CallSeqN{j_2-j_1}_\progd g_2\,\seq{u}_2 \CallSeqN{j_3 - j_2}_{\progd} \cdots.
  \end{align*}
  Let \( q_i = \hat{\delta}(\qinit, \ell_1 \dots \ell_{j_i}) \).
  Then we have
  \[
  \exists \ITE_i.\;\; \ITE_i \pInter g_i\;\seq{u}_i \COL q_i
  \quad\mbox{and}\quad \ITE_i \EnvRel \TopEnv
  \]
  by using Lemma~\ref{appx:es:lem:sim1} iteratively.
  Hence by Lemma~\ref{appx:es:lem:typeenv:summary},
  \[
  \Pfun_{\TopEnv}(g_i) = \SUMMARY(q_{i-1}, \ell_{j_{i-1} + 1} \dots \ell_{j_{i}}).
  \]

  Let \( \ell_1' \ell_2' \dots \) be the infinite sequence obtained by removing \( \epsilon \) from \( \ell_1 \ell_2 \dots \).
  Then we have an infinite sequence \( 0 = k_0 \le k_1 \le k_2 \le \dots \) such that \( \ell_1' \dots \ell_{k_i}' = \ell_1 \dots \ell_{j_i} \) (when ignoring \( \epsilon \)) for every \( i \ge 0 \).
  Then \( \lim_{i \to \infty} k_i = \infty \) since the generated event sequence is infinite by the assumption.
  Hence we have
  \[
  \Pfun_{\TopEnv}(g_i) = \MAX \{ 0, \Omega(R(k_{i-1} + 1)), \dots, \Omega(R(k_{i})) \}
  \]
  for every \( i \ge 1 \).
  Therefore the maximum number appearing infinitely often in
  \(
  R(1)\,R(2)\,R(3)\,\dots
  \)
  is equivalent to that in
  \(
  \Pfun_{\TopEnv}(g_1)\,\Pfun_{\TopEnv}(g_2)\,\Pfun_{\TopEnv}(g_3)\,\dots
  \).
%% Since \(\TopEnvZ \pInter \mainfun \COL \qinit\) and \(\TopEnv\) is simple,
%%  by using Lemma~\ref{appx:es:lem:typeenv:summary} iteratively,
%%  for each \(g_i\), we have \(\ITE_i \EnvRel \TopEnvZ\) such that
%%  \begin{align*}
%%   \ITE_i \pInter g_i\;\seq{u}_i \COL \hat{\delta}(\qinit, \ell_1\dots\ell_{j_i}) \qquad
%%   m_i = \SUMMARY(\hat{\delta}(\qinit, \ell_1\dots\ell_{j_{(i-1)}}), \ell_{j_{i-1}+1} \dots \ell_{j_{i}}) \qquad
%%   g \COL (\Atype_i, m_i, m_i) \in \ITE_i.
%%  \end{align*}
%%
%%  Now, we obtain another infinite sequence \(k_0 \le k_1 \le k_2 \le \dots\) by:
%%  \begin{align*}
%%   k_0 = 0 \qquad
%%   \text{for each \(i \ge 0\). }R(k_{i+1}) = \hat{\delta}(R(k_i), \ell_{j_{i-1} +1} \dots \ell_{j_{i}}).
%%  \end{align*}
%%  For each \(i \ge 0\), \(k_i \le j_i\) holds, since there may exists \(d\) such that
%%  \((j_{i-1}+1) \le d \le j_i\) and \(\ell_d = \epsilon\).
%%  Since we assume that every program only has infinite full traces in Section~\ref{sec:liveness},
%%  \(\lim_{i \to \infty} k_i = \infty\) also holds.
%%
%%  By the definition of \(\SUMMARY\), we have
%% \begin{align*}
%%  m_i = \MAX(\{0\} \cup \{\Omega(R(k_{i-1}+1)), \dots, \Omega(R(k_{i}))\}).
%% \end{align*}
%%
%%  Therefore,
%%  \( \max \mathbf{Inf}(\Omega(R)) = \max \mathbf{Inf}(m_1 m_2 \dots) \) holds.
\end{proof}

%As a special case of the above corollary, if \( g_i \) has a unique type binding in \( \TopEnv \) for each \( i \), then the sequence \( m_1 m_2 \dots \) is uniquely determined and the parity condition of \( m_1 m_2 \dots \) coincides with that of the run \( R \).
%Let us say that a top-level environment \( \TopEnv \) is \emph{simple} if \( \TopEnv(f) := \{ (\Atype,m) \mid f : (\Atype,m) \in \TopEnv \} \) is singleton for every \( f \in \dom(\ITE) \).
%For a simple top-level environment \( \TopEnv \), we define a priority assignment \( \Pfun_{\TopEnv} \) by \( \Pfun_{\TopEnv}(f) = m \) if \( \exists \Atype.\, f : (\Atype,m) \in \TopEnv \).


\subsubsection{Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}}
Let \( \prog = (\progd, \mainfun) \) be a program and \( \PWA \) be a parity automaton.
Suppose that \( \TopEnv \pInter \prog \Rightarrow (\prog', \Pfun) \).
Let \( \prog' = (D', \mainfun_{\qinit,0}) \).
By Lemma~\ref{lem:appx:liveness:translation-typable}, \( \EffTypeTrans{\TopEnv} \pInter \prog' \) and \( \EffTypeTrans{\TopEnv} \) is simple.
Furthermore \( \Pfun(f) = \Pfun_{\EffTypeTrans{\TopEnv}}(f) \).


(\( \Rightarrow \))
Assume that \( \InfTraces(\prog) \subseteq \Lang(\PWA) \).
Then by Lemma~\ref{lem:liveness:trace-coincidence}, \( \InfTraces(\prog') \subseteq \Lang(\PWA) \).
Suppose \( g_0 g_1 \dots \) be an infinite call-sequence of \( \prog' \).
Then \( g_0 = \mainfun_{\qinit,0} \) and there exists \( \RTyPath \) such that \( \RTyPath \Vdash \mainfun_{\qinit,0} \CallSeq_{D'} g_1\,\tilde{u}_1 \CallSeq_{D'} g_2\,\tilde{u}_1 \CallSeq_{D'} \cdots \).
Let \( \RTyPath \Vdash \mainfun_{\qinit,0} \stackrel{\ell_1}{\red}_{D'} t_1 \stackrel{\ell_2}{\red}_{D'} t_2 \stackrel{\ell_3}{\red_E} \cdots \) be the corresponding reduction sequence.
Then \( \ell_1 \ell_2 \dots \in \Lang(\PWA) \), i.e.~the unique run \( \runseq \) of \( \PWA \) over \( \ell_1 \ell_2 \dots \) satisfies the parity condition.
Let \( m_i \) (\( i \ge 1 \)) be the unique priority such that \( g_i : (\Atype_i, m_i) \in \TopEnv \) for some \( i \).
So by Corollary~\ref{cor:liveness:summarising-priority}, \( \mathbf{max} \mathbf{Inf}(\Omega(R)) = \mathbf{max} \mathbf{Inf}(\Pfun(g_0)\Pfun(g_1)\Pfun(g_2) \dots) \).
Hence \( g_0 g_1 \dots \) satisfies the parity condition with respect to \( \Pfun \), i.e.~\(\models_\CSA (P',\Pfun)\).


  (\( \Leftarrow \)) We show the contraposition.
  Suppose that \( \InfTraces(\prog) \nsubseteq \Lang(\PWA) \), which implies \( \InfTraces(\prog') \nsubseteq \Lang(\PWA) \) by Lemma~\ref{lem:liveness:trace-coincidence}.
  So there exists an infinite trace \( \ell_1 \ell_2 \dots \in \InfTraces(\prog') \) such that the unique run of \( \PWA \) over \( \ell_1 \ell_2 \dots \) violates the parity condition.
  Let \( \RTyPath \) be a choice sequence which generates \( \ell_1 \ell_2 \dots \), i.e.~\( \RTyPath \Vdash \mainfun_{\qinit,0} \stackrel{\ell_1}{\red}_{D'} t_1 \stackrel{\ell_2}{\red}_{D'} t_2 \stackrel{\ell_3}{\red_E} \cdots \).
  By Corollary~\ref{cor:liveness:unique-existence-of-call-seq}, there exists an infinite call-sequence \( \RTyPath \Vdash \mainfun_{\qinit,0} \CallSeq_{D'} g_1\,\tilde{u}_1 \CallSeq_{D'} g_2\,\tilde{u}_1 \CallSeq_{D'} \cdots \).
  By Corollary~\ref{cor:liveness:summarising-priority}, \( \mathbf{max} \mathbf{Inf}(\Omega(R)) = \mathbf{max} \mathbf{Inf}(\Pfun(g_0)\Pfun(g_1)\Pfun(g_2) \dots) \).
  Hence \( g_0 g_1 \dots \) violates the parity condition with respect to \( \Pfun \).


==> appx-liveness-effective-selection.tex <==
\subsection{Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}}

 \subsubsection{Modified type-based translation}
 %\wtnb{
 % memo: In order to represent non-determinism originated from automata,
 % I added a new syntax \(\term_1 \enondet \term_2\) and a new transformation rule \rn{(IT-Event-Alt)}.
 % Thanks to them,
 % one-step reduction in the source program corresponds to one-step reduction in the transformed program.
 % More preciously, I added rules to do the \emph{one}-step reduction like the following second line:
 % \begin{align*}
 %  \evexp{\lab}{\term} &\Pred{\lab}{\progd} \term &\text{(source program)} \\
 %  \evexp{\lab}{(\termalt_1 \enondet \dots \enondet \termalt_n)} &\Pred{\lab}{\progd'} \termalt_i &\text{(transformed program)}
 % \end{align*}
 % If I use \(\nondet\) here, the reduction takes \emph{two} steps like the following:
 % \begin{align*}
 %  \evexp{\lab}{(\termalt_1 \nondet \dots \nondet \termalt_n)} \Pred{\lab}{\progd'} (\termalt_1 \nondet \dots \nondet \termalt_n) \Pred{\epsilon}{\progd'} \termalt_i
 % \end{align*}
 %}

 Given programs \( \prog \) and \( \prog' \) with \( \TopEnv \pInter \prog \ESRel (\prog', \Pfun) \), the first step to prove Theorem~\ref{thm:linevess:eff-sel-sound-and-complete} is to compare reduction sequences of \( \prog \) and \( \prog' \).
 There is a little gap between reduction sequences of \( \prog \) and \( \prog' \) since a reduction sequence of \( \prog' \) expresses a reduction sequence of \( \prog \) together with a run of \( \PWA \) over the events generated by the reduction sequence of \( \prog \).
 In particular a nondeterministic branch in \( \term' \) comes from either
 \begin{itemize}
 \item a non-deterministic branch \( \term_1 \nondet \term_2 \) in \( P \), or
 \item non-determinism of the transition rule of the automaton \( \PWA \).
 \end{itemize}
 To fill the gap, we shall distinguish between the two kinds of non-deterministic branches, by using \( \enondet \) for the latter.

 Formally let us introduce a new binary construct \( \enondet \) to the syntax of terms.
 Here we use the convention that \( \nondet \) and \( \enondet \) are right associative, i.e.~\( t_1 \nondet t_2 \nondet t_3 \) (resp.~\( t_1 \enondet t_2 \enondet t_3 \)) means \( t_1 \nondet (t_2 \nondet t_3) \) (resp.~\( t_1 \enondet (t_2 \enondet t_3) \)).
  The operational behaviour of \( \enondet \) is the same as that of \( \nondet \), i.e.,
 \[
 (\term_1 \enondet \term_2;\, \PLeft \RTyPath) \stackrel{\epsilon}{\red}_D (\term_1; \RTyPath)
 \qquad
 (\term_1 \enondet \term_2;\, \PRight \RTyPath) \stackrel{\epsilon}{\red}_D (\term_2; \RTyPath)
 \]
 where \( \RTyPath \in \{\PLeft,\PRight\}^{\omega} \) is a choice sequence.
 Hence we have
 \[
 ((\evexp{\lab}{(\term_1 \enondet \dots \enondet \term_n)});\,
 \underbrace{\PRight \dots \PRight}_{i-1} \PLeft  \RTyPath)
 \Preds{\lab}{\progd}
 (\term_{i};\, \RTyPath)
 \]
 for \( 1 \le i < n \) and
 \[
 ((\evexp{\lab}{(\term_1 \enondet \dots \enondet \term_n)});\,
 \underbrace{\PRight \dots \PRight}_{n-1} \RTyPath)
 \Preds{\lab}{\progd}
 (\term_{n};\, \RTyPath).
 \]
 \begin{definition}[Modified type-based transformation]
   The \emph{modified type-based transformation judgement} \( \ITE \pInter \term : \Atype \eESRel \term' \) is a quadruple where \( \term \) is a term without \( \enondet \) and \( \term' \) is a term possibly having \( \enondet \).
   The \emph{modified type-based transformation relation} is defined by the rules in Fig.~\ref{appx:fig:inter-alternative}.
   The translation \(\pInter \prog \eESRel (P', \Pfun)\) of programs is defined in the same way as \(\pInter \prog \ESRel (P', \Pfun)\).
 \end{definition}
 \begin{figure}[t]
   \infrule[IT-Event-Alt]{
     \delta(q, \lab) = \{q_1, \dots, q_n\} \quad\text{(\(q_1 < q_2 < \dots < q_n\))} \\
     \ITE \RaiseP \Omega(q_i) \pInter \term \COL q_i \eESRel \term'_i \quad\text{(for each \(i \in \{1, \dots, n\}\))}
   }{
     \ITE
     \pInter
     (\evexp{\lab}{\term}) \COL q  \eESRel (\evexp{\lab}{\term'_1 \enondet \cdots \enondet \term'_n})
   }
   %% \bigskip
   %%  \infrule{
   %%   \term \neq \evexp{\lab}{\term'} \andalso
   %%   \ITE \pInter \term \COL \Atype \ESRel \term'
   %%  } {
   %%   \ITE \pInter \term \COL \Atype \eESRel \term'
   %%  }
   \caption{Modified type-based transformation rules.  Other rules are obtained by replacing \( \ESRel \) with \( \eESRel \) in the rules in Figure~\ref{fig:inter} except for \textsc{(IT-Event)}.}
  \label{appx:fig:inter-alternative}
 \end{figure}
 The next lemma establishes the connection between the original and modified transformations.
 Given a program \( \prog' \) with \( \enondet \), we write \( [\nondet/\enondet]\prog' \) for the program obtained by replacing \( \enondet \) with \( \nondet \).
 \begin{lemma}~\label{lem:appx:liveness:relating-modified-and-original-translations}%{lem:liveness:equivalence-of-two-csa}
   If \(\TopEnv \pInter \prog \eESRel (\prog', \Pfun)\), then \( \TopEnv \pInter \prog \ESRel ([\nondet/\enondet]\prog', \Pfun) \).
   Conversely, if \( \TopEnv \pInter \prog \ESRel (\prog', \Pfun) \), then there exists \( \prog'' \) such that \( \TopEnv \pInter \prog \eESRel (\prog'', \Pfun) \) and \( \prog' = [\nondet/\enondet]\prog'' \).
 \end{lemma}
 \begin{proof}
   Straightforward induction.
 \end{proof}



%%  Before the proof, we prepare some definitions.
%%  We first introduce a new non-deterministic branch operator \(\enondet\).
%%  Intuitively, this operator is used to represent non-determinism originated from automata in the call-sequence analysis.



%%  \infrule{
%%   i \in \{1, \dots, n\}
%%  }{
%%  \evexp{\lab}{(\term_1 \enondet \dots \enondet \term_n)}  \EPred{\lab}{\progd}\term_i
%%  }

%%  By using this new operator, we define a new transformation rule \(\ITE \pInter \term \COL \Atype \eESRel \term' \),
%%  which is a variant of the relation \(\ITE \pInter \term \COL \Atype \ESRel \term' \) defined in Figure~\ref{fig:inter}.
%%  \begin{definition}
%%   We define a transformation relation \(\ITE \pInter \term \COL \Atype \eESRel \term' \) by Figure~\ref{appx:fig:inter-alternative}.
%%   We also define a transformation of programs \(\pInter \prog \eESRel (P', \Pfun)\) in the same way as \(\pInter \prog \ESRel (P', \Pfun)\).
%%  \end{definition}
%%  Below, we assume without loss of generality that the sets of state of automata are totally ordered.
%%  Thanks to this assumption, we can regard this program translation as a deterministic one.
%%  \tk{This claim is highly nontrivial (and perhaps not true).  A difficulty lies in the case of application, for which the types for arguments are not defined from the conclusion.}

%%  Between the original transformation rule and this rule, the following property holds.
%% \begin{lemma}~\label{lem:liveness:equivalence-of-two-csa}
%%   Suppose that \(\TopEnv \pInter \prog \ESRel (\prog_0, \Pfun_0)\),
%%  \(\TopEnv \pInter \prog \eESRel (\prog_1, \Pfun_1)\).
%%   \(\models_\CSA (\prog_0, \Pfun_0)\) if and only if \(\models_\CSA (\prog_1, \Pfun_1)\).
%% \end{lemma}
%% \begin{proof}
%%   By straightforward induction.
%%   \tk{I think this is not so obvious.  This lemma implies the following result, which is non-trivial; If \(\TopEnv \pInter \prog \ESRel (\prog_0, \Pfun_0)\) and \(\TopEnv \pInter \prog \ESRel (\prog_1, \Pfun_1)\), then \(\models_\CSA (\prog_0, \Pfun_0)\) if and only if \(\models_\CSA (\prog_1, \Pfun_1)\).  Note that the type-based transformation has not been proved to be functional, and thus it can be the case that \( \prog_0 \neq \prog_1 \).}
%% \end{proof}

%%  We also extend the definition of choice sequences.
%%  \begin{definition}[Extended Choice sequences]
%%   Let \( \RTyPath \in \{\PLeft, \PRight\}^{\omega} \), called a \emph{(extended) choice sequence}.
%%   We define a reduction relation for pairs of terms and extended choice sequences by
%%   \begin{align*}
%%    (\term_1 \nondet \term_2;\, \PLeft \RTyPath) \Pred{\epsilon}{\progd} (\term_1; \RTyPath)
%%   \qquad
%%    (\term_1 \nondet \term_2;\, \PRight \RTyPath) \Pred{\epsilon}{\progd} (\term_2; \RTyPath)
%%   \end{align*}
%%   \infrule{
%%    0 \le i \le n-2
%%   }{
%%    ((\evexp{\lab}{(\term_1 \enondet \dots \enondet \term_n)});\,
%%    \underbrace{\PRight \dots \PRight}_{i} \PLeft  \RTyPath)
%%    \Pred{\lab}{\progd}
%%    (\term_{i+1};\, \RTyPath)
%%   }
%%   \[
%%    ((\evexp{\lab}{(\term_1 \enondet \dots \enondet \term_n)});\,
%%    \underbrace{\PRight \dots \PRight}_{n-1} \RTyPath)
%%    \Pred{\lab}{\progd}
%%    (\term_{n};\, \RTyPath)
%%   \]
%%   and \( (u; \RTyPath) \Pred{\epsilon}{\progd} (u'; \RTyPath) \)
%%   if \( u \neq u_1 \nondet u_2, u \neq (\evexp{\lab}{(u_1 \enondet \dots \enondet u_n)})\) and \( u \stackrel{\ell}{\red}_D u' \).
%%   Other notations are defined in the same way as those of original choice sequences.
%%  \end{definition}

%%  For extended choice sequences, Corollary~\ref{cor:liveness:unique-existence-of-call-seq} also holds.
%%  \wtnb{need to prove?}

 Suppose that \( \TopEnv \pInter P \eESRel (P', \Pfun) \).
 Since \( P' \) simulates both \( P \) and the automaton \( \PWA \), an infinite reduction sequence of \( P' \) induces a pair of an infinite event sequence \( \seq{\ell} \) and a run \( R \) of \( \PWA \) over \( \seq{\ell} \).
 \begin{definition}[Induced event sequence and run]
   Suppose that \( \TopEnv \pInter D \eESRel D' \) and \( \ITE \pInter \term : q \eESRel \termalt \) with \( \ITE \EnvRel \TopEnv \).
   If \( \RTyPath \Vdash \termalt \Preds[N]{\seq{\ell}}{D'} \termalt' \), we define \( \EvSeq_{\prog, \PWA}(\termalt, \RTyPath, N) = \seq{\ell} \).
   Similarly \( \EvSeq_{\prog, \PWA}(\termalt, \RTyPath, \omega) \) is the infinite event sequence generated by
   \[
   \RTyPath \Vdash \termalt \Pred{\ell_1}{D'} \termalt_1 \Pred{\ell_2}{D'} \termalt_2 \Pred{\ell_3}{D'} \cdots,
   \]
   i.e.~the unique infinite sequence of which \( \EvSeq_{\prog, \PWA}(\termalt, \RTyPath, N) \) is a prefix for each \( N \in \omega \).
  %% \(\prog = (\progd, \mainfun)\) be a program and
  %% \(\RTyPath\) be an infinite choice sequence.
  %% Suppose
  %% \[
  %% \RTyPath \Vdash \mainfun \Pred{\ell_1}{\progd} \term_1 \Pred{\ell_2}{\progd} \term_2 \Pred{\ell_3}{\progd} \dots.
  %% \]
  %% We write \(\EvSeq_{\prog, \PWA}(\RTyPath)\) for the event sequence \(\ell_1 \ell_2 \dots\).
  %% \wtnb{I want to define
  %% \(\Run_{D,\PWA}(\term, q, \RTyPath, n)\) as a label generated by a reduction of 4-tuples like
  %%  \[
  %%   (\term, q, \RTyPath_0\RTyPath_1, n) \stackrel{q}{\rightharpoonup}_D (\term', q', \RTyPath_1, n-1) \stackrel{q'}{\rightharpoonup}_D \dots.
  %%  \]
  %%  I think this style of a definition makes the proof of Lemma~\ref{lem:liveness:eff-sel-red-sim-multi-sim1} easier.
  %% }
  Given \( N \in \omega \), the corresponding run \(\Run_{D', \PWA}(q, \termalt, \RTyPath, N)\) of \(\PWA\) is defined by the following rules:
  %
  \infrule{
    \mathstrut
  }{
    \Run_{D, \PWA}(q, \termalt, \RTyPath, 0) = q
  }
  \infrule{
    (\termalt;\, \RTyPath) \Pred{\epsilon}{\progd'} (\termalt';\, \RTyPath')
  }{
    \Run_{D,\PWA}(q, \termalt, \RTyPath, N) = \Run_{D,\PWA}(q, \termalt', \RTyPath', N-1)
  }
  \infrule{
    \delta(q, \lab) = \{q_{1}, \dots, q_{n}\} \quad\text{ (\( q_1 < q_2 < \dots < q_n \))}
    \qquad
    j < n
  }{
    \Run_{D,\PWA}(q, (\evexp{\lab}{(\termalt_1 \enondet \dots \enondet \termalt_n)}), \PLeft^{j-1} \PRight \RTyPath, 1+j+N) = q \; \Run_{D',\PWA}(q_{j}, \termalt_j, \RTyPath, N)
  }
  \infrule{
    \delta(q, \lab) = \{q_{1}, \dots, q_{n}\} \quad\text{ (\( q_1 < q_2 < \dots < q_n \))}
  }{
    \Run_{D,\PWA}(q, (\evexp{\lab}{(\termalt_1 \enondet \dots \enondet \termalt_n)}), \PLeft^{n-1} \RTyPath, n+N) = q \; \Run_{D',\PWA}(q_{n}, \termalt_n, \RTyPath, N)
  }
  %
  It is easy to see that \( \Run_{D,\PWA}(q, \termalt, \RTyPath, N) \) is a prefix of \( \Run_{D,\PWA}(q, \termalt, \RTyPath, N') \) when \( N \le N' \).
  We write \( \Run_{D,\PWA}(q, \termalt, \RTyPath, \omega) \) for the shortest sequence of which \( \Run_{D,\PWA}(q, \termalt, \RTyPath, N) \) is a prefix for every \( N \in \omega \).
  We write \(\Run_{\prog, \PWA}(\RTyPath)\) for \(\Run_{\progd, \PWA}(\qinit, \mainfun, \RTyPath)\) where \(\prog = (\progd, \mainfun)\).
  \wtnb{\(\Run_{\progd, \PWA}(\qinit, \mainfun, \RTyPath,\omega)\)?}
 \end{definition}

 \begin{lemma}
   Suppose that \( \TopEnv \pInter D \eESRel D' \) and \( \ITE \pInter \term : q \eESRel \termalt \) with \( \ITE \EnvRel \TopEnv \).
   Let \( N \in \omega \), \( \RTyPath \in \{\PLeft, \PRight\}^{\omega} \) be a choice sequence and \( \termalt' \) be the unique term such that \( \RTyPath \Vdash \termalt \Preds[N]{\seq{\ell}}{D'} \termalt' \).
   If \( \termalt' \) is not of the form \( \termalt'_1 \enondet \termalt'_2 \), then \( \Run_{D,\PWA}(q, \termalt, \RTyPath, N) \) is a run of \( \PWA \) over \( \seq{\ell} \) starting from \( q \).
 \end{lemma}
 \begin{proof}
   \tk{to do}
 \end{proof}

 \begin{corollary}\label{cor:liveness:eff-sel-induced-run}
   Suppose that \( \TopEnv \pInter D \eESRel D' \) and \( \ITE \pInter \term : q \eESRel \termalt \) with \( \ITE \EnvRel \TopEnv \).
   Let \( \RTyPath \in \{\PLeft, \PRight\}^{\omega} \) be a choice sequence.
   Then \( \Run_{D,\PWA}(q, \termalt, \RTyPath, \omega) \) is an infinite run of \( \PWA \) over the infinite sequence \( \EvSeq_{\prog, \PWA}(\termalt, \RTyPath, \omega) \).
 \end{corollary}
 %% Note that \(\Run_{\prog, \PWA}(\RTyPath)\) is a run of \(\PWA\) over \(\EvSeq_{\prog, \PWA}(\RTyPath)\) for any \(\RTyPath \in \{\PLeft, \PRight\}\).
 %% In addition, \(\EvSeq_{\prog, \PWA}(\RTyPath)\) and \(\Run_{\prog, \PWA}(\RTyPath)\) are defined for any \(\RTyPath \in  \{\PLeft, \PRight\}^{\omega}\)
 %% by the assumption that both reductions of programs and runs of automata do not stuck.

\subsubsection{Notations}
Given an intersection type \( \Itype = \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \) and a variable \( x \), we abbreviate the sequence \( x_{\Atype_1, m_1} x_{\Atype_2, m_2} \dots x_{\Atype_k, m_k} \) as \( \dup{x,\Itype} \).
For \( \Itype = \INT \), we write \( \dup{x,\Itype} \) for \( x_{\INT} \).

For an intersection type \( \Itype = \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \), we write \( \ZEnv{x : \Itype} \) for the intersection type environment \( \{ x : (\Atype_i, m_i, 0) \mid 1 \le i \le k \} \).
If \(\Itype = \Tint\), \(\ZEnv{x \COL \Itype}\) means \(\{x \COL \Tint\}\).
Similarly, for a top-level environment \( \TopEnv \), we write \( \TopEnvZ \) to mean \( \{ x : (\Atype, m, 0) \mid x : (\Atype, m) \in \TopEnv \} \).

Given an intersection type environment \( \ITE \), we write \( \ITE^{\Mark} \) for \( \{ x^{\Mark} : (\Atype, m, m') \mid x : (\Atype, m, m') \in \ITE \} \cup \{ x^{\Mark} : \INT \mid x : \INT \in \ITE \} \).
Similarly, for a top-level environment \( \TopEnv \), we write \( \TopEnv^{\Mark} \) for \( \{ x^{\Mark} : (\Atype, m) \mid x : (\Atype, m) \in \TopEnv \} \).

For an intersection type environment \( \ITE \) and a top-level environment \( \TopEnv \), we write \(\ITE \EnvRel \TopEnv\) if
\(f \COL (\Atype, m) \in \TopEnv\) for each \((f \COL (\Atype, m, m')) \in \ITE\).
%%it satisfies the following conditions: if \((f \COL (\Atype, m, m')) \in \ITE\), then \(f \COL (\Atype, m) \in \TopEnv\).

%\input{appx-liveness-effective-selection-draft}

\subsubsection{Basic properties of the type system and transformation}

\begin{lemma}[Weakening]
 \label{appx:es:lem:weakening}
 If \(\ITE \pInter \term \COL \Atype \eESRel \term'\) and \(\ITE \subseteq \ITE'\),
 then \(\ITE' \pInter \term \COL \Atype \eESRel \term'\).
\end{lemma}
\begin{proof}
  Straightforward induction on structure of the derivations.
  We discuss only one case below.
  \begin{itemize}
   \item Case for \rn{IT-Event-Alt}:
    Then we have
    \begin{align*}
      \Atype = q \qquad
      \delta(q, \lab) = \{q_1, \dots, q_n\} \qquad
      \term &= \evexp{\lab}{\termalt} \qquad
      \term' = \evexp{\lab}{(\termalt_1' \enondet \dots \enondet \termalt_n')} \\
     \forall i \in \{1, \dots, n\}. &\ITE \RaiseP \Omega(q_i) \pInter \termalt \COL \Atype \eESRel \termalt'_i.
    \end{align*}
    Since \(\ITE \subseteq \ITE'\), for each \(i \in \{1, \dots, n\}\), we have \(\ITE \RaiseP \Omega(q_i) \subseteq \ITE' \RaiseP \Omega(q_i)\).
    By the induction hypothesis,
    \[
     \forall i \in \{1, \dots, n\}. \ITE' \RaiseP \Omega(q_i) \pInter \termalt \COL \Atype \eESRel \termalt'_i.
    \]
    By using \rn{IT-Event-Alt}, we obtain
    \(\ITE' \pInter \term \COL \Atype \eESRel \term'\).
  %\item Case for \rn{IT-Event}:
  %  Then
  %  \begin{align*}
  %    \Atype = q \qquad
  %    \term = \evexp{\lab}{\termalt} \qquad
  %    \term' = \evexp{\lab}{\termalt'} \qquad
  %    \ITE \RaiseP \Omega(\delta(q, \lab)) \pInter \termalt \COL \Atype \eESRel \termalt'.
  %  \end{align*}
  %  Since \(\ITE \subseteq \ITE'\), we have \(\ITE \RaiseP \Omega(\delta(q, \lab)) \subseteq \ITE' \RaiseP \Omega(\delta(q, \lab))\).
  %  By the induction hypothesis,
  %  \[
  %  \ITE' \RaiseP \Omega(\delta(q, \lab)) \pInter \termalt \COL \Atype \eESRel \termalt'.
  %  \]
  %  By using \rn{IT-Event}, we obtain
  %  \(\ITE' \pInter \term \COL \Atype \eESRel \term'\).
  \end{itemize}
\end{proof}


\begin{lemma}[Substitution (Integer)]
 \label{appx:es:lem:subst:integer}
 Assume \(\ITE, x \COL \Tint \pInter \term \COL \Atype \eESRel \term'\) and
 \(\ITE \pInter u \COL \Tint \eESRel u'\).
 Then, \(\ITE \pInter [u/x] \term \COL \Atype \eESRel [u'/\xint]\term'\) holds.
\end{lemma}
\begin{proof}
 By straightforward induction.
\end{proof}



\begin{lemma}[Substitution (Intersection Type)]
 \label{appx:es:lem:subst:inter}
 Assume:
 \begin{align*}
  \Itype = \bigwedge_{1 \le i \le l} (\Atype_i, m_i) \qquad
  &x \notin dom(\ITE) \\
  ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' \pInter \term \COL \Atype \eESRel \term' \qquad
  &\forall i \in \{1,\dots,l\}.\ \ITE \RaiseP m_i \pInter u \COL \Atype_i \eESRel u'_i.
 \end{align*}
 Then,
 \[
 (\ITE \RaiseP n) \cup \ITE' \pInter [u/x] \term \COL \Atype \eESRel [\seq{u}'/\dup{x,\Itype}]t'.
 \]
 % Then, \(\ITE \RaiseP n \pInter [u/x] \term \COL \Atype \eESRel [u'_1/x_{\Atype_1, m_1}]\dots[u'_l/x_{\Atype_l, m_l}] t'\) holds.
\end{lemma}
\begin{proof}
 The proof proceeds by induction on the derivation of
 \((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \pInter \term \COL \Atype \eESRel \term'\),
 with case analysis on the last rule used.

 \begin{itemize}
  \item Case for \rn{IT-Var}:
        The case where \(\term \neq x\) is trivial.
        Assume that \(\term = x\).
        Then there exists \(k \in \{1, \dots, l\}\) such that \( \theta = \theta_k \), \( t' = x_{\theta_k,m_k} \) and \( n = m_k \).
        %% \begin{align*}
        %%   (\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n &\pInter x \COL \Atype_k \eESRel x_{\Atype_k, m_k} \\
        %%  n &= m_k \tag{Since \(x \COL (\Atype_k, m_k, m_k) \in (\ITE \cup \ZEnv{x \COL \Itype})\RaiseP n\)}
        %% \end{align*}
        By the assumption, we have \(\ITE \RaiseP m_k \pInter u \COL \Atype_k \eESRel u'_k\).
        Since \([u/x]x = u\) and \([\seq{u'}/\dup{x,\Itype}]x_{\Atype_k, m_k} = u'_k\), we have
        \begin{align*}
         \ITE \RaiseP m_k &\pInter [u/x]x \COL \Atype_k \eESRel [\seq{u'}/\dup{x,\Itype}] x_{\Atype_k, m_k}.
        \end{align*}
        By Lemma~\ref{appx:es:lem:subst:inter}, we have
        \begin{align*}
         (\ITE \RaiseP m_k) \cup \ITE' &\pInter [u/x]x \COL \Atype_k \eESRel [\seq{u'}/\dup{x,\Itype}] x_{\Atype_k, m_k}.
        \end{align*}
        as required.
  \item Case for \rn{IT-Event-Alt}:
        Then \(\term = \evexp{\lab}{\term_1}\) and we have
        \begin{align*}
         \Atype = q \qquad
         \delta(q, \lab) = \{q_1, \dots, q_k\} \qquad
         \term'=\evexp{\lab}{(\term'_1 \enondet \dots \enondet \term'_k)} \\
         \forall j \in \{1, \dots, k\}. (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(q_j) &\pInter \term_1 \COL q_j \eESRel \term'_j.
        \end{align*}
        For each \(j \in \{1, \dots, k\}\), we have
        \begin{align*}
          & (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(q_j) \\
          & = ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \RaiseP \Omega(q_j)) \cup (\ITE' \RaiseP \Omega(q_j)).
        \end{align*}
        Thus, one can apply the induction hypotheses, obtaining
        \begin{align*}
         \forall j \in \{1, \dots, k\}. ((\ITE  \RaiseP n) \cup \ITE') \RaiseP \Omega(q_j) &\pInter [u/x] \term_1 \COL q_j \eESRel  [\seq{u'}/\dup{x,\Itype}] \term'_j.
        \end{align*}
        By using \rn{IT-Event-Alt}, we have the following as required:
        \begin{align*}
         (\ITE  \RaiseP n) \cup \ITE' &\pInter [u/x] (\evexp{\lab}{\term_1}) \COL q \eESRel  [\seq{u'}/\dup{x,\Itype}] (\evexp{\lab}{(\term'_1 \enondet \dots \enondet \term'_k)}).
        \end{align*}
  %\item Case for \rn{IT-Event}:
  %      Then \(\term = \evexp{\lab}{\term_1}\) and we have
  %      \begin{align*}
  %       \term'=\evexp{\lab}{\term'_1} \qquad
  %       \Atype = q \\
  %       (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) &\pInter \term_1 \COL \delta(q, \lab) \eESRel \term'_1.
  %      \end{align*}
  %      Since
  %      \begin{align*}
  %        & (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) \\
  %        & = ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \RaiseP \Omega(\delta(q,\lab))) \cup (\ITE' \RaiseP \Omega(\delta(q, \lab))),
  %      \end{align*}
  %      one can apply the induction hypothesis, obtaining
  %      \begin{align*}
  %       ((\ITE  \RaiseP n) \cup \ITE') \RaiseP \Omega(\delta(q, \lab)) &\pInter [u/x] \term_1 \COL \delta(q, \lab) \eESRel  [\seq{u'}/\dup{x,\Itype}] \term'_1.
  %      \end{align*}
  %      By using \rn{IT-Event}, we have the following as required:
  %      \begin{align*}
  %       \ITE \RaiseP n &\pInter [u/x] (\evexp{\lab}{\term_1}) \COL q \eESRel  [\seq{u'}/\dup{x,\Itype}] (\evexp{\lab}{\term'_1}).
  %      \end{align*}
  \item Case for \rn{IT-App}:
        Then \(\term=\term_1\;\term_2\) and we have
        \begin{align*}
         \term'=\term'_1\;\term'_{2,1}\dots \term'_{2,k} \qquad
         ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' &\pInter \term_1 \COL \bigwedge_{1 \le j \le k}(\Atype'_{j}, m'_{j}) \to \Atype
         \eESRel \term'_1 \\
         \forall j \in \{1,\dots,k\}. (((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE') \RaiseP m'_{j} &\pInter \term_2 \COL \Atype'_{j} \eESRel \term'_{2,j}.
        \end{align*}
        By the induction hypothesis, we have
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' \pInter [u/x]\term_1 \COL \bigwedge_{1 \le j \le k}(\Atype'_{j}, m'_{j}) \to \Atype
         \eESRel [\seq{u'}/\dup{x,\Itype}]\term'_1 \\
         \forall j \in \{1,\dots,k\}. ((\ITE \RaiseP n) \cup \ITE') \RaiseP m'_{j} \pInter [u/x]\term_2 \COL \Atype'_{j} \eESRel [\seq{u'}/\dup{x,\Itype}] \term'_{2,j}.
        \end{align*}
        By using \rn{IT-App}, we obtain:
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' &\pInter [u/x](\term_1\;\term_2) \COL \Atype
         \eESRel [\seq{u'}/\dup{x,\Itype}](\term'_1\;\term'_{2,1}\dots\term'_{2,k})
        \end{align*}
        as required.
  \item Case for \rn{IT-Abs}:
        Then \(\term=\lambda y.\termalt\) and we have
        \begin{align*}
         \Atype = \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j) \to \Atype'_0 \qquad
         &\term'=\lambda y_{\Atype'_1,m'_1}\dots y_{\Atype'_k,m'_k}. s' \\
         y \not\in dom((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \qquad
         &((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n) \cup \ITE' \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)} \pInter \termalt \COL \Atype'_0
         \eESRel \termalt'
        \end{align*}
        %% Since
        %% \[
        %% ((\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n, \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)}) \RaiseP 0 = (\ITE \cup \ZEnv{x \COL \Itype}) \RaiseP n \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)},
        %% \]
        By the induction hypothesis, we have
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE' \cup \ZEnv{y \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j)} &\pInter [u/x]\termalt \COL \Atype'_0
         \eESRel [\seq{u'}/\dup{x,\Itype}] \termalt'.
        \end{align*}
        By using \rn{IT-Abs}, we obtain:
        \begin{align*}
         (\ITE \RaiseP n) \cup \ITE'
         &\pInter [u/x]\lambda y.\termalt \COL \bigwedge_{1 \le j \le k} (\Atype'_j, m'_j) \to \Atype'_0
         \eESRel [\seq{u'}/\dup{x,\Itype}]
         \lambda y_{\Atype'_1,m'_1}\dots y_{\Atype'_k,m'_k}. \termalt'
        \end{align*}
        as required.
 \end{itemize}
\end{proof}




\subsubsection{Translation preserves traces}
The next lemma shows that the reduction of the original program can be simulated by the result of translation.
(It also proves an additional result on types, which shall be used.)
\begin{lemma}
  \label{appx:es:lem:sim1}
  Assume
  \begin{itemize}
   \item \( \TopEnv \pInter D \eESRel D' \),
   \item \( \ITE \pInter \term \COL q \eESRel \termalt \),
   \item \( \ITE \EnvRel \TopEnv \), and
   \item \(\term \Preds{\seq{\ell}}{D} \term' \).
  \end{itemize}
  Let \(\runseq \) be an arbitrary run of \( \PWA \) over \( \seq{\ell} \) starting from \( q \) and ending with \( q' \).
  Then there exist a choice sequence \( \RTyPath \in \{\PLeft, \PRight\}^{\omega} \) and a term \( \termalt' \) and a type environment \( \ITE' \EnvRel \TopEnv \) such that
  \[
  \RTyPath \Vdash \termalt \Preds[N]{\seq{\ell}}{D'} \termalt'
  \]
  and
  \[
  \ITE' \pInter \term' \COL q' \eESRel \termalt'
  \]
  and \( \runseq = \Run_{D',\PWA}(q, \termalt, \RTyPath, N) \).
\end{lemma}
\begin{proof}
  By induction on the length of the reduction sequence \(\term \Preds{\seq{\ell}}{D} \term' \).
  The claim trivially holds if the length is \( 0 \); we assume that the length is not \( 0 \).
  The proof proceeds by case analysis on the shape of \(\term\).
 \begin{itemize}
  \item Case \( \term = \evexp{\lab}{\term_1} \):
        Since the last rule used to derive \( \ITE \pInter \term \COL q \eESRel \termalt \) is \rn{IT-Event-Alt}, we have:
        \begin{align*}
         \delta(q, \lab) &= \{q_1, \dots, q_k\} \text{ (\( q_1 < q_2 < \dots < q_k \))} \\
         \forall i \in \{1, \dots, k\}. \ITE \RaiseP \Omega(q_i) &\pInter \term_1 \COL q_i \eESRel \termalt_i \\
         \termalt &= \evexp{\lab}{(\termalt_1 \enondet \dots \enondet \termalt_k)}.
        \end{align*}
        Since \( \runseq \) is a run over \( \seq{\ell} = \lab \seq{\ell}' \), it must be of the form \( \runseq = q q_i \runseq' \) for some \( 1 \le i \le k \), where \( q_i \runseq' \) is a run over \( \seq{\ell}' \).
        By applying the induction hypothesis to \( \term_1 \Preds{\seq{\ell}'}{D} \term' \), we have
        \[
        \ITE' \pInter \term' \COL q' \eESRel \termalt'
        \qquad
        \RTyPath \Vdash \termalt_i \Preds[N']{\seq{\ell}'}{D'} \termalt'
        \qquad
        q_i \runseq' = \Run_{D',\PWA}(q_i, \termalt_i, \RTyPath, N').
        \]
        for some \( \ITE' \EnvRel \TopEnv \), \( \termalt' \) and \( \RTyPath \).
        Then we have
        \[
        \RTyPath_0 \RTyPath \Vdash \evexp{\lab}{(\termalt_1 \enondet \dots \enondet \termalt_k)} \Preds[N'']{\lab}{D'} \termalt_i \Preds[N']{\seq{\ell}'}{D'} \termalt'
        \]
        for an appropriate \( \RTyPath_0 \).
        Obviously \( R = qq_i\runseq' = \Run_{D',\PWA}(q, \termalt, \RTyPath_0\RTyPath, N'' + N') \).
  \item Case \(\term = \term_1 \nondet \term_2\):
        Suppose that the reduction sequence is \( \term \Pred{\epsilon}{D} \term_1 \Preds{\seq{\ell}}{D} \term' \);
        the case that \( \term \Pred{\epsilon}{D} \term_2 \Preds{\seq{\ell}}{D} \term' \) can be proved similarly.
        Since the last rule used to derive \( \ITE \pInter \term \COL q \eESRel \termalt \) is \rn{IT-NonDet}, we have:
        \begin{align*}
         \termalt = \termalt_{1} \nondet \termalt_{2} \qquad
         \ITE \pInter \term_{1} \COL q \eESRel \termalt_{1} \qquad
         \ITE \pInter \term_{2} \COL q \eESRel \termalt_{2}
        \end{align*}
        By applying the induction hypothesis to \( \term_1 \Preds{\seq{\ell}}{D} \term' \), we have
        \[
        \ITE' \pInter \term' \COL q' \eESRel \termalt'
        \qquad
        \RTyPath \Vdash \termalt_1 \Preds[N']{\seq{\ell}}{D'} \termalt'
        \qquad
        \runseq = \Run_{D',\PWA}(q, \termalt_1, \RTyPath, N').
        \]
        for some \( \ITE' \EnvRel \TopEnv \), \( \termalt' \) and \( \RTyPath \).
        Then
        \[
        \PLeft \RTyPath \Vdash \termalt_1 \nondet \termalt_2 \Pred{\epsilon}{D'} \termalt_1 \Preds[N']{\seq{\ell}'}{D'} \termalt'
        \]
        and \( R = \Run_{D',\PWA}(q, \termalt, \PLeft \RTyPath, 1+N') \).
  \item Case \(\term = \ifexp{p(\term_{1}, \dots, \term_{n})}{\term_{n+1}}{\term_{n+2}}\):
        Suppose \((\sem{\term_{1}}, \dots, \sem{\term_{n}}) \in \sem{p}\).
        Then the reduction sequence is \( \term \Pred{\epsilon}{D} \term_{n+1} \Preds{\seq{\ell}}{D} \term' \).
        Since the last rule used to derive \( \ITE \pInter \term \COL q \eESRel \termalt \) is \rn{IT-IF}, we have:
        \begin{align*}
         \termalt &= \ifexp{p(\termalt_{1}, \dots, \termalt_{n})}{\termalt_{n+1}}{\termalt_{n+2}} \qquad
         \forall i \in \{1,\dots, n\}.
         \ITE \pInter \term_{i} \COL \Tint \eESRel \termalt_{i} \\
         \ITE &\pInter \term_{n+1} \COL q \eESRel \termalt_{n+1} \qquad
         \ITE \pInter \term_{n+2} \COL q \eESRel \termalt_{n+2}
        \end{align*}
        By the well-typedness of the program,
        for every \(i \in \{1,\dots,n\}\), \(\term_{i}\) consists of only integers and integer operations.
        Thus, we have \(\sem{\term_i} = \sem{\termalt_i}\) for each \(i \in \{1,\dots,n\}\) and
        \(\termalt \Pred{\epsilon}{D'} \termalt_{n+1}\).
        
        By applying the induction hypothesis to \( \term_{n+1} \Preds{\seq{\ell}}{D} \term' \),  we have
        \[
        \ITE' \pInter \term' \COL q' \eESRel \termalt'
        \qquad
        \RTyPath \Vdash \termalt_1 \Preds[N']{\seq{\ell}}{D'} \termalt'
        \qquad
        \runseq = \Run_{D',\PWA}(q, \termalt_{n+1}, \RTyPath, N').
        \]
        for some \( \ITE' \EnvRel \TopEnv \), \( \termalt' \) and \( \RTyPath \).
        Then
        \[
        \RTyPath \Vdash \termalt \Pred{\epsilon}{D'} \termalt_{n+1} \Preds[N']{\seq{\ell}'}{D'} \termalt'
        \]
        and \( R = \Run_{D',\PWA}(q, \termalt, \PLeft \RTyPath, 1+N') \).

        The case where
        \((\sem{\term_{1}}, \dots, \sem{\term_{n}}) \notin \sem{p}\) is similar.
  \item Case \(\term = f\;\term_1\dots \term_n\):
        Suppose \(D(f) = \lambda x_1\dots x_n. \term_0\).
        In this case, the reduction sequence is \( \term \Pred{\epsilon}{D} [\term_1/x_1]\dots[\term_n/x_n]\term_0 \Preds{\seq{\ell}}{D} \term' \).
        Since \( \ITE \pInter \term : q \eESRel \termalt \), we have
        \begin{align}
         \ITE \pInter f \COL \Atype \eESRel f_{\Atype, m} \nonumber\\
         \Atype = \Itype_1 \to \dots \Itype_n \to q \qquad
         I &\subseteq \{1, \dots, n\} \qquad
         \bar{I} = \{1,\dots,n\}\setminus I \nonumber\\
         \forall i \in I. \Itype_i = \bigwedge_{1 \le j \le \ell_i} (\Atype'_{i,j}, m'_{i,j}) \qquad
         &\forall i \in \bar{I}. \Itype_i = \Tint \nonumber\\
         \forall i \in I. \forall j \in \{1, \dots, \ell_i\}.
         (\ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j}
         \eESRel \termalt_{i, j}
         \label{appx:es:lem:sim1:1} \\
         \forall i \in \bar{I}.
         \ITE \cup \ITE' &\pInter \term_{i} \COL \Tint
         \eESRel \termalt_{i, 1}
         \label{appx:es:lem:sim1:2} \\
         \forall i \in \{1,\dots,n\}. \seq{\termalt_{i}} &=
         \begin{cases}
          \termalt_{i,1} \dots \termalt_{i,\ell_i} & (i \in I) \\
          \termalt_{i,1} & (\text{otherwise})
         \end{cases} \nonumber\\
         \termalt &= f_{\Atype, m}\;\seq{\termalt_{1}}\dots\seq{\termalt_{n}} \nonumber
        \end{align}

        Since \(\TopEnv \pInter D \eESRel D' \), 
        we have
        \begin{align}
          D'(f_{\Atype,m}) = \lambda \dup{x_1, \Itype_1}\dots\dup{x_n, \Itype_n}. \termalt_0
          \\
         \TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
         &\pInter \term_0 \COL q
         \eESRel \termalt_0
         \label{appx:es:lem:sim1:4}
        \end{align}


        By using Lemma~\ref{appx:es:lem:weakening} with
        \eqref{appx:es:lem:sim1:1}, \eqref{appx:es:lem:sim1:2} and \eqref{appx:es:lem:sim1:4},
        we have
        \begin{align}
         (\TopEnvZ \cup \ITE) \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j} \eESRel s_{i,j} \label{appx:es:lem:sim1:5} \\
         \forall i \in \bar{I}.
         (\TopEnvZ \cup \ITE) &\pInter \term_{i} \COL \Tint \label{appx:es:lem:sim1:6} \eESRel s_{i,1} \\
         \TopEnvZ \cup \ITE \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
         &\pInter \term_0 \COL q
         \eESRel \termalt_0
         \label{appx:es:lem:sim1:7}
        \end{align}

        Since
        \[
        (\TopEnvZ \cup \ITE \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}) \RaiseP 0 =
        \TopEnvZ \cup \ITE \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n},
        \]
        by using Lemma~\ref{appx:es:lem:subst:inter} and Lemma~\ref{appx:es:lem:subst:integer} repeatedly
        with \eqref{appx:es:lem:sim1:5}, \eqref{appx:es:lem:sim1:6} and \eqref{appx:es:lem:sim1:7},
        we have
        \begin{align*}
         \TopEnvZ \cup \ITE &\pInter [\term_{1}/x_1] \dots [\term_{n}/x_n] \term_0 \COL q
         \eESRel [\seq{\termalt_1}/\dup{x_1, \Itype_1}]\dots [\seq{\termalt_n}/\dup{x_n, \Itype_n}] \termalt_0.
        \end{align*}
        Since \( (\TopEnvZ \cup \ITE) \EnvRel \TopEnv \), we can apply the induction hypothesis to \( [\term_1/x_1]\dots[\term_n/x_n]\term_0 \Preds{\seq{\ell}}{D} \term' \); we have
        \[
        \ITE' \pInter \term' \COL q' \eESRel \termalt'
        \qquad
        \RTyPath \Vdash \termalt'' \Preds[N']{\seq{\ell}}{D'} \termalt'
        \qquad
        \runseq = \Run_{D',\PWA}(q, \termalt'', \RTyPath, N')
        \]
        for some \( \ITE' \EnvRel \TopEnv \), \( \termalt' \) and \( \RTyPath \), where
        \[
        \termalt'' = [\seq{\termalt_1}/\dup{x_1, \Itype_1}]\dots [\seq{\termalt_n}/\dup{x_n, \Itype_n}] \termalt_0.
        \]
        We have \( \termalt \Pred{\epsilon}{D'} \termalt'' \Preds{\seq{\ell}}{D'} \termalt' \) and \( R = \Run_{D',\PWA}(q, \termalt, \RTyPath, 1+N') \) as desired.
 \end{itemize}
\end{proof}

We show the converse in a bit stronger form.
\begin{lemma}
 \label{appx:es:lem:summary}
 Assume:
 \begin{align*}
  \TopEnv \pInter D \eESRel D' \qquad
  \ITE_1 \EnvRel \TopEnv \qquad
  \ITE_2 \EnvRel \TopEnv^\Mark \qquad
  \ITE_1 \cup \ITE_2 &\pInter \term \COL q \eESRel \termalt \qquad
  \RTyPath \Vdash \termalt \Preds[N]{\seq{\ell}}{D'^\Mark} \termalt'
 \end{align*}
 where \( \term \) is an applicative term (i.e.~a term without abstraction) and \( \termalt' \) is not of the form \( \termalt'_1 \enondet \termalt'_2 \).
 Let \( \runseq = \Run_{\prog, \PWA}(q, \termalt, \RTyPath, N) \) be the run over \( \seq{\ell} \) corresponding to the reduction sequence and \( q' \) be the last state in \( \runseq \).
 Then there exists \( \term' \) and \( \ITE_1' \) such that
 \[
 \ITE_1' \EnvRel \TopEnv \qquad
 \ITE_1' \cup (\ITE_2 \RaiseP{\SUMMARY(\runseq)}) \pInter \term' \COL q' \eESRel \termalt' \qquad
 \term \Preds{\seq{\ell}}{D^\Mark} \term'.
 \]
\end{lemma}
\begin{proof}
  \tk{Now the proof does not rely on the simulation lemmas.}
  By induction on the length \( N \) of the reduction sequence.
  If \( N = 0 \), then \(\term' = \term\) and \( \seq{\ell} = \epsilon\); so \(\runseq = q\) and \( \SUMMARY(\runseq) = 0\).
  Hence the required result holds for \( s' = s \) and \(\ITE'_1 = \ITE_1\).

  Assume that \( N > 0 \).
  The proof proceeds by case analysis on the shape of \(\termalt\).
  By the assumption
  \(\termalt \Preds[N]{\ell}{D'^\Mark} \termalt'\), it suffices to consider
  only the cases where the shape of \(\termalt\) mathces the lefthand side of a transition rule.
 \begin{itemize}
  \item Case \(\termalt = \evexp{\lab}{\termalt_0}\):
        By the shape of \(\termalt\),
        the last rule used on the derivation of \(\ITE \cup \ITE' \pInter \term \COL q \eESRel \termalt\) is
        either \rn{IT-Event-Alt} or \rn{IT-App} (\rn{IT-Abs} is not applicable since \( \term \) is assumed to have no abstraction).
        By induction on the derivation, one can prove that \( \term = (\evexp{\lab}{\term_0})\,\term_1\,\dots\,\term_k \) for some \( k \).
        By the simple-type system, one cannot apply \( \evexp{\lab}{\term_0} \) to a term; hence \( k = 0 \) (i.e.~\( \term = \evexp{\lab}{\term_0} \)) and the last rule used on the derivation is \rn{IT-Event-Alt}.
        Then we have:
        \begin{align*}
         \delta(q, \lab) &= \{q_1, \dots, q_l\} \text{ (\( q_1 < q_2 < \dots < q_l \))} \\
         \forall i \in \{1, \dots, l\}. (\ITE_1 \cup \ITE_2) \RaiseP \Omega(q_i) &\pInter \term_0 \COL q_i \eESRel \termalt_i \\
         \termalt_0 = (\termalt_1 \enondet \dots \enondet \termalt_l)
        \end{align*}
        %\begin{align*}
        % (\ITE \cup \ITE') \RaiseP \Omega(\delta(q, a)) \pInter \term_1 \COL \delta(q,\lab) \eESRel \termalt_1 \qquad
        % \term = \evexp{\lab}{\term_1}
        %\end{align*}
        Recall that \( \termalt' \) is not of the form \( \termalt'_1 \enondet \termalt'_2 \); hence the reduction sequence
        \[
        (\termalt, \RTyPath) \Preds[N]{\seq{\ell}}{D'^\Mark} (\termalt', \RTyPath')
        \]
        must be of the form
        \[
        (\termalt, \RTyPath) \Preds[N_1]{\lab}{D'^{\Mark}} (\termalt_i, \RTyPath'') \Preds[N_2]{\seq{\ell}'}{D'^{\Mark}} (\termalt', \RTyPath')
        \]
        for some \( 1 \le i \le n \) (here \( N_1 = i \) if \( i < n \) and \( n-1 \) if \( i = n \)).
        We have \( \runseq = q q_i \runseq' \) where \( q_i \runseq' = \Run_{\prog, \PWA}(q_i, \termalt_i, \RTyPath'', N_2) \) by definition.
        By the induction hypothesis, there exist \( \ITE_1' \) and \( \term' \) such that \( \ITE_1' \EnvRel \TopEnv \) and
        \[
        \ITE_1' \cup (\ITE_2 \RaiseP \Omega_{\PWA}(q_i) \RaiseP \SUMMARY(q_i \runseq')) \pInter \term' : q' \eESRel \termalt'.
        \]
        We have \( (\ITE_2 \RaiseP \Omega_{\PWA}(q_i) \RaiseP \SUMMARY(q_i \runseq')) = (\ITE_2 \RaiseP \SUMMARY(q q_i \runseq')) \) and \( \term \Pred{\lab}{D^{\Mark}} \term_0 \Preds{\seq{\ell}}{D^{\Mark}} \term' \) as desired.
        
  \item Case \(\termalt = \termalt_1 \nondet \termalt_2\):
        As with the previous case,
        the last rule used on the derivation is \rn{IT-NonDet}.
        Then we have
        \begin{align*}
         (\ITE_1 \cup \ITE_2) \pInter \term_{1} \COL q \eESRel \termalt_{1} \qquad
         (\ITE_1 \cup \ITE_2) \pInter \term_{2} \COL q \eESRel \termalt_{2} \qquad
         \term = \term_{1} \nondet \term_{2}
        \end{align*}
        Suppose \( \RTyPath = \PLeft \RTyPath'' \); the other case can be proved by a similar way.
        Then the reduction sequence
        \[
        (\termalt, \RTyPath) \Preds[N]{\seq{\ell}}{D'^\Mark} (\termalt', \RTyPath')
        \]
        must be of the form
        \[
        (\termalt, \RTyPath) \Preds[1]{\epsilon}{D'^{\Mark}} (\termalt_1, \RTyPath'') \Preds[N-1]{\seq{\ell}'}{D'^{\Mark}} (\termalt', \RTyPath').
        \]
        Then \( \runseq = \Run_{\prog, \PWA}(q, \termalt_1, \RTyPath'', N-1) \) by definition.
        Hence, by applying the induction hypothesis to \( \ITE_1 \cup \ITE_2 \pInter \term_{1} \COL q \eESRel \termalt_{1} \), we obtain the desired result.
  \item Case \(\termalt = \ifexp{p(\termalt_{1}, \dots, \termalt_{n})}{\termalt_{n+1}}{\termalt_{n+2}}\):
        As with the previous cases,
        the last rule used on the derivation is \rn{IT-If}.
        %
        %By rule \rn{IT-IF}, we have:
        Hence we have
        \begin{align*}
          &
          \term = \ifexp{p(\term_{1}, \dots, \term_{n})}{\term_{n+1}}{\term_{n+2}} \\&
          \forall i \in \{1,\dots, n\}.
          \ITE_1 \cup \ITE_2 \pInter \term_{i} \COL \Tint \eESRel \termalt_{i} \\&
          \ITE_1 \cup \ITE_2 \pInter \term_{n+1} \COL q \eESRel \termalt_{n+1} \qquad
          \ITE_1 \cup \ITE_2 \pInter \term_{n+2} \COL q \eESRel \termalt_{n+2}
        \end{align*}
        Recall that the result type of a function cannot be the integer type in our language.
        This implies that \( \term_i \) (\( 1 \le i \le n \)) consists only of constants and numerical operations, and thus \( \term_i = \termalt_i \) for every \( 1 \le i \le n \).

        Suppose that \((\sem{\termalt_{1}}, \dots, \sem{\termalt_{n}}) = (\sem{\term_1}, \dots, \sem{\term_n}) \in \sem{p}\).
        Then the reduction sequence
        \[
        (\termalt, \RTyPath) \Preds[N]{\seq{\ell}}{D'^\Mark} (\termalt', \RTyPath')
        \]
        must be of the form
        \[
        (\termalt, \RTyPath) \Preds[1]{\epsilon}{D'^{\Mark}} (\termalt_{n+1}, \RTyPath'') \Preds[N-1]{\seq{\ell}'}{D'^{\Mark}} (\termalt', \RTyPath')
        \]
        and \( \runseq = \Run_{\prog, \PWA}(q, \termalt_1, \RTyPath'', N-1) \) by definition.
        We obtain the desired result by applying the induction hypothesis to \( \ITE_1 \cup \ITE_2 \pInter \term_{n+1} \COL q \eESRel \termalt_{n+1} \); the corresponding reduction sequence is \( \term \Pred{\epsilon}{D^{\Mark}} \term_{n+1} \Preds{\seq{\ell}}{D^{\Mark}} \term' \).
        
        The case that \((\sem{\termalt_{1}}, \dots, \sem{\termalt_{n}}) \notin \sem{p}\) can be proved similarly.
        %% In this case, we have \(\ell = \epsilon\) and \(\termalt' = \termalt_{n+1}\).
        %% By the well-typedness of the program,
        %% for every \(i \in \{1,\dots,n\}\), \(\term_{i}\) consists of only integers and integer operations.
        %% Thus, we have \(\sem{\term_i} = \sem{\termalt_i}\) for each \(i \in \{1,\dots,n\}\) and
        %% \(\term \Pred{\epsilon}{D^\Mark} \term_{n+1}\).

        %% Let \(\runseq = q \in \RunSet(q, \ell)\).
        %% Then, \(\SUMMARY(\runseq) = 0\) holds.
        %% Thus, by using Lemma~\ref{appx:es:lem:weakening}, we have:
        %% \begin{align*}
        %%  \TopEnvZ \cup ((\ITE \cup \ITE') \RaiseP \SUMMARY(\runseq)) &\pInter \term' \COL q
        %%  \eESRel \termalt_{n+1}.
        %% \end{align*}
        %% Hence, the required result holds for \(\term' = \term_{n+1}\).

        %% In the case where
        %% \((\sem{\termalt_{1}}, \dots, \sem{\termalt_{n}}) \notin \sem{p}\),
        %% we obtain \(\runseq = q\) and \(\term' = \term_{n+2}\) in a similar way.
  \item Case \(\termalt = g\;\termalt_1\dots \termalt_n\) with \(g\in\dom(D')\):
        \newcommand\bdy{\mathit{body}}
        By the shape of \(\termalt\),
        the last rule used on the derivation is \rn{IT-App} or \rn{IT-AppInt}.
        By induction on the derivation,
        we have \(\term = f \term_1 \dots \term_k\) for some \(k\).
        Then
        \begin{align}
         g = f_{\Atype, m} \qquad
         \ITE_1 \cup \ITE_2 \pInter f \COL \Atype \eESRel f_{\Atype, m} \nonumber\\
         D(f) = \lambda x_1\dots x_k. \term_\bdy \qquad
         D'(f_{\Atype, m}) = \lambda y_1\dots y_n. \termalt_\bdy \nonumber\\
         \TopEnvZ \pInter \lambda x_1\dots x_k. \term_\bdy \COL \Atype
         \eESRel
         \lambda y_1\dots y_n. \termalt_\bdy. \label{appx:es:lem:sim2:app:0}
        \end{align}
        \begin{align}
         \Atype = \Itype_1 \to \dots \Itype_{k} \to q \qquad
         I &\subseteq \{1, \dots, k\} \qquad
         \bar{I} = \{1,\dots,k\}\setminus I \nonumber\\
         \forall i \in I. \Itype_i = \bigwedge_{1 \le j \le \ell_i} (\Atype'_{i,j}, m'_{i,j}) \qquad
         &\forall i \in \bar{I}. \Itype_i = \Tint \nonumber\\
         \forall i \in I. \forall j \in \{1, \dots, \ell_i\}.
         (\ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j}
         \eESRel u_{i, j}
         \label{appx:es:lem:sim2:1} \\
         \forall i \in \bar{I}.
         \ITE \cup \ITE' &\pInter \term_{i} \COL \Tint
         \eESRel u_{i, 1}
         \label{appx:es:lem:sim2:2} \\
         \forall i \in \{1,\dots,k\}. \seq{u_{i}} &=
         \begin{cases}
          u_{i,1} \dots u_{i,\ell_i} & (i \in I) \\
          u_{i,1} & (\text{otherwise})
         \end{cases} \nonumber\\
         \seq{u_1} \dots \seq{u_k} &= \termalt_1 \dots \termalt_n \nonumber\\
         \dup{x_1,\Itype_1} \dots \dup{x_k,\Itype_k} &= y_1\dots y_n\nonumber\\
        \end{align}
        Then the reduction sequence
        \[
        (\termalt, \RTyPath) \Preds[N]{\seq{\ell}}{D'^\Mark} (\termalt', \RTyPath')
        \]
        must be of the form
        \[
        (\termalt, \RTyPath) \Preds[1]{\epsilon}{D'^{\Mark}} ([\seq{u_1}/\dup{x_1, \Itype_1}]\dots [\seq{u_k}/\dup{x_k, \Itype_k}] \termalt_\bdy, \RTyPath'') \Preds[N-1]{\seq{\ell}'}{D'^{\Mark}} (\termalt', \RTyPath')
        \]
        and \( \runseq = \Run_{\prog, \PWA}(q, \termalt_1, \RTyPath'', N-1) \) by definition.

        By \eqref{appx:es:lem:sim2:app:0},
        we have
        \begin{align}
         \TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}
         &\pInter \term_{\bdy} \COL q
         \eESRel \termalt_{\bdy}
         \label{appx:es:lem:sim2:4}
        \end{align}

        By using Lemma~\ref{appx:es:lem:weakening} with
        \eqref{appx:es:lem:sim2:1}, \eqref{appx:es:lem:sim2:2} and \eqref{appx:es:lem:sim2:4},
        we have
        \begin{align}
         (\TopEnvZ \cup \ITE \cup \ITE') \RaiseP m'_{i,j} &\pInter \term_{i} \COL \Atype'_{i,j} \eESRel u_{i,j} \label{appx:es:lem:sim2:5} \\
         \forall i \in \bar{I}.
         (\TopEnvZ \cup \ITE \cup \ITE') &\pInter \term_{i} \COL \Tint \label{appx:es:lem:sim2:6} \eESRel u_{i,1} \\
         \TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k} &\pInter \term_{\bdy} \COL q
         \eESRel \termalt_{\bdy}
         \label{appx:es:lem:sim2:7}
        \end{align}
        By applying the induction hypothesis to this judgement, we complete the proof.
        %Since
        %\[
        %(\TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}) \RaiseP 0 =
        %\TopEnvZ \cup \ITE \cup \ITE' \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_k \COL \Itype_k}
        %\]
        By using Lemma~\ref{appx:es:lem:subst:inter} and Lemma~\ref{appx:es:lem:subst:integer} repeatedly
        with \eqref{appx:es:lem:sim2:5}, \eqref{appx:es:lem:sim2:6} and \eqref{appx:es:lem:sim2:7},
        we have
        \begin{align*}
         \TopEnvZ \cup \ITE \cup \ITE' &\pInter [\term_{1}/x_1] \dots [\term_{k}/x_k] \term_\bdy \COL q
         \eESRel [\seq{u_1}/\dup{x_1, \Itype_1}]\dots [\seq{u_k}/\dup{x_k, \Itype_k}] \termalt_{\bdy}.
        \end{align*}
        By applying the induction hypothesis to this judgement, we complete the proof; the corresponding reduction sequence is \( \term \Pred{\epsilon}{D^\Mark}  [\term_{1}/x_1] \dots [\term_{k}/x_k] \term_\bdy \Preds{\seq{\ell}}{D^{\Mark}} \term' \) where \( \term' \) is the term obtained by the induction hypothesis.
 \end{itemize}
\end{proof}



% \begin{lemma}\label{cor:liveness:eff-sel-ev-seq-vs-choice-seq2}
%  \wtnb{obsoleted}
%  Suppose \(\TopEnv \pInter P \Rightarrow (P', \Pfun)\),
%  \(\seq{\ell} \in \InfTraces(P')\) and
%  \(\runseq\) be a run of \(\PWA\) over \(\seq{\ell}\).
%  There exists a choice sequence \(\RTyPath\) such that
%  \(\EvSeq_{P, \PWA}(\RTyPath) = \seq{\ell}\) and
%  \(\Run_{P, \PWA}(\RTyPath) = \runseq\).
% \end{lemma}
% \begin{proof}
%  Let \(P = (D, \mainfun)\) and \(P' = (D', \mainfun')\).
%  By the definition of \(\InfTraces(P')\), we have \(\RTyPath_0\) such that
%  \[
%   \RTyPath_0 \Vdash \mainfun' \Pred{\ell_1}{D'} \termalt_1 \Pred{\ell_2}{D'} \termalt_2 \Pred{\ell_3}{D'} \dots \qquad
%   \seq{\ell} = \ell_1 \ell_2 \ell_3 \dots.
%  \]
%  By using Lemma~\ref{appx:es:lem:sim2} iteratively,
%  we have
%  \[
%   \RTyPath_1 \Vdash \mainfun \Pred{\ell_1}{D} \term_1 \Pred{\ell_2}{D} \term_2 \Pred{\ell_3}{D} \dots \qquad
%  \forall i \in \omega.\; \exists \ITE_i \EnvRel \TopEnv.\; \ITE_i \pInter \term_i \COL \runseq(|\ell_1 \dots \ell_i|) \ESRel \termalt_i.
%  \]
%  Hence, the required result holds for \(\RTyPath = \RTyPath_1\).
 %  \wtnb{to do: Why \(\Run_{P, \PWA}(\RTyPath_1) = \runseq\).}
% \end{proof}

\begin{lemma}\label{lem:liveness:eff-sel-red-sim-multi-sim1}
 Suppose \(\TopEnv \pInter (D, \term_0) \eESRel ((D', \termalt_0), \Omega_0)\).
 Given
 \[
 \RTyPath \Vdash \term_0 \Pred{\ell_1}{D} \term_1 \Pred{\ell_2}{D} \term_2 \Pred{\ell_3}{D} \dots.
 \]
 Suppose \(\runseq\) be a run of \(\PWA\) over \(\ell_1 \ell_2 \dots\).
 Then, there exists an infinite reduction sequence
 \[
 \RTyPath' \Vdash \termalt_0 \Preds{\ell_1}{D'} \termalt_1 \Preds{\ell_2}{D'} \termalt_2 \Preds{\ell_3}{D'} \dots
 \]
 such that \(\Run_{D', \PWA}(\termalt_0, \qinit, \RTyPath_1, \omega) = \runseq\).
\end{lemma}
\begin{proof}
 We construct an infinite sequence \(\{\termalt_i\}_{i \in \omega}\) by induction on \(i\).

 For the base case, let \(\ITE_0 = \TopEnv, a_i = 0, n_i = 0\).
 Then, the followings hold:
 \begin{align*}
  \ITE_0 \pInter \term_0 \COL \runseq(a_0) \eESRel \termalt_0 \qquad
  \runseq(a_0) = \Run_{D', \PWA}(\termalt_0, \runseq(0), \RTyPath_{0}, n_0).
 \end{align*}

 For the induction step, suppose
 \begin{align*}
  \RTyPath_i \Vdash \termalt_0 \Preds[n_i]{\ell_1 \dots \ell_i}{D'} \termalt_i \qquad
  \ITE_i \pInter \term_i \COL \runseq(a_i) \eESRel \termalt_i \qquad
  \runseq(a_0)\dots\runseq(a_i) = \Run_{D', \PWA}(\termalt_i, \runseq(0), \RTyPath_{i}, n_i).
 \end{align*}
 By using Lemma~\ref{appx:es:lem:sim1}, we have \(\RTyPath'_{i+1}, \termalt_{i+1}, \ITE_{i+1}, a_{i+1}\) and \(m_{i+1}\) such that
 \begin{align*}
  \RTyPath'_{i+1} \Vdash \termalt_{i} \Preds[m_{i+1}]{\ell_{i+1}}{D'} \termalt_{i+1} \qquad
  \ITE_{i+1} \pInter \term_{i+1} \COL \runseq(a_{i+1}) \eESRel \termalt_{i+1} \\
  \runseq(a_i)\dots\runseq(a_{i+1}) = \Run_{D', \PWA}(\termalt_i, \runseq(a_i), \RTyPath'_{i+1}, m_i).
 \end{align*}
 Let \(n_{i+1} = n_i + m_{i+1}\).
 Then there exists \(\RTyPath_{i+1}\) such that
 \[
  \RTyPath_{i+1} \Vdash \termalt_0  \Preds[n_{i+1}]{\ell_1 \dots \ell_{i+1}}{D'} \termalt_{i+1} \qquad
  \runseq(a_0)\dots\runseq(a_{i+1}) = \Run_{D', \PWA}(\termalt_0, \runseq(0), \RTyPath_{i+1}, n_{i+1}).
 \]
 These conditions are the assumption for the next step.

 Hence, we obtain the following as required:
 \[
  \RTyPath_{\omega} \Vdash \termalt_0  \Preds[n_{1}]{\ell_{1}}{D'} \termalt_1 \Preds[n_{2}]{\ell_{2}}{D'} \termalt_2 \Preds[n_{3}]{\ell_{3}}{D'} \dots \qquad
 \runseq(0) \runseq(1) \dots = \Run_{D', \PWA}(\termalt_0, \runseq(0), \RTyPath_\omega, \omega).
 \]
\end{proof}

\begin{lemma}\label{lem:liveness:eff-sel-red-sim-multi-sim2}
 Suppose \(\TopEnv \pInter (D, \term_0) \eESRel ((D', \termalt_0), \Omega_0)\).
 Given
 \[
  \termalt_0 \Pred{\ell_1}{D'} \termalt_1 \Pred{\ell_2}{D'} \termalt_2 \Pred{\ell_3}{D'} \dots.
 \]
 Then, there exists an infinite reduction sequence
 \[
  \term_0 \Preds{\seq{\ell'_1}}{D} \term_1 \Preds{\seq{\ell'_2}}{D} \term_2 \Preds{\seq{\ell'_3}}{D} \dots
 \]
 such that \(\ell_1\ell_2 \dots = \seq{\ell'_1}\seq{\ell'_2} \dots\).
\end{lemma}
\begin{proof}
 We have \(\{n_i\}_{i \in \omega}\) and \(\RTyPath_0, 0 = j_0 < j_1 < \dots\) such that each \(\termalt_{j_i}\) is not of the form \( \termalt' \enondet \termalt'' \) and
 \[
  \termalt_{j_0} \Preds[n_1]{\ell_{j_0+1} \dots \ell_{j_1}}{D'} \termalt_{j_1} \Preds[n_2]{\ell_{j_1+1} \dots \ell_{j_2}}{D'} \termalt_{j_2} \Preds[n_3]{\ell_{j_2+1} \dots \ell_{j_3}}{D'} \dots.
 \]

 We construct an infinite sequence \(\{\term_i\}_{i \in \omega}\) by induction on \(i\).

 For the base case, let \(\ITE_0 = \TopEnv, q_0 = \qinit\).
 Then, \(\ITE_0 \pInter \term_0 \COL q_0 \eESRel \termalt_{j_0}\).

 For the induction step, let \(i \in \omega\).
 Suppose \(\ITE_i \pInter \term_{i} \COL q_i \eESRel \termalt_{j_i}\).
 By Lemma~\ref{appx:es:lem:summary}, we have \(\ITE_{i+1}\) and \(\term_{i+1}\) such that
 \[
  \ITE_{i+1} \pInter \term_{i+1} \COL q_{i+1} \eESRel \termalt_{j_{i+1}} \qquad
  \seq{\ell'_{i+1}} = \ell_{j_i + 1} \dots \ell_{j_{i+1}} \qquad
  \term_i \Preds{\seq{\ell'_{i+1}}}{D} \term_{i+1}.
 \]
 Hence, we obtain the required reduction sequence
 \[
  \term_0 \Preds{\seq{\ell'_{1}}}{D} \term_1 \Preds{\seq{\ell'_{2}}}{D} \dots.
 \]
\end{proof}

\begin{corollary}\label{cor:liveness:eff-sel-ev-seq-vs-choice-seq}
 Suppose \(\TopEnv \pInter P \eESRel (P', \Omega_0)\). Then,
 \begin{align*}
  &\forall \seq{\ell} \in \InfTraces(\prog).\;
  \forall \runseq \in \RunSet(q, \seq{\ell}).\;
  \MAX\mathbf{Inf}(\Omega(\runseq)) \text{ is \emph{odd}.} \\
  \IFF
  &\forall \RTyPath \in \{\PLeft, \PRight\}^{\omega}.\;
  \MAX\mathbf{Inf}(\Omega(\Run_{P',\PWA}(\RTyPath))) \text{ is \emph{odd}.}
 \end{align*}
\end{corollary}
\begin{proof}
 Let \(P = (D, \term_0)\) and \(P' = (D', \termalt_0)\).

 \((\Rightarrow)\)
 Let \(\RTyPath \in \{\PLeft, \PRight\}\).
 Suppose
 \(
 \RTyPath \VDash \termalt_0 \Pred{\ell_1}{D'} \termalt_1 \Pred{\ell_2}{D'} \termalt_2 \Pred{\ell_3}{D'} \dots
 \).
 By Lemma~\ref{lem:liveness:eff-sel-red-sim-multi-sim2}, \(\ell_1 \ell_2 \dots \in \InfTraces(\prog)\) holds.
 In addition, by Corollary~\ref{cor:liveness:eff-sel-induced-run}, \(\Run_{P', \PWA}(\RTyPath) \in \RunSet(q, \ell_1 \ell_2 \dots)\).
 Hence, \( \MAX\mathbf{Inf}(\Omega(\Run_{P',\PWA}(\RTyPath)))\) is odd.

 \((\Leftarrow)\)
 The result follows immediately from Lemma~\ref{lem:liveness:eff-sel-red-sim-multi-sim1}.
\end{proof}

\subsubsection{Analysis of the result of the translation}
\label{sec:appx:liveness:analysis-of-result}
%% By the translation, an intersection type \( \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \) is transformed into the product type \( \prod_{1 \le i \le k} (\Atype_i, m_i) \).
%% Formally the translation on types is defined by:
%% \begin{align*}
%%   \EffTypeTrans{q} &:= q \\
%%   \EffTypeTrans{(\INT \to \Atype)} &:= \INT \to (\EffTypeTrans{\Atype}) \\
%%   \EffTypeTrans{\left(\bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype_0\right)} &:= (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to \EffTypeTrans{\Atype_0}.
%% \end{align*}
%% For an intersection type environment \(\ITE\), we define \( \EffTypeTrans{\ITE} := \{ x_{\Atype,m} : (\Atype,m, m') \mid x : (\Atype,m, m') \in \ITE \} \).
%% Similarly, for a top-level type environment \( \TopEnv \), we define \( \EffTypeTrans{\TopEnv} := \{ x_{\Atype,m} : (\Atype,m) \mid x : (\Atype,m) \in \TopEnv \} \).

%% We say that a top-level environment \( \TopEnv \) is \emph{simple} if, for every \( x \), there exists at most one binding \( x : (\Atype, m) \in \TopEnv \).
%% Given a simple top-level environment \( \TopEnv \), if \( x : (\Atype, m) \in \TopEnv \), then we write \( \Pfun_{\TopEnv}(x) = m \).
%% Since \( \TopEnv \) is simple, \( \Pfun_{\TopEnv} \) is a partial mapping.

%% Below, we write
%% \(\ITE \pInter \term \COL \Atype \) if
%% \(\ITE \pInter \term \COL \Atype \eESRel \termalt\) for some \(\termalt\).
%% %\nk{Has this been mentioned elsewhere?}

%% \begin{lemma}\label{lem:appx:liveness:translation-typable:pre}
%%  If \(\ITE \pInter \term \COL \Atype \eESRel \termalt\),
%%  then \(\EffTypeTrans{\ITE} \pInter \termalt \COL \EffTypeTrans{\Atype}\).
%% \end{lemma}
%% \begin{proof}
%%  The proof proceeds by induction on the derivation of \(\ITE \pInter \term \COL \Atype \eESRel \termalt\),
%%  with case analysis on the last rule used.
%%  We prove only interesting cases.
%%  \begin{itemize}
%%   \item Case for \rn{IT-App}:
%%     %%        Let \(\term = \term_1 \term_2\).
%%     By \rn{IT-App}, we have:
%%         \begin{align*}
%%           &   \term=\term_1\term_2 \qquad
%%                    \termalt = \term'_1 \term'_{2,1} \dots \term'_{2,k}\\
%%       &   \ITE \pInter \term_1 \COL \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype \eESRel \term'_1 \qquad
%%          \forall i \in \{1,\dots, k\}.\;\ITE \RaiseP m_i \pInter \term_2 \COL \Atype_i \eESRel \term'_{2,i} \qquad
%%         \end{align*}
%%         By the induction hypothesis, we have
%%         \begin{align*}
%%          \EffTypeTrans{\ITE} \pInter \term'_1 \COL (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to (\EffTypeTrans{\Atype}) \qquad
%%          \forall i \in \{1,\dots, k\}.\;\EffTypeTrans{(\ITE \RaiseP m_i)} &\pInter \term'_{2,i} \COL \EffTypeTrans{\Atype_i}.
%%         \end{align*}
%%         Since
%%         \(\EffTypeTrans{(\ITE \RaiseP m_i)} = (\EffTypeTrans{\ITE}) \RaiseP m_i\),
%%         by using \rn{IT-App} \(k\) times,
%%         we obtain \(\EffTypeTrans{\ITE} \pInter \term'_1 \term'_{2,1}\dots \term'_{2,k} \COL \EffTypeTrans{\Atype}\) as required.
%%   \item Case for \rn{IT-Abs}:
%%         By \rn{IT-Abs}, we have:
%%         \begin{align*}
%%       &  \term = \lambda x. \term' \qquad \termalt = \lambda x_{\Atype_1,m_1}\dots x_{\Atype_k,m_k}.\;\termalt'\qquad
%%         \Atype = \bigwedge_{1 \le i \le k} (\Atype_i,m_i)\to \Atype'\\
%%        &  \ITE, x \COL (\Atype_1, m_1, 0), \dots, x \COL (\Atype_k, m_k, 0)
%%          \pInter \term' \COL \Atype' \eESRel \termalt' \qquad
%%          x \notin dom(\ITE)
%%         \end{align*}
%%         By the induction hypothesis, we have
%%         \begin{align*}
%%          \EffTypeTrans{\ITE} \cup \{x_{\Atype_1, m_1} \COL (\Atype_1, m_1, 0), \dots, x_{\Atype_k, m_k} \COL (\Atype_k, m_k, 0) \} \pInter \termalt' \COL \EffTypeTrans{\Atype'}.
%%         \end{align*}
%%         In addition, \(x_{\Atype_i, m_i} \notin dom(\EffTypeTrans{\ITE})\) for each \(i\),
%%          since \(x \notin dom(\ITE)\).
%%         Thus, by using \rn{IT-Abs} \(k\) times, we obtain the following as required:
%%         \[
%%         \EffTypeTrans{\ITE} \pInter \lambda x_{\Atype_1,m_1}\dots x_{\Atype_k,m_k}.\;\termalt'
%%         \COL (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to \EffTypeTrans{\Atype'}.
%%         \]
%%  \end{itemize}
%% \end{proof}

%% \begin{lemma}\label{lem:appx:liveness:translation-typable}
%%   If \( \TopEnv \pInter P \Rightarrow (P', \Pfun) \), then \( \EffTypeTrans{\TopEnv} \pInter P' \).
%%   Furthermore \( \EffTypeTrans{\TopEnv} \) is simple and \( \Pfun = \Pfun_{\EffTypeTrans{\TopEnv}} \).
%% \end{lemma}
%% \begin{proof}
%%  The former condition follows immediately from Lemma~\ref{lem:appx:liveness:translation-typable:pre}. %\tk{to do}\wtnb{done}
%%  The latter condition follows immediately from the definition of
%%  \( \TopEnv \pInter P \Rightarrow (P', \Pfun) \).
%% \end{proof}


\begin{lemma}
 \label{appx:es:lem:mark-type}
 If \( \TopEnv \pInter D \eESRel D' \) and \(\ITE \cup \ITE' \pInter s \COL q \eESRel \term \) with \( \Funcs(D) \cap \dom(\ITE') = \emptyset \),
 then \(\ITE \cup \ITE^\Mark \cup \ITE' \pInter s^{\Mark} \COL q \eESRel \term^\Mark \).
\end{lemma}
\begin{proof}
 By straightforward induction.
\end{proof}

\begin{lemma}
 \label{appx:es:lem:callseq-summary-one}
 Assume that
 \begin{align*}
  \TopEnv \pInter D \eESRel D' \qquad
  &\ITE_0 \EnvRel \TopEnv \qquad
  \ITE_0 \pInter f\,t_1\,\dots\,t_n : q \eESRel g\,\seq{s}_1\,\dots\,\seq{s}_n \qquad
%  (g\,\seq{s}; \RTyPath_0\RTyPath_1)  \mathrel{\stackrel{\seq{\ell}}{\red}\!\!{}_{\progd}^{N}} (h\,\seq{u}; \RTyPath_1) \qquad
  &\RTyPath \Vdash g\,\seq{s}_1\,\dots\,\seq{s}_n \CallSeqN{N}_{D'} h_{\Atype,m}\,\seq{u}_1\,\dots\,\seq{u}_{n'}.
 \end{align*}
 Then \( m=\SUMMARY(\Run_{D', \PWA}(q, g\,\seq{s}, \RTyPath, N)) \).
\end{lemma}
\begin{proof}
 %% Let \(n = |\seq{\termalt}|\).
 Since \(\ITE_0 \pInter f\;\seq{s} \COL q \eESRel g\,\seq{s} \),
 there exist \( \Atype_0 \) and \( m_0 \) such that
 \begin{align}
   & f \COL (\Atype_0, m_0, m_0) \in \ITE_0 \nonumber\\
   & \Atype_0 = \Itype_1 \to \dots \to \Itype_n \to q \nonumber\\
   & \forall i \in \{ 1,\dots,n \}.\; \ITE_0 \pInter t_i \COL \Itype_i \eESRel \seq{s}_i
   \label{eq:appx:lem:summary2}
 \end{align}
 where \( \ITE_0 \pInter t_i \COL \bigwedge_{1 \le j \le k} (\Atype'_{j}, m_j) \eESRel s_{i,1}\,\dots\,s_{i,k} \) means \( \forall j \in \{1,\dots\,k\}.\, \ITE_0 \RaiseP m_j \pInter t_i \COL \Atype'_j \eESRel s_{i,j} \).

 Suppose \( D(f) = \lambda x_1 \dots x_n. t_0 \).
 Since \( \TopEnv \pInter D \eESRel D' \), %\rn{IT-Abs} and \rn{IT-AbsInt},
 we have
 \begin{align*}
   & D'(f) = \lambda \seq{x}_1 \dots \seq{x}_n. s_0
   &\TopEnvZ \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
   &\pInter t_0 \COL q \eESRel s_0.
 \end{align*}
 By Lemma~\ref{appx:es:lem:mark-type}, we have
 \begin{align}
  \TopEnvZ \cup \TopEnvZM \cup \ZEnv{x_1 \COL \Itype_1} \cup \dots \cup \ZEnv{x_n \COL \Itype_n}
  &\pInter \term^\Mark \COL q. \label{eq:appx:lem:summary:lambda}
 \end{align}

 By using Weakening (Lemma~\ref{appx:es:lem:weakening}) and Substitution Lemmas (Lemmas~\ref{appx:es:lem:subst:integer} and \ref{appx:es:lem:subst:inter}), from \eqref{eq:appx:lem:summary2} and \eqref{eq:appx:lem:summary:lambda},
 we have
 \begin{align}
  \TopEnvZ \cup \TopEnvZM \cup \ITE_0
  &\pInter [\termalt_1/x_1]\dots[\termalt_n/x_n] \term_0^\Mark \COL q \eESRel [\seq{s}_1/\seq{x}_1]\dots[\seq{s}_s/\seq{x}_n]s_0^\Mark. \label{eq:appx:lem:summary4:1}
 \end{align}

 Now, by the definition of call sequence, we have
 \begin{align}
  \RTyPath \Vdash [\termalt_1/x_1]\dots[\termalt_n/x_n] s_0^\Mark \Predk{\seq{\ell}}{N-1}{D'^\Mark} h_{\Atype,m}^\Mark\;\seq{u'}. \label{eq:appx:lem:summary4:2}
 \end{align}

 %% In addition, we have
 %% \begin{align}
 %%  \runseqPZ \in \RunSet(q, \seq{\ell}). \label{eq:appx:lem:summary4:3}
 %% \end{align}

 Let \( \runseq = \Run_{D', \PWA}(q, g\,\seq{s}, \RTyPath, N) \).
 By Lemma~\ref{appx:es:lem:summary}, there exists \( \term' \) and \( \ITE' \) such that
 \[
 \ITE' \cup (\TopEnvZM \RaiseP \SUMMARY(\runseq)) \pInter \term' : q' \eESRel h_{\Atype,m}^\Mark\;\seq{u'}
 \]
 where \( q' \) is the last state in \( \runseq \).
 Hence \( h : (\Atype, m, m) \in (\TopEnvZM \RaiseP \SUMMARY(\runseq)) \) and thus \( m = \SUMMARY(\runseq) \) by definition of \( \TopEnvZM \).
\end{proof}

\begin{corollary}\label{cor:liveness:summarising-priority}
  Assume that \( \TopEnv \pInter P \eESRel (P', \Pfun) \).
  Let \( P = (\mainfun, D) \) and \( P' = (\mainfun', D') \).
  For each choice sequence \( \RTyPath \in \{\PLeft,\PRight\}^{\omega} \), the following conditions are equivalent.
  \begin{enumerate}
  \item \( \MAX\mathbf{Inf}(\Omega_{\PWA}(\Run_{D',\PWA}(\qinit, \mainfun', \RTyPath, \omega))) \text{ is \emph{odd}} \).
  \item \( \forall \seq{g} \in \InfCallseq(\prog', \RTyPath).\; \MAX \mathbf{Inf}(\Omega(\seq{g})) \text{ is \emph{even}} \).
  \end{enumerate}
\end{corollary}
\begin{proof}
  (\( (1) \Rightarrow (2) \))
  Assume that \( \MAX\mathbf{Inf}(\Omega_{\PWA}(\Run_{D',\PWA}(\qinit, \mainfun', \RTyPath, \omega))) \text{ is \emph{odd}} \).
  By Corollary~\ref{cor:liveness:unique-existence-of-call-seq}, we have a (unique) infinite call-sequence
  \[
  (\mainfun', \RTyPath) = (g^0_{\Atype_0,m_0}\,\tilde{u}_0, \RTyPath_0) \CallSeqN{k_0}_{D'} (g^1_{\Atype_1,m_1}\,\tilde{u}_1, \RTyPath_1) \CallSeq{k_1}_{D'} (g^2_{\Atype_2, m_2}\,\tilde{u}_2, \RTyPath_2) \CallSeq{k_2}_{D'} \cdots.
  \]
  Let \( R_i = \Run_{D',\PWA}(q_i, g^i_{\Atype_i,m_i}\,\tilde{u}_i, \RTyPath_i, k_i) \) where \( q_0 = \qinit \) and \( q_i \) is the last state of \( R_{i-1} \) (\( i > 0 \)).
  By Lemma~\ref{appx:es:lem:callseq-summary-one}, \( m_i = \SUMMARY(R_i) \).
  Since \( R = \Run_{D',\PWA}(\qinit, \mainfun', \RTyPath, \omega) \) is the ``limit'' of \( R_0 \RunConcat R_1 \RunConcat \dots \RunConcat R_N \) (\( N \to \infty \)), we have
  \[
  \MAX\mathbf{Inf}(\Omega_{\PWA}(\Run_{D',\PWA}(\qinit, \mainfun', \RTyPath, \omega))) = \MAX\mathbf{Inf} \{ m_i \mid i = 0, 1, \dots \}.
  \]
  Since \( \Pfun(g^i_{\Atype_i,m_i}) = m_i + 1 \), we obtain the claim.

  (\( (2) \Rightarrow (1) \))
  By Lemma~\ref{appx:es:lem:callseq-summary-one}, \( \InfCallseq(\prog', \RTyPath) \) is not empty.
  Let \( \mainfun_{\qinit} g^1_{\Atype_1,m_1} g^2_{\Atype_2,m_2} \dots \) be an element of \( \InfCallseq(\prog', \RTyPath) \), i.e.,
  \[
  (\mainfun', \RTyPath) = (g^0_{\Atype_0,m_0}\,\tilde{u}_0, \RTyPath_0) \CallSeqN{k_0}_{D'} (g^1_{\Atype_1,m_1}\,\tilde{u}_1, \RTyPath_1) \CallSeq{k_1}_{D'} (g^2_{\Atype_2, m_2}\,\tilde{u}_2, \RTyPath_2) \CallSeq{k_2}_{D'} \cdots.
  \]
  By an argument similar to the above case, we have
  \[
  \MAX\mathbf{Inf}(\Omega_{\PWA}(\Run_{D',\PWA}(\qinit, \mainfun', \RTyPath, \omega))) = \MAX\mathbf{Inf} \{ m_i \mid i = 0, 1, \dots \},
  \]
  which implies the claim.
  
 %% By the definition of call-sequence,
 %% we have
 %% \begin{align*}
 %%  \RTyPath \Vdash \mainfun \Preds{\seq{\ell}_1}{D} g_1\,\seq{u}_1 \Preds{\seq{\ell}_2}{D} g_2\,\seq{u}_2 \Preds{\seq{\ell}_3}{D} \cdots.
 %% \end{align*}
 %% Now, we write \(a_i\) for \((|\seq{\ell}_1| + \dots + |\seq{\ell}_i|)\).
 %% By using Lemma~\ref{appx:es:lem:sim1} iteratively,
 %% for each \(i\), we have \(\ITE_i\) such that
 %% \begin{align*}
 %%  \ITE_i \pInter g_i\,\seq{u}_i \COL \runseqP(a_i)
 %%  \quad\mbox{and}\quad
 %%  \ITE_i \EnvRel \TopEnv.
 %% \end{align*}
 %% Hence by Lemma~\ref{appx:es:lem:callseq-summary-one},
 %% \begin{align*}
 %%  \Pfun_{\TopEnv}(g_i)
 %%  & = \SUMMARY(\runseqP(a_i)\dots\runseqP(a_{i+1})) + 1 \\
 %%  & = \MAX\{0, \Pfun(\runseqP(a_i + 1)), \dots , \Pfun(\runseqP(a_{i+1}))\} + 1
 %% \end{align*}
 %% for each \(i \ge 1\).
 %% In addition, \(0 \le a_1 \le a_2 \le \dots \) and \( \lim_{i \to \infty} a_i = \infty \) hold
 %% since the generated event sequence is infinite by the assumption.
 %% Therefore, we obtain the required result.
\end{proof}

\subsubsection{Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}}
%We are now ready to prove Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}.
%\begin{proof}
Assume that \( \TopEnv \pInter \prog \ESRel (\prog_0, \Pfun) \).
Then by Lemma~\ref{lem:appx:liveness:relating-modified-and-original-translations}, there exists \( \prog_1 \) such that \( \TopEnv \pInter \prog \eESRel (\prog_1, \Pfun) \) and \( \prog_0 = [\nondet/\enondet]\prog_1 \).
Obviously \( \models_\CSA (\prog_1, \Pfun) \) if and only if \( \models_\CSA (\prog_0, \Pfun) \).
 %% Suppose that \(\TopEnv \pInter \prog \ESRel (\prog_0, \Pfun_0)\),
 %% \(\TopEnv \pInter \prog \eESRel (\prog_1, \Pfun_1)\) and \(\prog_1 = (\progd, \mainfun)\).
 %% Then, we obtain the required result as follows.
 \[
 \begin{array}{l}
   \InfTraces(\prog) \cap \Lang(\PWA) = \emptyset \\
     \hfill \mbox{(by definition)}\\
  \IFF
  \forall \seq{\ell} \in \InfTraces(\prog). \forall \runseq \COL \text{run of \(\PWA\) over \(\seq{\ell}\)}.\;
  \MAX\mathbf{Inf}(\Omega_{\PWA}(\runseq)) \text{ is \emph{odd}.} \hspace{5em}\\
    \hfill \mbox{(by Corollary~\ref{cor:liveness:eff-sel-ev-seq-vs-choice-seq})}\\
  \IFF
  \forall \RTyPath \in \{\PLeft, \PRight\}^{\omega}.\;
  \MAX\mathbf{Inf}(\Omega(\Run_{D,\PWA}(\RTyPath))) \text{ is \emph{odd}.} \\
    \hfill \mbox{(by Corollaries~\ref{cor:liveness:summarising-priority} and \ref{cor:liveness:unique-existence-of-call-seq})} \\
  \IFF
  \forall \RTyPath \in \{\PLeft, \PRight\}^{\omega}. \forall \seq{g} \in \InfCallseq(\prog, \RTyPath).\;
    \MAX \mathbf{Inf}(\Omega(\seq{g})) \text{ is \emph{even}.} \\
  %% \forall \RTyPath \in \{\PLeft, \PRight\}^{\omega}.\\
  %% \qquad \text{If } \RTyPath \Vdash \mainfun \CallSeq_{\progd} g_1\,\seq{u}_1 \CallSeq_{\progd} g_2\,\seq{u}_2 \CallSeq_{\progd} \dots \text{, then }
  %% \MAX \mathbf{Inf}(\Omega_1(g_1) \Omega_1(g_2) \dots) \text{ is \emph{even}.} \\
    \hfill \mbox{(by definition)}\\
  \IFF
  \models_\CSA (\prog_1, \Pfun_1) \\
  \IFF
  \models_\CSA (\prog_0, \Pfun_0)
  %\hfill \mbox{(by Lemma~\ref{lem:liveness:equivalence-of-two-csa})}
 \end{array}
 \]
%\end{proof}


==> appx-liveness-effectiveness.tex <==
\subsection{Proof (Sketch) of Theorem~\ref{thm:liveness:eff-sel-effective}}
\label{sec:proof-effectiveness}
This follows by 
 essentially the same argument as the proof of completeness of
the intersection type system for trivial model checking of HORS (\cite{Kobayashi13JACM},
Theorem 4.6); thus, we provide only a proof sketch.

First, we restrict intersection types by the following refinement relation.

\begin{definition}
The \emph{refinement relation} \(\Atype\DCOL \Pst\) between intersection types and simple types
is defined by:
\infrule{}{q\DCOL \Tunit}
\infrule{\Itype\DCOL\Pest \andalso \Atype\DCOL\Pst}{(\Itype\to\Atype)\DCOL (\Pest\to\Pst)}
\infrule{}{\INT\DCOL \Tint}
\infrule{\Atype_i\DCOL\Pst\mbox{ for each \(i\in\set{1,\ldots,k}\)}}
{\bigwedge_{1\le i\le k}(\Atype_i,m_i)\DCOL \Pst}
The relation is extended to the one on type environments by:
\(\TopEnv\DCOL \STE\) iff \(\Atype\DCOL \STE(x)\) for each \(x\COL (\Atype,m)\in \TopEnv\),
and 
\(\ITE\DCOL \STE\) iff \(\Atype\DCOL \STE(x)\) for each \(x\COL (\Atype,m,m')\in \ITE\).
\end{definition}

Let \(\prog=(\progd,t)\) be a program such that \(\STE\p \prog\). Here, we assume without loss of generality
that \(t\) is a function symbol \(f_1\). 
Let \(\TopEnvMax = \set{f\COL (\Atype,m) \mid f\COL\Pst\in \STE, \Atype\DCOL\Pst}\),
i.e., the largest type environment that refines \(\STE\). 
We define the function \(\StepFun\) on top type environments by:
\[ \StepFun(\TopEnv) = \set{f\COL(\Atype,m)\in \TopEnv \mid \TopEnv \pInter \progd(f)\COL \Atype\ESRel \term'}.\]
As in \cite{Kobayashi13JACM}, \(\StepFun\) just filters out invalid type assumptions.
%%Since \(\TopEnvMax\) is a finite set and \(\StepFun\) is monotonic,
%%there exists \(n\) such that \(\TopEnv^{(n)} = \StepFun^n(\TopEnvMax)\) is a
%%fixpoint of \(\StepFun\).
To show Theorem~\ref{thm:liveness:eff-sel-effective},
it is sufficient to prove the existence of a fixpoint \(\TopEnv\) of
\(\StepFun\) such that \(f_1\COL \qinit\in \TopEnv\)
(which serves as a witness of Theorem~\ref{thm:liveness:eff-sel-effective}).

To this end, we prepare a restriction of Theorem~\ref{thm:liveness:eff-sel-effective} for recursion-free programs:
\begin{lemma}
\label{thm:liveness:eff-sel-effective-for-recfree}
Let \(\prog=(\progd,f)\) be a recursion-free program such that \(\STE\p \prog\),
and \(\PWA\) be a non-deterministic parity automaton.
Then, there exists \(\TopEnv\), \( P' \) and \(\Pfun\)
such that \( \TopEnv \pInter P \Rightarrow (P',\Pfun) \).
\end{lemma}
\begin{myproof}[Sketch]
Consider a non-standard reduction relation \(\term\nsred{\progd}\term'\), 
where conditionals, non-deterministic branches, and events
are just considered tree constructors. Thus, the reduction rule just consists of:
 \infrule[R-Fun]{
 f \seq{x} = \termalt \in \progd \andalso
 |\seq{x}|=|\seq{\term}|
 } {
 \EC[f\;\seq{\term}] \nsred{\progd} \EC[[\seq{\term}/\seq{x}]\termalt]
 }
where \(\EC\) ranges over the set of evaluation contexts defined by:
\[
\begin{array}{l}
\EC ::= \Hole \mid \EC\nondet \term \mid \term\nondet \EC \mid \evexp{\lab}\EC\\\qquad
\mid \ifexp{p(\term'_1,\dots,\term'_k)}{\EC}{\term}
\mid \ifexp{p(\term'_1,\dots,\term'_k)}{\term}{\EC}.
\end{array}
\]
Since \(\prog\) is recursion-free and simply-typed, 
there must be a non-standard reduction sequence \(f\nsreds{\progd}\term\not{\nsred{\progd}}\).
Since the term \(\term\) does not contain any function symbol, we have \(\emptyset\pInter (\progd,\term)\Rightarrow
(\prog'', \emptyset)\). 
%%(here, recall that 
%%in Definition~\ref{def:pwa}, we required that the transition function is total; so, transformation derivations
%%cannot fail at \rn{IT-Event}).
 By the subject expansion property (i.e., the preservation of
the transformation relation by the inverse of reductions, which we omit to prove, as it is standard),
we have \( \TopEnv \pInter P \Rightarrow (P',\Pfun) \) for some \(\TopEnv\) such that \(\TopEnv\DCOL \STE\),
as required.
\end{myproof}

Now, let \(\prog^{(n)}\) be the recursion-free program
defined in the proof of Theorem~\ref{th:mayreach}, where \(n=|\TopEnvMax|+1\).
%%is a number such that
%%\(\TopEnv^{(n)} = \StepFun^n(\TopEnvMax)\) is a least fixpoint of \(\StepFun\) as discussed above.
Let \(\TopEnv'\) be the witness type environment \(\TopEnv\) for \(\prog^{(n)}\) given in 
Lemma~\ref{thm:liveness:eff-sel-effective-for-recfree}. 
Define \(\TopEnv_0,\ldots,\TopEnv_n\) by:
\(\TopEnv_k = \set{f\COL(\Atype,m)\mid f^{(j)}\COL(\Atype,m)\in \TopEnv', j\geq k}\).
Then, we have (i) \(\TopEnv_{k+1}\subseteq \StepFun(\TopEnv_k)\subseteq \TopEnv_k\)
for each \(k<n\)
(the first equality follows from the fact that
the body of \(f^{(k+1)}\) is typed by using only type bindings for \(f_1^{(k)},\ldots,
f_\ell^{(k)}\); the second equality follows from the definition of \(\StepFun\)),
%%(note that by the definition of 
%%\(\prog^{(n)}\), the body of \(f^{(k+1)}\) only uses only function symbols \(f_1^{(k)},\ldots,f_\ell^{(k)}\);
%%thus, \(\set{
(ii) \(f_1\COL\qinit\in \TopEnv_n\), and (iii) \(\TopEnv_k\subseteq \TopEnvMax\), and (iv)
\( \TopEnv_n \subseteq \TopEnv_{n-1} \subseteq \cdots \subseteq \TopEnv_0\).
From the conditions (iii), (iv) and \(n=|\TopEnvMax|+1\), there must exist \(k\) such that
\(\TopEnv_k=\TopEnv_{k+1}\). Thus, by this, (i), and (ii), \(\TopEnv_k\) is a fixpoint of
\(\StepFun\) and contains \(f_1\COL \qinit\).
This completes the proof of Theorem~\ref{thm:liveness:eff-sel-effective}.
%%%By the monotonicity of \(\StepFun\), we have:
%%%\[ f_1\COL\qinit\in \TopEnv_n \subseteq \StepFun(\TopEnv_{n-1}) \subseteq \cdots \subseteq \StepFun^n(\TopEnv_0)\subseteq 
%%%\StepFun^n(\TopEnvMax).\]
%%%Thus, we have \(f_1\COL\qinit\in \StepFun^n(\TopEnvMax) = \TopEnv^{(n)}\) as required.
%%%

The witness type environment \(\TopEnv^{(n)}\) is too large in general. In practice, one can find a smaller
witness type environment by using a practical HORS model checking 
algorithm~\cite{Kobayashi13JACM,Kobayashi13horsat,Ramsay14POPL}; by regarding conditionals, non-determinism,
and events as tree constructors, we can see the problem of finding a witness type environment as that of
finding a witness type environment for HORS model checking.


==> appx-liveness-typing-call-seq.tex <==
%subsection: An intersection type system characterising the parity condition of call sequences
\newcommand{\ConstNum}[1]{\overline{#1}}
\newcommand{\Tunitval}{\overline{()}}
\newcommand{\subtype}{\preceq}
\newcommand{\isotype}{\sim}

\newcommand{\PTypeSet}[1]{\mathord{\mathrm{PType}_{#1}}}
\newcommand{\ITypeSet}[1]{\mathord{\mathrm{IType}_{#1}}}

%\newcommand{\sem}[1]{[\![{#1}]\!]}

We define the set of intersection types by:
\begin{align*}
 \Atype &::= \ConstNum{n} \mid \Tunitval \mid \Itype \to \Atype \\
 \Itype &::= \bigwedge_{i \in I} \Atype_{i}.
\end{align*}
Here \( \ConstNum{n} \) is the type for integer expressions evaluated to \( n \), \( \Tunitval \) is the type for the unit value \( () \) and \( \Itype \to \Atype \) is a function type, of which the type for the argument is an intersection type.
An intersection type \( \Itype \) is a collection of types; here the index \( I \) can be empty or infinite.

Formally the families \( \{\, \PTypeSet{\Pst} \,\}_{\Pst} \) and \( \{\, \ITypeSet{\Pest} \,\}_{\Pest} \) of prime types and intersection types are defined by induction on \( \Pst \) and \( \Pest \) as follows:
\begin{align*}
  \PTypeSet{\Tunit} &:= \{\,\Tunitval \,\} \\
  \PTypeSet{\Pest \to \Pst} &:= \ITypeSet{\Pest} \times \PTypeSet{\Pst} \\
  \ITypeSet{\Tint} &:= \{\, \ConstNum{n} \mid n \in \mathbb{N} \,\} \\
  \ITypeSet{\Pst} &:= \mathcal{P}(\PTypeSet{\Pst}).
\end{align*}
A prime type \( \Atype \in \PTypeSet{\Pst} \) is called a \emph{refinement type of \( \Pst \)} and \( \Itype \in \ITypeSet{\Pest} \) a \emph{refinement intersection of \( \Pest \)}.
Given \( \Itype \in \ITypeSet{\Pest} \) and \( \Atype \in \PTypeSet{\Pst} \), we write \( \Itype \to \Atype \) for \( (\Itype, \Atype) \in \PTypeSet{\Pest \to \Pst} \).
Similarly, given a set \( I \) and a family \( \{\,\Atype_{i} \in \PTypeSet{\Pst} \,\}_{i \in I} \), we write \( \bigwedge_{i \in I} \Atype_{i} \) for \( \{\,\Atype_i \mid i \in I \,\} \in \ITypeSet{\Pst} \).

The \emph{subtyping relations} \( \subtype_{\Pst} \) and \( \subtype_{\Pest} \) are defined by induction on \( \Pst \) and \( \Pest \) by the rules in Fig.~\ref{fig:appx:liveness:typing-call-seq:subtyping}.
\begin{figure}[t]
  \infax[]{
    \Tunitval \subtype_{\Tunit} \Tunitval
  }

  \infrule[]{
    \Itype' \subtype_{\Pest} \Itype
    \andalso
    \Atype \subtype_{\Pst} \Atype'
  }{
    \Itype \to \Atype \subtype_{\Pest \to \Pst} \Itype' \to \Atype'
  }
  
  \infax[]{
    \overline{n} \subtype_{\Tint} \overline{n}
  }
  \infrule[]{
    \forall j \in J. \exists i \in I.\; \Atype_i \subtype_{\Pst} \Atype_j'
  }{
    \bigwedge_{i \in I} \Atype_i \subtype_{\Pst} \bigwedge_{j \in J} \Atype_j'
  }
 \caption{Subtyping relations \( ({\subtype_{\Pst}}) \subseteq \PTypeSet{\Pst} \times \PTypeSet{\Pst} \) and \( ({\subtype_{\Pest}}) \subseteq \ITypeSet{\Pest} \times \ITypeSet{\Pest} \).}
 \label{fig:appx:liveness:typing-call-seq:subtyping}
\end{figure}

It is not difficult to see that \( \subtype_{\Pst} \) and \( \subtype_{\Pest} \) are preorders.
Let \( \sim_{\Pst} \) and \( \sim_{\Pest} \) be the equivalence relations induced by \( \subtype_{\Pst} \) and \( \subtype_{\Pest} \).
Then \( (\PTypeSet{\Pst}/{\sim_{\Pst}}, \subtype_{\Pst}) \) and \( (\ITypeSet{\Pest}/{\sim_{\Pest}}, \subtype_{\Pest}) \) are posets.
We shall establish a well-known correspondence between those posets and complete lattices (cf.~Terui~\cite{Terui2012-RTA} and Salvati et al.~\cite{Salvati-ICALP-2012}).
Let us identify \( \typProp \) with \( \Tunit \); then a simple type \( \typ \) for HFL can be naturally identified with a simple type \( \Pst \) for the target language and similarly \( \etyp \) as \( \Pest \).
\begin{lemma}
  Let \( \lts \) be the trivial LTS with one state and no transition.
  Then, for every \( \Pest \), we have
  \[
  (\ITypeSet{\Pest}/{\sim_{\Pest}}, \subtype_{\Pst}) \cong (D_{\lts, \Pest}, \sqleq_{\Pest})
  \]
  as posets.
  (Note that the class ranged over by \( \Pst \) is a subclass of that by \( \Pest \).)
\end{lemma}

A \emph{type environment} \( \ITE \) is a finite mapping from variables to \( \bigcup_{\Pest} \ITypeSet{\Pest} \) that respects the simple types, i.e.~\( (x \COL \Itype) \in \Gamma \) implies \( \Itype \in \ITypeSet{\Pest} \) where \( \Pest \) is the simple type of \( x \).

\begin{figure}[htb]
 \infax[]{
  \pInter \unitexp \COL\Tunitval
 }

 \infax[]{
  \ITE \cup \{x \COL \ConstNum{n}\} \pInter x \COL \ConstNum{n}
 }

 \infrule[]{
   \Atype \subtype \Atype'
 }{
  \ITE \cup \{x \COL \Atype\} \pInter x \COL \Atype'
 }

 \infrule[]{
   \Atype \subtype \Atype'
 }{
   \ITE \cup \{f \COL \Atype\} \pInter f \COL \Atype'
 }

 \infax[]{
  \ITE \pInter n \COL \ConstNum{n}
 }

 \infrule[]{
  \ITE \pInter \term_1 \COL \ConstNum{n} \\
  \ITE \pInter \term_2 \COL \ConstNum{m}
 } {
  \ITE \pInter \term_1 \OP \term_2 \COL \ConstNum{n \OP m}
 }

 \infrule[]{
  \ITE \pInter \term_i \COL \ConstNum{n}_i \; \text{(for i in \{1,\dots,k\})} \\
  \vDash p(n_1, \dots, n_k) \\
  \ITE \pInter \term_{k+1} \COL \Tunitval
 } {
  \ITE \cup \ITE \pInter \ifexp{p(\term_1, \dots, \term_k)}{\term_{k+1}}{\term_{k+2}} \COL \Tunitval
 }

 \infrule[]{
  \ITE \pInter \term_i \COL \ConstNum{n}_i \; \text{(for i in \{1,\dots,k\})} \\
  \vDash \neg p(n_1, \dots, n_k) \\
  \ITE \pInter \term_{k+2} \COL \Tunitval
 } {
  \ITE \cup \ITE \pInter \ifexp{p(\term_1, \dots, \term_k)}{\term_{k+1}}{\term_{k+2}} \COL \Tunitval
 }

 \infrule[]{
  \ITE \pInter \term \COL \Tunitval
 } {
  \ITE \pInter (\evexp{\lab}{\term}) \COL \Tunitval
 }

 \infrule[]{
  \ITE \pInter \term_1 \COL \Tunitval \\
  \ITE \pInter \term_2 \COL \Tunitval
 } {
  \ITE \pInter \term_1 \nondet \term_2 \COL \Tunitval
 }

  \infrule[]{
  \ITE \pInter \term_1 \COL \ConstNum{n} \to \Atype \\
  \ITE \pInter \term_2 \COL \ConstNum{n}
  } {
    \ITE \pInter \App{\term_1}{\term_2} \COL \Atype
  }

 \infrule[]{
 \ITE \pInter \term_1 \COL \bigwedge_{i \in I} \Atype_i \to \Atype' \Rightarrow \term'_1\\
 \ITE \pInter \term_2 \COL \Atype_i \: \text{(for each \(i \in I\))}
 } {
 \ITE \pInter \App{\term_1}{\term_2} : \Atype'
 }
 \caption{intersection type system}
 \label{fig:appx:liveness:inter}
\end{figure}




\tk{to do: define the game \( \mathcal{G}(Q, \Omega) \)}

\tk{I say that \( \Callseq(Q) \) satisfies the parity condition with respect to \( \Omega \) if for every sequence \( (F_1 F_2 \dots) \in \Callseq(Q) \), \( \Omega(F_1) \Omega(F_2) \dots \) satisfies the parity condition; where \( \Omega \) is a mapping from non-terminals to priorities.}
\begin{lemma}
  \( \Callseq(Q) \) satisfies the parity condition with respect to \( \Omega \) if and only if the proponent has a winning strategy of the parity game \( \mathcal{G}(Q, \Omega) \).
\end{lemma}


==> callseq2.tex <==
\nk{I would move the section-specific assumption about programs and the definition
of parity automaton to Section 7.2}


\subsection{Call-sequence analysis}
\label{sec:callsequence}
The call-sequence analysis is a problem on the structure of recursive calls of a given program.
This subsection gives a definition of the problem and reduces it to HFL model checking.

Let us start from an informal description of the problem.
Let \( D \) be a set of function definitions and suppose \( f\,\seq{v} \red_D [\seq{v}/\seq{x}]t \red_D^k g\,\seq{w} \), where \( (f\,\seq{x} = t) \in D \).
We say that \emph{\( f \) is the caller of \( g \)} \nk{This notion of ``caller'' is non-standard;
we should at least say so, or use a different word.} if \( g \) in the right-most term originates from an occurrence of \( g \) in \( t \) in the middle
(strictly speaking, the caller-callee relation relates \emph{occurrences} of function symbols, not the function symbols themselves).
A \emph{call sequence} is a chain of (occurrences of) function symbols related by the caller-callee relation.
The \emph{call sequence analysis} asks, for a given program and a given priority assignment for function symbols, whether every infinite call-sequence of the program satisfies the parity condition.

We need some auxiliary definitions to give a formal definition of the problem.

%% The target language is nondeterministic because of \( \nondet \); hence a term may have different reduction sequences.
%% Here we give a way to describe a particular reduction sequence.
Let \( \RTyPath \) be an infinite sequence consisting of \( \PLeft \) and \( \PRight \), called a \emph{choice sequence}.
We define a reduction relation for pairs of terms and choice sequences by
\[
(\term_1 \nondet \term_2;\, \PLeft \RTyPath) \stackrel{\epsilon}{\red}_D (\term_1; \RTyPath)
\qquad
(\term_1 \nondet \term_2;\, \PRight \RTyPath) \stackrel{\epsilon}{\red}_D (\term_2; \RTyPath)
\]
and \( (u; \RTyPath) \stackrel{\ell}{\red}_D (u'; \RTyPath) \) if \( u \neq u_1 \nondet u_2 \) and \( u \stackrel{\ell}{\red}_D u' \).
A choice sequence resolves nondeterminism of a program \( P \); a reduction sequence is completely determined by its initial term, its length and a choice sequence.
We write \( \red_D^{k} \) for the \( k \)-step reduction relation.
If \( (t_0, \RTyPath_0) \red_D (t_1, \RTyPath_1) \red_D \cdots \red_D (t_k, \RTyPath_k) \), then we write \( \RTyPath_0 \Vdash t_0 \red_D t_1 \red_D \cdots \red_D t_k \) and say that the reduction sequence \( t_0 \red_D t_1 \red_D \cdots \red_D t_k \) follows \( \RTyPath_0 \).

Let \( D = \{ f_i\,\tilde{x}_i = u_i \}_{1 \le i \le n} \) be a finite set of function definitions.
We define \( D^{\dagger} := D \cup \{ f^{\dagger}_i\,\tilde{x} = u_i \}_{1 \le i \le n} \) where \( f^{\dagger}_1, \dots, f^{\dagger}_n \) are fresh symbols.
So \( D^{\dagger} \) has two copies of each function symbol, one of which is marked.
Note that reduction does not introduce a ``new'' marked symbol, although it may increase the number of checked symbols by duplicating them (e.g., if \( (f\,x = g\,x\,x) \in D \), then \( f\,\check{h} = g\,\check{h}\,\check{h} \)).
For a term \( t \), let \( t^{\dagger} \) be the term obtained by replacing \( f \) with \( f^{\dagger} \), i.e.~\( t^{\dagger} := [f_1^{\dagger}/f_1, \dots,f_n^{\dagger}/f_n]t \).
\begin{definition}[Caller-callee relation, call sequence]
  Let \( D \) be a set of function definitions.
  The \emph{caller-callee relation} \( \CallSeqN{k}_D \) (\( k > 0 \)) is defined by
  \[
  (f\,\tilde{v}; \RTyPath) \CallSeqN{k+1}_{D} (g\,\tilde{w}; \RTyPath')
  \qquad\mbox{if}\qquad
  (f\,\seq{x} = t) \in D \quad\mbox{and}\quad ([\tilde{v}/\tilde{x}](t^{\dagger}); \RTyPath) \red_{D^{\dagger}}^k (g^{\dagger}\,\tilde{w}'; \RTyPath'),
  \]
  %
  provided that \( f\,\seq{x} \) and \( g\,\seq{w} \) does not contains \( \dagger \).
  (Here \( \seq{w}' \) may differ from \( \seq{w} \) since some occurrence of \( g \) in \( \seq{w}' \) may be marked.)
  If there exists a (finite or infinite) sequence \( (f\,\tilde{s}; \RTyPath) \CallSeqN{k_1}_D (g_1\,\tilde{u}_1; \RTyPath_1) \CallSeqN{k_2}_D (g_2\,\tilde{u}_2; \RTyPath_2) \CallSeqN{k_3}_D \cdots \), then we write \( \RTyPath \Vdash f\,\tilde{s} \CallSeqN{k_1}_D g_1\,\tilde{u}_1 \CallSeqN{k_2}_D g_2\,\tilde{u}_2 \CallSeqN{k_3}_D \cdots \) and call it a \emph{call sequence of \( f\,\tilde{s} \) following \( \RTyPath \)}.
  We often omit the number \( k_j \) of steps and the choice sequence \( \RTyPath \).
  %
  Given a program \( P = (D, \mainfun) \), the \emph{set of call sequences of \( P \)} is a subset of (finite or infinite) sequences of function symbols defined by
  \( \Callseq(P) := \{\, \mainfun\, g_1\, g_2 \dots \mid \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots \,\} \).
\end{definition}
%% Intuitively, \( (f\,\tilde{v}; \RTyPath) \CallSeqN{k} (g\,\tilde{w}; \RTyPath') \) means that (the occurrence of) \( g \) originates from the body of (this occurrence of) \( f \).
%% Obviously \( f\,\tilde{s} \CallSeqN{k}_D g\,\tilde{u} \) implies \( f\,\tilde{s} \red^k_D g\,\tilde{u} \) but the converse does not hold in general.

\begin{example}
  \tk{to do}
\end{example}

The following property is fundamental.
Here the assumption that a program is simply typed is essential.
\begin{lemma}\label{lem:liveness:unique-existence-of-call-seq}
  Let \( P = (D, \mainfun) \) be a well-typed program and \( \RTyPath \in \{ \PLeft, \PRight \}^{\omega} \) be a choice sequence.
  If the unique reduction sequence \( \RTyPath \Vdash \mainfun \red_D t_1 \red_D t_2 \red_D \cdots \) is infinite, then there exists a unique infinite call-sequence \( \RTyPath \Vdash \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D \cdots \) following \( \RTyPath \).
\end{lemma}


\begin{definition}[Call-sequence analysis]
  A \emph{priority assignment} for a program \( P \) is a function \( \Pfun \COL \Funcs(P) \to \mathbb{N} \) from function symbols of \( P \) to natural numbers.
  %; \( \Pfun(f) \) is called the priority of \( f \).
  \emph{Call-sequence analysis} is the problem of, given a program \( P \) with priority \( \Pfun \), deciding whether every call-sequence \( g_0 g_1 g_2 \dots \in \Callseq(P) \) of \( P \) satisfies the parity condition w.r.t.~\( \Pfun \) (i.e.~\( \max \INF (\Pfun(g_0) \Pfun(g_1) \Pfun(g_2) \dots) \) is even).
\end{definition}

\begin{example}
 \wtnb{Through this example, I wanted to show informal overview of our method without introducing effective selection.}
 Consider the program \(P_{\APP} = (D_\APP, \mainfun)\) where \(D_\APP\) is:
 \begin{align*}
  \mainfun &= \APP\;f\;(-10) \qquad
  \APP\;x\;y = \evexp{\labA}{x\;y} \\
  f\;x &= \ifexp{x \ge 0}{(\evexp{\labB}{\APP\;f\;(x+1)})}{(\APP\;f\;(x+1))}
 \end{align*}
 Let \(\PWA = (\{q_1, q_2\}, \{\labA, \labB\}, \delta, q_1, \Omega)\) be a deterministic parity word automaton,
 where \(\delta(q, \labA) = q_1, \delta(q, \labB) = q_2\) and \(\Omega(q_i) = i\).
 Now, we consider a problem ``\(\InfTraces(P){\stackrel{?}{\subseteq}} \Lang(\PWA)\)``.

 This problem can be translated to a call-sequence analysis for another problem \(Q = (D_Q, \mainfun_D)\) with a priority assignment \(\Pfun_Q\), where \(D_Q\) is:
 \begin{align*}
  \mainfun_Q &= \APP_0\;f_1\;(-10) \qquad
  \APP_0\;x\;y = \termalt_1 \qquad \APP_2\;x\;y = \termalt_1 \qquad
  f_1\;x = \termalt_2 \qquad  f_2\;x = \termalt_2 \\
  \termalt_1 &= \evexp{\labA}{x\;y} \qquad
  \termalt_2 = \ifexp{x \ge 0}{(\evexp{\labB}{\APP_2\;f_2\;(x+1)})}{(\APP_0\;f_1\;(x+1))},
 \end{align*}
 and \(\Pfun_Q(f_i) = i, \Pfun_Q(\APP_i) = i\).
 (A method for constructing such \(Q\) will be discussed in the next subsection.)
 This program \(Q\) is constructed by duplicating function symbols in \(P_\APP\) while adding subscripts.
 Thus, \(\InfTraces(P_\APP) = \InfTraces(Q)\) holds.

 Intuitively, a subscript for a function symbol corresponds the maximal priority of states encountered
 during processing the event sequence generated
 since it is introduced until it appears at the head of a term.

 For example, the following reductions exist:
 \begin{align*}
  \mainfun_Q \Preds{\labA}{D_Q} f_1\;(-10) \Preds{\epsilon}{D_Q} [-10/x]\termalt_2 \Preds{\seq{\ell}}{D_Q} f_1\;(-9), \qquad
  f_1\;(-10) \CallSeqN{2}_{D_Q} f_1\;(-9)
 \end{align*}
 Here, the subscript 1 for \(f_1\) in the term \(f_1\;(-9)\) corresponds
 the maximal priority of states encountered during processing the sequence \(\seq{\ell} = \labA\).

 Therefore, intuitively, the problem whether a run of \(\PWA\) satisfies the parity condition
 can be solved by checking whether a corresponding call-sequence of \(Q\) satisfies the parity condition.

 In this case, \(\Callseq(Q)\) is the following set:
 \begin{align*}
  \Callseq(Q) =
  \{\mainfun f_1^{n} \APP_0 \mid 0 \le n \le 10 \} \cup
  \{\mainfun f_1^{10} f_2^{m} \APP_2 \mid m \in \mathbb{N}\} \cup
  \{\mainfun f_1^{10} f_2^{\omega}\}
 \end{align*}
 The only infinite sequence in \(\Callseq(Q)\) is \(\mainfun f_1^{10} f_2^{\omega}\), which satisfies the parity condition.
 Thus, \(\InfTraces(P) \subseteq \Lang(\PWA)\) holds.
 %
 \qed
\end{example}

The call-sequence analysis can be quite naturally reduced to the HFL model checking against the trivial LTS \( \lts_0 = (\{\star\}, \emptyset, \emptyset, \star) \).

\begin{definition}%[HES \(\HESf_{P}\)]
  Let \(P=(\set{f_{1}\,\seq{x}_1 = \term_1,\ldots,f_{n}\,\seq{x}_n=\term_n}, t_0)\) be a program and \(\Pfun\) be a priority assignment for \(Q\).
  Suppose \(\Pfun(f_i) \ge \Pfun(f_{i+1})\) for each \(i \in \{1,\dots,n-1\}\).
  %For each function symbol \( f \), let us choose a variable of HFL, say \( F \), in such a way that \( f \neq g\) implies \( F \neq G \).
  %\nk{We can just use \(f\) as a variable of HFL, as in the previous sections. We have not made it a rule to use a capital letter for variables of HFL.}
  The translation \( \livetrans{({-})} \) from terms to (fixed-point free) HFL formulas is defined by
  \[
  \begin{array}{l}
    \livetrans{\unitexp} = \TRUE \qquad
    %\livetrans{f} = f \tk{\text{This rule can be removed}}\qquad
    \livetrans{x} = x \qquad
    \livetrans{n} = n \qquad
    \livetrans{(\term_1 \OP \term_2)} = \livetrans{\term_1} \OP \livetrans{\term_2} \\
    \livetrans{(\evexp{\lab}{\term})} = \livetrans{\term} \qquad
    \livetrans{(\term_1\,\term_2)} = \livetrans{\term_1}\,\livetrans{\term_2} \qquad
    \livetrans{(\term_1 \nondet \term_2)} = \livetrans{\term_1} \wedge \livetrans{\term_2} \\
    \livetrans{(\ifexp{p(\Pae_1,\ldots,\Pae_k)}{\term_1}{\term_2})} = (p(\livetrans{\Pae_1},\ldots,\livetrans{\Pae_k}) \wedge \livetrans{\term_1}) \vee (\neg p(\livetrans{\Pae_1},\ldots,\livetrans{\Pae_k}) \wedge \livetrans{\term_2}).
  \end{array}
  \]
  We define the HES \(\HESf_{P} := (\HES_{P}, \livetrans{\term_0})\) by
  \(
  \HES_{P} :=
  (
    f_1\,\seq{x}_1 =_{\munu_1} \livetrans{\term_1};\;
    f_2\,\seq{x}_2 =_{\munu_2} \livetrans{\term_2}; \dots;\;
    f_n\,\seq{x}_n =_{\munu_n} \livetrans{\term_n}
  )
  \)
  where \(\munu_i = \nu \) if \(\Pfun(f_i)\) is even and \(\mu\) otherwise.
\end{definition}

\begin{theorem}
  Let \( P = (D, \mainfun) \) be a program with priority \( \Pfun \).
  Every call-sequence of \( P \) satisfies the parity condition if and only if \( \lts_0 \models \HESf_{P} \).
\end{theorem}


==> liveness-omitted.tex <==
\section{Definitions and Theorems removed from the main text}
\subsection{From 7.1}
Let \( \RTyPath \) be an infinite sequence consisting of \( \PLeft \) and \( \PRight \), called a \emph{choice sequence}.
We define a reduction relation for pairs of terms and choice sequences by
\[
(\term_1 \nondet \term_2;\, \PLeft \RTyPath) \stackrel{\epsilon}{\red}_D (\term_1; \RTyPath)
\qquad
(\term_1 \nondet \term_2;\, \PRight \RTyPath) \stackrel{\epsilon}{\red}_D (\term_2; \RTyPath)
\]
and \( (u; \RTyPath) \stackrel{\ell}{\red}_D (u'; \RTyPath) \) if \( u \neq u_1 \nondet u_2 \) and \( u \stackrel{\ell}{\red}_D u' \).
A choice sequence resolves nondeterminism of a program \( P \); a reduction sequence is completely determined by its initial term, its length and a choice sequence.
We write \( \red_D^{k} \) for the \( k \)-step reduction relation.
If \( (t_0, \RTyPath_0) \red_D (t_1, \RTyPath_1) \red_D \cdots \red_D (t_k, \RTyPath_k) \), then we write \( \RTyPath_0 \Vdash t_0 \red_D t_1 \red_D \cdots \red_D t_k \) and say that the reduction sequence \( t_0 \red_D t_1 \red_D \cdots \red_D t_k \) follows \( \RTyPath_0 \).

Let \( D = \{ f_i\,\tilde{x}_i = u_i \}_{1 \le i \le n} \) be a finite set of function definitions.
We define \( D^{\dagger} := D \cup \{ f^{\dagger}_i\,\tilde{x} = u_i \}_{1 \le i \le n} \) where \( f^{\dagger}_1, \dots, f^{\dagger}_n \) are fresh symbols.
So \( D^{\dagger} \) has two copies of each function symbol, one of which is marked.
Note that reduction does not introduce a ``new'' marked symbol, although it may increase the number of checked symbols by duplicating them (e.g., if \( (f\,x = g\,x\,x) \in D \), then \( f\,\check{h} = g\,\check{h}\,\check{h} \)).
For a term \( t \), let \( t^{\dagger} \) be the term obtained by replacing \( f \) with \( f^{\dagger} \), i.e.~\( t^{\dagger} := [f_1^{\dagger}/f_1, \dots,f_n^{\dagger}/f_n]t \).
\begin{definition}[Caller-callee relation, call sequence]
  Let \( D \) be a set of function definitions.
  The \emph{caller-callee relation} \( \CallSeqN{k}_D \) (\( k > 0 \)) is defined by
  \[
  (f\,\tilde{v}; \RTyPath) \CallSeqN{k+1}_{D} (g\,\tilde{w}; \RTyPath')
  \qquad\mbox{if}\qquad
  (f\,\seq{x} = t) \in D \quad\mbox{and}\quad ([\tilde{v}/\tilde{x}](t^{\dagger}); \RTyPath) \red_{D^{\dagger}}^k (g^{\dagger}\,\tilde{w}'; \RTyPath'),
  \]
  %
  provided that \( f\,\seq{x} \) and \( g\,\seq{w} \) does not contains \( \dagger \).
  (Here \( \seq{w}' \) may differ from \( \seq{w} \) since some occurrence of \( g \) in \( \seq{w}' \) may be marked.)
  If there exists a (finite or infinite) sequence \( (f\,\tilde{s}; \RTyPath) \CallSeqN{k_1}_D (g_1\,\tilde{u}_1; \RTyPath_1) \CallSeqN{k_2}_D (g_2\,\tilde{u}_2; \RTyPath_2) \CallSeqN{k_3}_D \cdots \), then we write \( \RTyPath \Vdash f\,\tilde{s} \CallSeqN{k_1}_D g_1\,\tilde{u}_1 \CallSeqN{k_2}_D g_2\,\tilde{u}_2 \CallSeqN{k_3}_D \cdots \) and call it a \emph{call sequence of \( f\,\tilde{s} \) following \( \RTyPath \)}.
  We often omit the number \( k_j \) of steps and the choice sequence \( \RTyPath \).
  %
  Given a program \( P = (D, \mainfun) \), the \emph{set of call sequences of \( P \)} is a subset of (finite or infinite) sequences of function symbols defined by
  \( \Callseq(P) := \{\, \mainfun\, g_1\, g_2 \dots \mid \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots \,\} \).
\end{definition}
%% Intuitively, \( (f\,\tilde{v}; \RTyPath) \CallSeqN{k} (g\,\tilde{w}; \RTyPath') \) means that (the occurrence of) \( g \) originates from the body of (this occurrence of) \( f \).
%% Obviously \( f\,\tilde{s} \CallSeqN{k}_D g\,\tilde{u} \) implies \( f\,\tilde{s} \red^k_D g\,\tilde{u} \) but the converse does not hold in general.

\begin{lemma}\label{lem:liveness:unique-existence-of-call-seq}
  Let \( P = (D, \mainfun) \) be a program and \( \RTyPath \in \{ \PLeft, \PRight \}^{\omega} \) be a choice sequence.
  If the unique reduction sequence \( \RTyPath \Vdash \mainfun \red_D t_1 \red_D t_2 \red_D \cdots \) is infinite, then there exists a unique infinite call-sequence \( \RTyPath \Vdash \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D \cdots \) following \( \RTyPath \).
\end{lemma}

\obsolete{
\begin{definition}[Call-sequence analysis]
  A \emph{priority assignment} for a program \( P \) is a function \( \Pfun \COL \Funcs(P) \to \Nat \) from function symbols of \( P \) to natural numbers.
  %; \( \Pfun(f) \) is called the priority of \( f \).
  \emph{Call-sequence analysis} is the problem of, given a program \( P \) with priority \( \Pfun \), deciding whether every call-sequence of \( P \) satisfies the parity condition w.r.t.~\( \Pfun \).
  Here an infinite sequence \( g_0 g_1 g_2 \dots \in \Callseq(P) \) is said to satisfy the parity condition if the maximum of the numbers appearing infinitely often in \( \Pfun(g_0) \Pfun(g_1) \Pfun(g_2) \dots \) is even.
\end{definition}
\begin{example}
 \wtnb{Through this example, I wanted to show informal overview of our method without introducing effective selection.}
 Consider the program \(P_{\APP} = (D_\APP, \mainfun)\) where \(D_\APP\) is:
 \begin{align*}
  \mainfun &= \APP\;f\;(-10) \qquad
  \APP\;x\;y = \evexp{\labA}{x\;y} \\
  f\;x &= \ifexp{x \ge 0}{(\evexp{\labB}{\APP\;f\;(x+1)})}{(\APP\;f\;(x+1))}
 \end{align*}
 Let \(\PWA = (\{q_1, q_2\}, \{\labA, \labB\}, \delta, q_1, \Omega)\) be a deterministic parity word automaton,
 where \(\delta(q, \labA) = q_1, \delta(q, \labB) = q_2\) and \(\Omega(q_i) = i\).
 Now, we consider a problem ``\(\InfTraces(P){\stackrel{?}{\subseteq}} \Lang(\PWA)\)``.

 This problem can be translated to a call-sequence analysis for another problem \(Q = (D_Q, \mainfun_D)\) with a priority assignment \(\Pfun_Q\), where \(D_Q\) is:
 \begin{align*}
  \mainfun_Q &= \APP_0\;f_1\;(-10) \qquad
  \APP_0\;x\;y = \termalt_1 \qquad \APP_2\;x\;y = \termalt_1 \qquad
  f_1\;x = \termalt_2 \qquad  f_2\;x = \termalt_2 \\
  \termalt_1 &= \evexp{\labA}{x\;y} \qquad
  \termalt_2 = \ifexp{x \ge 0}{(\evexp{\labB}{\APP_2\;f_2\;(x+1)})}{(\APP_0\;f_1\;(x+1))},
 \end{align*}
 and \(\Pfun_Q(f_i) = i, \Pfun_Q(\APP_i) = i\).
 (A method for constructing such \(Q\) will be discussed in the next subsection.)
 This program \(Q\) is constructed by duplicating function symbols in \(P_\APP\) while adding subscripts.
 Thus, \(\InfTraces(P_\APP) = \InfTraces(Q)\) holds.

 Intuitively, a subscript for a function symbol corresponds the maximal priority of states encountered
 during processing the event sequence generated
 since it is introduced until it appears at the head of a term.

 For example, the following reductions exist:
 \begin{align*}
  \mainfun_Q \Preds{\labA}{D_Q} f_1\;(-10) \Preds{\epsilon}{D_Q} [-10/x]\termalt_2 \Preds{\seq{\ell}}{D_Q} f_1\;(-9), \qquad
  f_1\;(-10) \CallSeqN{2}_{D_Q} f_1\;(-9)
 \end{align*}
 Here, the subscript 1 for \(f_1\) in the term \(f_1\;(-9)\) corresponds
 the maximal priority of states encountered during processing the sequence \(\seq{\ell} = \labA\).

 Therefore, intuitively, the problem whether a run of \(\PWA\) satisfies the parity condition
 can be solved by checking whether a corresponding call-sequence of \(Q\) satisfies the parity condition.

 In this case, \(\Callseq(Q)\) is the following set:
 \begin{align*}
  \Callseq(Q) =
  \{\mainfun f_1^{n} \APP_0 \mid 0 \le n \le 10 \} \cup
  \{\mainfun f_1^{10} f_2^{m} \APP_2 \mid m \in \mathbb{N}\} \cup
  \{\mainfun f_1^{10} f_2^{\omega}\}
 \end{align*}
 The only infinite sequence in \(\Callseq(Q)\) is \(\mainfun f_1^{10} f_2^{\omega}\), which satisfies the parity condition.
 Thus, \(\InfTraces(P) \subseteq \Lang(\PWA)\) holds.
 %
 \qed
\end{example}
}


\subsection{From 7.2}

\obsolete{
Let \(P\) be a program and \(\PWA\) be a deterministic parity word automaton.
This subsection gives a construction of another program \( \progqPA \) with priority \( \Pfun_{P, \PWA} \) such that \( \InfTraces(P){\subseteq} \Lang(\PWA) \) if and only if every infinite call-sequence of \( \progqPA \) satisfies the parity condition with respect to \( \Pfun_{P,\PWA} \).

For the sake of simplicity, we assume that every program \(\prog=(\progd, \mainfun)\) in this section has no terminating reduction and
every infinite reduction sequence produces infinite events.
Hence \(\FullTraces(\prog) = \InfTraces(\prog)\).
We can assume this without loss of generality.

We use deterministic parity word automata~\cite{Automata} to describe \(\omega\)-regular languages.
\begin{definition}[Parity automaton]
 An \emph{deterministic parity word automaton} is a quintuple \(\PWA = (Q, \Sigma, \delta, \qinit, \Omega)\) where
 \begin{itemize}
  \item \(Q\) is a finite set of states,
  \item \(\Sigma\) is a finite alphabet,
  \item \(\delta \COL Q \times \Sigma \to Q\) is a transition function,
  \item \(\qinit \in Q\) is the initial state and
  \item \(\Omega \COL Q \to \{0, \dots, p-1\}\) is the priority function.
 \end{itemize}
 \wtnb{The name \(Q\) conflicts with \(Q_{\prog,\PWA}\)}
 %Let \(\PWA = (Q, \Sigma, \delta, \qinit, \Omega)\) be a deterministic parity word automaton.
 The \emph{run} of \(\PWA\) on a word \(a_0 a_1 \dots \in \Sigma^* \cup \Sigma^{\omega}\) is
 a sequence of states \(\rho = \rho(0) \rho(1) \dots \in Q^{*} \cup Q^{\omega}\) of the same length as \( a \) such that
 \begin{enumerate}
  \item \(\rho(0) = \qinit\), and
  \item \(\forall i \ge 0. \rho(i+1) = \delta(\rho(i), a_i)\).
 \end{enumerate}
 %
 An \(\omega\)-word \(w \in \Sigma^{\omega}\) is \emph{accepted} by \(\PWA\) when
 the run \(\rho\) of \(\PWA\) on \(w\) satisfies the following:
 \[
  \MAX\{\Omega(q) \mid q \in \INF(\rho)\} \text{is even},
 \]
 where \(\INF(\rho)\) is the set of states that occur infinitely often in \(\rho\).
 We write \( \Lang(\PWA) \) for the set of \( \omega \)-words accepted by \( \PWA \).
\end{definition}
%% For the sake of simplicity, we only consider \(\PWA\) that does not get stuck
%% and we assume that \(\Omega(\qinit) = 0\).

Since \( \PWA \) is deterministic, it has a run for every infinite trace.
So the matter is whether, for every trace, the unique run satisfies the parity condition.
The idea is to use an intersection type system characterising the behaviour of \( \PWA \) over a given program, which is a modification of the type system of Kobayashi and Ong~\cite{KO09LICS}.
This is also related to the technique known as effective selection~\cite{Carayol12LICS, DBLP:conf/csl/TsukadaO14, DBLP:conf/fsttcs/Haddad13}.

%% First, we prepare a renaming function \(\renameFun_P(\term, d)\).
%% \begin{definition}
%%  Let \(P\) be a program, \(\term\) be a term and \(d\) be a symbol.
%%  Suppose \(\Funcs(P) = \{f_1,\dots,f_n\}\).
%%  We define \emph{renaming function} \(\renameFun_P\) by
%%  \[
%%  \renameFun_P(\term, d) ::= [\wtLabel{f}{d}_{1}/f_{1}, \dots, \wtLabel{f}{d}_{n}/f_{n}]\term.
%%  \]
%%  We sometimes omit the subscript \(P\) if it is clear from the context.
%% \end{definition}
%% The symbol \([d]\) in \(\wtLabel{f}{d}\) is used to identify where \(f\) originates.
%%
%% In addition, we add the following rule to the labeled transition semantics defined in Figure~\ref{fig:os}:
%% \infrule{
%%  f \seq{x} = \termalt \in \progd \andalso
%%  |\seq{x}|=|\seq{\term}|
%% } {
%%  \wtLabel{f}{d}\;\seq{\term} \Pred{\epsilon}{\progd} [\seq{\term}/\seq{x}]\termalt
%% }
%% This means that the symbol \(\wtLabel{f}{d}\) is different from the symbol \(f\) syntactically, but same with \(f\) semantically.

%\tk{I propose not to remove events by the effective selection.  Then the property expected to \( Q_{P, \PWA} \) can be simply expressed as follows.
%  \begin{itemize}
%  \item \( \InfTraces(P) = \InfTraces(Q_{P, \PWA}) \).
%    Hence \( P \) satisfies \( \PWA \) if and only if so does \( Q_{P, \PWA} \).
%  \item If
%    \(
%    \mainfun \stackrel{\ell_1 \dots \ell_{k-1}}{\longrightarrow_Q^*}
%    f_{i_1, m_{i_1}}\;\tilde{\term} \stackrel{\epsilon}{\longrightarrow}
%    [\tilde{f}^{(1)}/\tilde{f}][\tilde{\term}/\tilde{x}]\term_{i_1} \stackrel{\ell_{k+1} \dots \ell_{k'}}{\longrightarrow_Q^*}
%    f^{(1)}_{i_2, m_{i_2}}\;\tilde{\term_2}
%    \),
%    then \( m_{i_2} \) is the maximal priority of states encountered during processing \( \ell_{k+1} \dots \ell_{k'} \).
%    That means, if \( q_0 \stackrel{\ell_1}{\to} q_1 \stackrel{\ell_2}{\to} \dots \stackrel{q_{k-1}}{\to} q_{k-1} \stackrel{\epsilon}{\to} q_k \stackrel{\ell_{k+1}}{\to} \dots \stackrel{\ell_{k'}}{\to} q_{k'} \) is the transition of \( \PWA \) (which is unique since \( \PWA \) is deterministic), then \( i_{m_2} = \max_{k \le j \le k'} \Omega(q_j) \).
%  \end{itemize}
%  Under the second condition, \( Q_{P, \PWA} \) satisfies the specification given by \( \PWA \) if and only if the call sequences of \( Q_{P, \PWA} \) satisfies the parity condition.
%}

%% Now, we would like to create a program \(\progqPA = (\progd_Q, \mainfun_Q)\) and a function \(\Pfun_Q \COL \Funcs(\progqPA) \to \mathbb{N}\) that satisfies the following two conditions:
%%   \begin{itemize}
%%    \item[Cond. (i)] \( \InfTraces(P) = \InfTraces(\progqPA) \).
%%    \item[Cond. (ii)]
%%                 If
%%                 \(
%%                 \mainfun_Q \stackrel{\ell_1 \dots \ell_{k-1}}{\longrightarrow_{\progd_Q}^*}
%%                 f_{1}\;\seq{\term_1} \stackrel{\epsilon}{\longrightarrow}
%%                 [\seq{\term}/\seq{x}]\termalt_{1}
%%                 \),
%%                 \(
%%                 [\seq{\term}/\seq{x}]\renameFun(\termalt_{1},d) \stackrel{\ell_{k+1} \dots \ell_{k'}}{\longrightarrow_{\progd_Q}^*}
%%                 \wtLabel{f}{d}_{2}\;\seq{\term_2}
%%                 \) and
%%                 \(\rho\) is the run of \(\PWA\) on \(\ell_1\dots\ell_{k-1}\ell_{k+1}\dots\ell_{k'}\),
%%                 then \( \Pfun_Q(f_2) = \MAX\{\Omega(\rho(i)) \mid k+1 \le i \le k'\}\) holds.
%%   \end{itemize}
%%   \wtnb{\(\MAX\{\Omega(\rho(i)) \mid k \le i \le k'\}\)? I will check it again.}

%% Cond. (ii) means, if \( q_0 \stackrel{\ell_1}{\to} q_1 \stackrel{\ell_2}{\to} \dots \stackrel{q_{k-1}}{\to} q_{k-1} \stackrel{\epsilon}{\to} q_k \stackrel{\ell_{k+1}}{\to} \dots \stackrel{\ell_{k'}}{\to} q_{k'} \) is the transition of \( \PWA \) (which is unique since \( \PWA \) is deterministic), then \( \Pfun_Q(f_2) = \MAX \{\Omega(q_j) \mid k \le j \le k'\}\).

%% We call a function \(\Pfun_Q\) a \emph{priority assignment for \(Q\)}.

%%We can obtain such \(\progqPA\) and \(\Pfun_Q\) by effective selection~\cite{Carayol12LICS, DBLP:conf/csl/TsukadaO14, DBLP:conf/fsttcs/Haddad13}.
We define the set of intersection types.
\begin{definition}
 Let \(\PWA = (Q, \Sigma, \delta, \qinit, \Omega)\) be a deterministic parity word automaton.
 Let \(q\) and \(m\) range over \(Q\) and the set of priorities. %\(\{\Omega(q) \mid q \in Q \} \).
 The set of \emph{intersection types}, ranged over by \(\Atype\), is defined by:
 \[
 \begin{array}{l}
  \Atype ::= q \mid \Itype \to \Atype \qquad
  \qquad \Itype ::= \INT \mid \bigwedge_{1 \le i \le k} (\Atype_i, m_i)
 \end{array}
\]
\end{definition}

%% The binary relation \(\Atype \CCOL \Pst\) is defined:
%% \begin{multicols}{3}
%%   \infrule{}{
%%     q \CCOL \Tunit
%%   }
%%   \infrule{
%%     \Atype \CCOL \Pst
%%   }{
%%     (\Tint \to \Atype) \CCOL (\Tint \to \Pst)
%%   }
%%   \infrule{
%%     \forall i \in \{1,\dots,k\}.\Atype_i \CCOL \Pst_1 \andalso
%%     \Atype \CCOL \Pst_2
%%   }{
%%     (\bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype) \CCOL (\Pst_1 \to \Pst_2)
%%   }
%% \end{multicols}

An \emph{intersection type environment} \( \ITE \) is a finite set of type bindings of the form \(x \COL \INT\) or \(x \COL (\Atype, m, m')\).
We allow multiple type binding for a variable \( x \) except for \( x \COL \INT \) (i.e.~if \( x \COL \INT \in \ITE \), then this must be the unique type binding for \(x \) in \( \ITE \)).

The \emph{effective selection relation} for expressions is of the form \(\ITE \pInter \term \COL \Atype \ESRel \term'\), where \(\ITE\) is an intersection type environment, \( \term \) is a term, \( \Atype \) is a type and \( \term' \) is a result of the translation.

The rules for effective selection are given in Figure~\ref{fig:inter}.
The operation \(\ITE \RaiseP m\) is defined by:
\[
 \ITE \RaiseP m ::= \{x \COL \INT \mid x \COL \INT \in \ITE \} \cup \{x \COL (\Atype, m_1, \MAX(m_2, m)) \mid x \COL (\Atype, m_1, m_2) \in \ITE \}
\]
%% These effective selection rules preserve typability of terms.
%% In other words,
%% if \(\STE \p \term \COL \Pst\) and \(\ITE \pInter \term \COL \Atype \ESRel \term'\) holds,
%% then there exists \(\STE'\) such that \(\STE' \p \term' \COL \Pst\).
%% Here, we write \(x:\Itype\) for \(\{x \COL (\Atype_i, m_i, m_i) \mid 1 \le i \le k \}\) if \(\Itype = \bigwedge_{1 \le i \le k} (\Atype_i, m_i)\).


Basically a judgement \( \ITE \pInter t : \Atype \Rightarrow t' \) is an intersection type judgement \( \ITE \pInter t : \Atype \) together with its term representation \( t' \).
We write \( \ITE \pInter t : \Atype \) if \( \ITE \pInter t : \Atype \Rightarrow t' \) for some \( t' \).

A \emph{top-level type environment} \( \TopEnv \) is a finite set of type bindings of the form \( x : (\Atype, m) \).
Similar to the intersection type environments, \( \TopEnv \) may have several bindings for a variable.
We write \( \TopEnv \pInter t : \Atype \) to mean \( \{ x : (\theta, m, 0) \mid x : (\theta, m) \in \TopEnv \} \pInter t : \Atype \).
} % obsolete


We write \( \TopEnv \pInter D \) if \( \TopEnv \pInter D(f) : \Atype \) for every \( f : (\Atype,m) \in \TopEnv \).
For a program \( P = (D, t) \), we write \( \TopEnv \pInter P \) if \( \TopEnv \pInter D \) and \( \TopEnv \pInter t : \qinit \).

Given a state \( q \in Q \) and a sequence \( \seq{\ell} \) of events, there exists a unique run \( R \) of \( \PWA \) over \( \seq{\ell} \) with \( R(0) = q \).
Then the \emph{summary of the run of \( \PWA \) from \( q \) over \( \seq{\ell} \)}, written as \( \SUMMARY_{\PWA}(q, \seq{\ell}) \) is defined as \( \max \{ \Omega(R(i)) \mid 0 < i \le |\seq{\ell}| \} \).
%% \[
%% \SUMMARY(q, \seq{\ell}) ::=
%% \begin{cases}
%%   0 & (\seq{\ell} = \epsilon) \\
%%   \MAX(\Omega(\delta(q, \ell_1)), \SUMMARY(\delta(q, \ell_1), \seq{\ell'})) & (\seq{\ell} = \ell_1\seq{\ell'}).
%% \end{cases}
%% \]
\begin{lemma}
  Let \( P = (D, \mainfun) \) be a program and assume \( \TopEnv \pInter P \).
  Suppose that \( \mainfun \mathrel{\stackrel{\seq{\ell}_1}{\red}{}\!\!{}_D^*} f\,\seq{s} \) and \( f\,\seq{s} \CallSeq_D g\,\seq{u} \).
  Let \( q = \delta^*_{\PWA}(\qinit, \seq{\ell}_1) \) and \( \seq{\ell}_2 \) be a sequence of events such that \( f\,\seq{s} \CallSeq_D g\,\seq{u} \).
  Then \( g : (\Atype, \SUMMARY(q, \seq{\ell}_2)) \in \TopEnv \) for some \( \Atype \).
\end{lemma}

%% \begin{lemma}
%%   Assume \( \TopEnv \pInter D \) and \( \TopEnv \pInter f\,\seq{s} : q \).
%%   If \( \RTyPath \Vdash f\,\seq{s} \mathrel{\stackrel{\seq{\ell}}{\red}\!\!{}^k_{D}} g\,\seq{u} \) %(\( \seq{\ell} \in (\lab \cup \{\epsilon\})^* \))
%%   and \( \RTyPath \Vdash f\,\seq{s} \CallSeqN{k}_{D} g\,\seq{u} \), then \( (g : (\Atype, \SUMMARY(q, \seq{\ell}))) \in \TopEnv \) for some \( \Atype \) and \( \ITE \pInter g\,\seq{u} : \delta(q,\seq{\ell}) \),
%%  where
%%  \[
%%  \SUMMARY(q, \seq{\ell}) ::=
%%  \begin{cases}
%%   0 & (\seq{\ell} = \epsilon) \\
%%   \MAX(\Omega(\delta(q, \ell_1)), \SUMMARY(\delta(q, \ell_1), \seq{\ell'})) & (\seq{\ell} = \ell_1\seq{\ell'}).
%%  \end{cases}
%%  \]
%% \end{lemma}


\begin{corollary}%\label{cor:liveness:summarising-priority}
  Assume \( \TopEnv \pInter (D, \mainfun) \) % and \( \TopEnv \pInter f\,\seq{s} : \qinit \).
  and let \( \mainfun \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2 \seq{u}_2 \CallSeq_D \cdots \) be an infinite call-sequence.
  Let \( R \) be the unique run of \( \PWA \) over the infinite event sequence generated by the corresponding reduction sequence.
  Then there exists a family \( \{ (\Atype_i, m_i) \}_{i \ge 1} \) such that \( g_i : (\Atype_i, m_i) \in \TopEnv \) (for every \( i \ge 1 \)) and \( \max \mathbf{Inf}(\Omega(R)) = \max \mathbf{Inf}(m_1 m_2 \dots) \).
\end{corollary}
\begin{proof}
  Iterative application of the above lemma.
\end{proof}

As a special case of the above corollary, if \( g_i \) has a unique type binding in \( \TopEnv \) for each \( i \), then the sequence \( m_1 m_2 \dots \) is uniquely determined and the parity condition of \( m_1 m_2 \dots \) coincides with that of the run \( R \).
Let us say that a top-level environment \( \TopEnv \) is \emph{simple} if \( \TopEnv(f) := \{ (\Atype,m) \mid f : (\Atype,m) \in \TopEnv \} \) is singleton for every \( f \in \dom(\ITE) \).
For a simple top-level environment \( \TopEnv \), we define a priority assignment \( \Pfun_{\TopEnv} \) by \( \Pfun_{\TopEnv}(f) = m \) if \( \exists \Atype.\, f : (\Atype,m) \in \TopEnv \).

%% \begin{corollary}\label{cor:liveness:summarising-priority}
%%   Assume \( \TopEnv \pInter D \) and \( \TopEnv \pInter f\,\seq{s} : \qinit \).
%%   Let \( \RTyPath \Vdash f\,\seq{s} \stackrel{\ell_1}{\red}_D t_1 \stackrel{\ell_2}{\red}_D \cdots \) be the infinite reduction sequence following \( \RTyPath \) and \( \runseq \) be the run of \( \PWA \) over \( \ell_1 \ell_2 \cdots \).
%%   Then, for every infinite call-sequence \( \RTyPath \Vdash f\,\seq{s} \CallSeq_D g_1\,\seq{u}_1 \CallSeq_D g_2\,\seq{u}_2 \CallSeq_D \cdots \) following \( \RTyPath \), there exists \( \{ (\Atype_i, m_i) \}_{i \ge 1} \) such that \( g_i : (\Atype_i, m_i) \in \TopEnv \) (for every \( i \ge 1 \)) and \( \max \mathbf{Inf}(\Omega(R)) = \max \mathbf{Inf}(m_1 m_2 \dots) \).
%% \end{corollary}
%% \begin{proof}
%%   Iterative application of the above lemma.
%% \end{proof}


The effective selection is a technique of translating an intersection type derivation to a simply-typed term, by regarding an intersection type \( \bigwedge_{1 \le i \le k} (\Atype_i, m_i) \) as the product type \( \prod_{1 \le i \le k} (\Atype_i, m_i) \).
Formally the translation on types is defined by:
\begin{align*}
  \EffTypeTrans{q} &:= q \\
  \EffTypeTrans{\INT \to \Atype} &:= \INT \to (\EffTypeTrans{\Atype}) \\
  \EffTypeTrans{\bigwedge_{1 \le i \le k} (\Atype_i, m_i) \to \Atype_0} &:= (\EffTypeTrans{\Atype_1}, m_1) \to \dots \to (\EffTypeTrans{\Atype_k}, m_k) \to \EffTypeTrans{\Atype_0}.
\end{align*}
For a top-level type environment \( \TopEnv \), we define \( \EffTypeTrans{\TopEnv} := \{ x_{\Atype,m} : (\Atype,m) \mid x : (\Atype,m) \in \TopEnv \} \).
The translation of terms is given by the right-most component \( t' \) of judgement \( \ITE \pInter t : \Atype \Rightarrow t' \).
For a set \( D \) of function definitions, we write \( \TopEnv \pInter D \Rightarrow D' \) if \( \dom(D') = \{\, f_{\Atype,m} \mid f : (\Atype, m) \in \TopEnv \,\} \) and \( \TopEnv \pInter D(f) : \Atype \Rightarrow D'(f_{\Atype,m}) \) for every \( f : (\Atype, m) \in \TopEnv \).
For a program \( P = (D, t) \), we write \( \TopEnv \pInter P \Rightarrow P' \) if \( P' = (D', t') \), \( \TopEnv \pInter D \Rightarrow D' \) and \( \TopEnv \pInter t : \qinit \Rightarrow t' \).


%% Given a program \( P = (D, t) \), the result of the translation is \( P' = (D', t') \) such that \( \TopEnv \pInter D \Rightarrow D' \), \( \TopEnv \pInter t : \qinit \Rightarrow t' \) for some \( \TopEnv \).
%% The priority assignment for \( P' \) is \( \Pfun_{\EffTypeTrans{\TopEnv}} \).
%% Let \( P = (D, t) \) and assume that \( \ITE \pInter D \).
%% If \( \ITE \pInter t : \qinit \Rightarrow t' \), then we define \( \progqPA = (\EffTypeTrans{D}, t') \).


%% \begin{definition}
%%  A \emph{trivial game} is a tuple \((V_{\forall}, V_{\exists}, v_0, E_{\forall} \cup E_{\exists})\) such that \wtnb{to do: fill out}
%% \end{definition}

%% We construct a trivial game \(\TG_{P,\PWA} = (V_{\forall}, V_{\exists}, v_0, E_{\forall} \cup E_{\exists})\), where
%% \begin{align*}
%%  V_{\forall} &= \{\ITE \mid dom(\ITE) \subseteq dom(\STE), \forall f \COL (\Atype, m, m') \in \ITE. \Atype \CCOL \STE(f) \wedge m = m'\} \\
%%  V_{\exists} &= \{ (f, \Atype, m) \mid \App{f}{\seq{x}}=\term \in \progd_\prog, \Atype \CCOL \STE(f), m \in cod(\Omega)\}\\
%%  E_{\forall} &= \{(\ITE, (f, \Atype, m)) \mid f : (\Atype, m, m) \in \ITE\} \\
%%  E_{\exists} &=
%%  \left\{\begin{array}{@{}c|c@{}}
%%   & \App{f}{\seq{x}}=\term \in \progd_\prog,\\
%%   & \Atype = \Itype_1 \to \dots \to \Itype_k \to \Atype',\\
%%   ((f, \Atype, m), \ITE) & \forall j \in \{1,\dots,k\}.\;\Itype'_j \le \Itype_j, \\
%%   &\forall j \in \{1,\dots,k\}.\; x_j \not\in dom(\ITE),\\
%%   &  \ITE, x_1 : \Itype'_1, \dots, x_k : \Itype'_k \pInter \term \COL \Atype' \ESRel \term'
%%  \end{array}\right\} \\
%%  v_0 &= (\mainfun, q_I, 0).
%% \end{align*}
%% where \(\Itype_1 \le \Itype_2\) is defined by:
%% \begin{multicols}{2}
%%  \infax{
%%   \Tint \le \Tint
%%  }
%%  \infrule{
%%   I \subseteq \{1,\dots,k\}
%%  }{
%%   \bigwedge_{1\le i \le k, i \in I}(\Atype_i, m_i) \le \bigwedge_{1\le i \le k}(\Atype_i, m_i)
%%  }
%% \end{multicols}

%% \(\TG_{P,\PWA}\) is a variant of parity game for HORS model checking~\cite{KO11LMCS} and there exists a winning strategy if \(P\) is a simply-typed program.\wtnb{Explain the reason.}

%% Now, we fix a wining strategy \(\winning\) for \(\TG_{P,\PWA}\) and
%% create a program \(\progqPAW = (\progd_Q, \mainfun_{q_I, 0})\) with a priority assignment \(\Pfun_{\progqPAW}\), where
%% \begin{align*}
%%  \progd_Q &=  \left\{\begin{array}{@{}c|c@{}}
%%   &((f, \Atype, m), \ITE) \in \winning, \\
%%   & \App{f}{\seq{x}}=\term \in \progd_\prog,\\
%%   f_{\Atype, m}\;\dup{x_1, \Itype_1} \dots \dup{x_k,\Itype_k} = \term'& \Atype = \Itype_1 \to \dots \to \Itype_k \to \Atype',\\
%%   & \forall j \in \{1,\dots,k\}.\;\Itype'_j \le \Itype_j, \\
%%   &\forall j \in \{1,\dots,k\}.\; x_j \not\in dom(\ITE),\\
%%   &  \ITE, x_1 : \Itype'_1, \dots, x_k : \Itype'_k \pInter \term \COL \Atype' \ESRel \term'
%%                      \end{array}\right\} \\
%%   \dup{x,\Itype} &::= \begin{cases}
%%               x_{\INT} & (\Itype = \INT) \\
%%               x_{\Atype_1,m_1} \dots x_{\Atype_k,m_k} & (\Itype = \bigwedge_{1\le i \le k} (\Atype_i, m_i))
%%              \end{cases} \\
%%  \Pfun_\progqPAW(f_{\Atype, m}) &= m.
%% \end{align*}

%% \begin{theorem}\label{theorem:q_pa}
%%  Let \(\prog\) be a program, \(\PWA\) be a deterministic parity word automaton.
%%  Suppose \(\winning\) is a winning strategy for the trivial game \(\TG_{\prog, \PWA}\).
%%  Then, the program \(\progqPAW\) and the priority assignment \(\Pfun_\progqPAW\) satisfy both of Cond.(i) and Cond.(ii).
%% \end{theorem}

\begin{example}
 \label{liveness:example:program}
 \wtnb{An example that needs intersection types. But, this may be too complicated.}
 Consider the program \(P = (\progd, \mainfun)\), where \(\progd\) is:
 \begin{align*}
  \mainfun &= \evexp{\labC}{f\;(g\;h)\;0} \\
  f\;k\;x &= \evexp{\labA}{\ifexp{x = 0}{k\;0}{f\;(g\;k)\;(x-1)}}\\
  g\;k\;x &= \evexp{\labB}{k\;(x+1)}\\
  h\;x &= \evexp{\labC}{f\;(g\;h)\;x}
 \end{align*}
 The reduction sequence of this program is like:
 \begin{align*}
  \mainfun
  &\Pred{\labC}{P}  f\;(g\;h)\;0 \Pred{\labA}{P}    g\;h\;0      \Pred{\labB}{P} h\;1 \\
  &\Preds{\labC}{P} f\;(g\;h)\;1 \Preds{\labA^2}{P} g\;(g\;h)\;0 \Pred{\labB^2}{P} h\;2 \\
  &\Preds{\labC}{P} \dots \\
  &\Preds{\labC}{P} f\;(g\;h)\;n \Preds{\labA^n}{P}
  g\;\underbrace{(g(\dots(g}_{(n-1) \text{times}}\;h)\dots)\;0 \Preds{\labB^n}{P} h\;n \\
  &\Preds{\labC}{P} \dots.
 \end{align*}
 Thus, \(P\) generates the event sequence \(\labC \labA\labB\labC \labA^2\labB^2\labC \labA^3\labB^3\labC \dots \labA^{n}\labB^{n}\labC \dots\).

 Now, we prepare a deterministic parity word automaton \(\PWA = (\{q_0, q_1, q_2\}, \{\labA, \labB, \labC\}, \delta, q_0, \{q_0 \mapsto 0, q_1 \mapsto 1, q_2 \mapsto 2\})\), where \(\delta(q, \labA) = q_0, \delta(q, \labB) = q_1\) and \(\delta(q, \labC) = q_2\).
 This automaton represent the specification that if event \(\labB\) occurs infinitely often in an event sequence generated by a program, event \(\labC\) must also occur infinitely often.
 Therefore, for every \(w \in \InfTraces(\prog)\) is accepted by \(\PWA\).
\end{example}
\begin{example}
 \label{liveness:example:effective_selection}
 Let \(P\) and \(\PWA\) be the program and the parity word automaton introduced in Example~\ref{liveness:example:program}.
 Now, we construct a program \(\progqPA = (\progd_\progq, \mainfun_{q_0, 0})\).
 \(\progd_\progq\) consists of the following:
 \begin{align*}
  &\funq{f}{0}{0}\;\funq{k}{5}{0}\;\funq{k}{4}{1}\;\xint = \term_0,
  &\funq{f}{1}{2}\;\funq{k}{5}{0}\;\funq{k}{4}{1}\;\xint = \term_0 \\
  &\funq{g}{2}{0}\;\funq{k}{4}{1}\;\xint = \term_1
  &\funq{g}{2}{2}\;\funq{k}{4}{1}\;\xint = \term_1 \\
  &\funq{g}{3}{1}\;\funq{k}{4}{1}\;\xint = \term_1
  &\funq{g}{3}{2}\;\funq{k}{4}{1}\;\xint = \term_1 \\
  \funq{h}{4}{2}\;\xint &= \evexp{\labC}{\funq{f}{1}{2}\;(\funq{g}{2}{2}\;\funq{h}{4}{2})\;(\funq{g}{3}{2}\;\funq{h}{4}{2})\;\xint} \\
  \mainfun_{q_0, 0} &= \evexp{\labC}{\funq{f}{1}{2}\;(\funq{g}{2}{2}\;\funq{h}{4}{2})\;(\funq{g}{3}{2}\;\funq{h}{4}{2})\;0}
 \end{align*}
 where
 \begin{align*}
  \term_0 &=
  \evexp{\labA}{
    \ifexp{\xint=0}
      {\funq{k}{5}{0}\;0}
      {\funq{f}{0}{0}\;(\funq{g}{2}{0}\;\funq{k}{4}{1})\;(\funq{g}{3}{1}\;\funq{k}{4}{1})\;(\xint - 1)}
  } \\
  \term_1 &= \evexp{\labB}{\funq{k}{4}{1}\;(\xint + 1)} \\
  \Atype_0 &= ((\Tint \to q_0, 0) \wedge (\Tint \to q_1, 1)) \to \Tint \to q_0 \\
  \Atype_1 &= ((\Tint \to q_0, 2) \wedge (\Tint \to q_1, 2)) \to \Tint \to q_2 \\
  \Atype_2 &= (\Tint \to q_1, 1) \to \Tint \to q_0 \\
  \Atype_3 &= (\Tint \to q_1, 1) \to \Tint \to q_1 \\
  \Atype_4 &= \Tint \to q_1 \\
  \Atype_5 &= \Tint \to q_0.
 \end{align*}
 %

 For this example, there exists the following call-sequence:
 \[
 \mainfun \recall{\progd_Q} h\;1 \recall{\progd_Q} h\;2 \recall{\progd_Q} h\;3 \recall{\progd} \dots.
 \]

 Thus, \(\Pfun(\funq{h}{4}{2}) \Pfun(\funq{h}{4}{2}) \Pfun(\funq{h}{4}{2}) \dots = 222\dots\) is a member of \(\Callseq(\progqPA)\) and this sequence satisfies the parity condition.
 \qed
\end{example}

%% \begin{definition}[\(\Callseq(Q)\)]
%%  Let \(Q\) be a program \((\set{f_{1}\;\seq{x}_1 = \termalt_1,\ldots,f_{n}\;\seq{x}_n=\termalt_n}, \mainfun)\) and \(\Pfun\) be a priority assignment for \(Q\).
%%  \(\Callseq(Q)\), the \emph{set of call sequences} generated by \(Q\), is defined as:
%%  \begin{align*}
%%   \Callseq(Q) &=  \left\{
%%   \begin{array}{@{}c|l@{}}
%%    & \mainfun \to_Q^* f_{i_1}\;\seq{\term_1},\\
%%    \Pfun(f_{i_1})\Pfun(f_{i_2})\Pfun(f_{i_3}) \dots \in \mathbb{N}^* \cup \mathbb{N}^\omega
%%    &[\seq{\term_1}/\seq{x_1}]\renameFun_Q(\termalt_{i_1}, 1) \to_Q^* \wtLabel{f}{1}_{i_2}\;\seq{\term_2},\\
%%    &[\seq{\term_2}/\seq{x_2}]\renameFun_Q(\termalt_{i_2}, 2) \to_Q^* \wtLabel{f}{2}_{i_3}\;\seq{\term_3},\\
%%    &\dots
%%   \end{array}
%%   \right\}
%%  \end{align*}
%% \end{definition}

%% \begin{theorem}\label{theorem:callseq}
%%  Let \(Q\) be a program that satisfies Cond.(ii).
%%  Then,

%%  Every \(\pi \in \InfTraces(Q)\) is accepted by \(\PWA\). \\
%%  \(\iff\) Every \(w \in \Callseq(Q)\) satisfies the parity condition.
%% \end{theorem}

%\begin{example}
% Consider a call sequence for the program \(\progqPA\) used in Example~\ref{liveness:example:effective_selection}.
% \begin{align*}
%  \termalt_1 &= \progd_{\progq}(\mainfun) = \evexp{\labC}{\funq{f}{1}{2}\;(\funq{g}{2}{2}\;\funq{h}{4}{2})\;(\funq{g}{3}{2}\;\funq{h}{4}{2})\;0} \qquad
%  \termalt_1^{\Mark} \Preds{\labC \labA \labB}{\progd_\progq} \funq{h^{\Mark}}{4}{2}\;1 \\
%  \termalt_2 &= \evexp{\labC}{\funq{f}{1}{2}\;(\funq{g}{2}{2}\;\funq{h}{4}{2})\;(\funq{g}{3}{2}\;\funq{h}{4}{2})\;\xint} \qquad
%  \termalt_2^{\Mark} \Preds{\labC \labA^2 \labB^2}{\progd_\progq} \funq{h^{\Mark}}{4}{2}\;2 \\
%  &\dots
% \end{align*}
%
 %
% \qed
%\end{example}

%% Suppose that \( \TopEnv \pInter D \).
%% For every \( f : (\Atype,m) \in \TopEnv \), let us choose a term \( \EffTerm{f}{\Atype}{m} \) such that \( \TopEnv \pInter D(f) : \Atype \Rightarrow \EffTerm{f}{\Atype}{m} \).
%% Then the set \( \EffTypeTrans{D} \) of function definitions is given by
%% \[
%% \EffTypeTrans{D} := \{ f_{\Atype,m} = \EffTerm{f}{\Atype}{m} \mid f : (\Atype,m) \in \TopEnv \}.
%% \]
%% Here we use the style of \( f = \lambda x_1 \dots x_k. t \).
\begin{lemma}
  If \( \TopEnv \pInter P \Rightarrow P' \), then \( \EffTypeTrans{\TopEnv} \pInter P' \).
  Furthermore \( \EffTypeTrans{\TopEnv} \) is simple.
  %% \( (1) \) \( \TopEnv \pInter t : \Atype \Rightarrow t' \) implies \( \EffTypeTrans{\TopEnv} \pInter t' : \EffTypeTrans{\Atype} \).
  %% \( (2) \) \( \TopEnv \pInter D \Rightarrow D' \) implies \( \EffTypeTrans{\TopEnv} \pInter D' \).
  %% \( (3) \) \( \EffTypeTrans{\TopEnv} \) is a simple environment, i.e.~it has no intersection type and it has at most one declaration for each variable.
\end{lemma}

It is not difficult to see that the translation does not changes the set of infinite traces.
\begin{lemma}\label{lem:liveness:trace-coincidence}
  If \( \TopEnv \pInter P \Rightarrow P' \), then \( \InfTraces(P) = \InfTraces(P') \).
\end{lemma}

%%\begin{theorem}\label{thm:linevess:eff-sel-sound-and-complete}
%%  Let \( P = (D, \mainfun) \) be a program and \( \PWA \) be a parity automaton.
%%  Suppose that \( \TopEnv \pInter P \Rightarrow P' \).
%%  Then \( \InfTraces(P) \subseteq \Lang(\PWA) \) if and only if every infinite call-sequence of \( P' \) satisfies the parity condition w.r.t.~\( \Pfun_{\EffTypeTrans{\TopEnv}} \).
%%\end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:linevess:eff-sel-sound-and-complete}]
  (\( \Rightarrow \))
  Suppose that \( \InfTraces(P) \subseteq \Lang(\PWA) \), which implies \( \InfTraces(\progqPA) \subseteq \Lang(\PWA) \) by Lemma~\ref{lem:liveness:trace-coincidence}.
  Let \( \progqPA = (E, \mainfun_{\qinit,0}) \) and suppose \( g_0 g_1 \dots \) be an infinite call-sequence of \( \progqPA \).
  Then \( g_0 = \mainfun_{\qinit,0} \) and there exists \( \RTyPath \) such that \( \RTyPath \Vdash \mainfun_{\qinit,0} \CallSeq_E g_1\,\tilde{u}_1 \CallSeq_E g_2\,\tilde{u}_1 \CallSeq_E \cdots \).
  Let \( \RTyPath \Vdash \mainfun_{\qinit,0} \stackrel{\ell_1}{\red}_E t_1 \stackrel{\ell_2}{\red}_E t_2 \stackrel{\ell_3}{\red_E} \cdots \) be the corresponding reduction sequence.
  Then \( \ell_1 \ell_2 \dots \in \Lang(\PWA) \), i.e.~the unique run \( \runseq \) of \( \PWA \) over \( \ell_1 \ell_2 \dots \) satisfies the parity condition.
  By Corollary~\ref{cor:liveness:summarising-priority}, there exists \( \{ (\Atype_i, m_i) \}_{i \ge 1} \) such that \( g_i : (\Atype_i, m_i) \in \EffTypeTrans{\TopEnv} \) for every \( i \ge 1 \) and \( \mathbf{max} \mathbf{Inf}(\Omega(R)) = \mathbf{max} \mathbf{Inf}(m_1 m_2 \dots) \).
  Since \( \EffTypeTrans{\TopEnv} \) is simple, there is at most one \( (\Atype_i, m_i) \) such that \( g_i : (\Atype_i, m_i) \in \EffTypeTrans{\TopEnv} \), and by definition, \( m_i = \Pfun_{P,\PWA} \).
  Hence \( g_0 g_1 \dots \) satisfies the parity condition with respect to \( \Pfun_{P,\PWA} \).

  (\( \Leftarrow \))
  Suppose that \( \InfTraces(P) \nsubseteq \Lang(\PWA) \), which implies \( \InfTraces(\progqPA) \nsubseteq \Lang(\PWA) \) by Lemma~\ref{lem:liveness:trace-coincidence}.
  So there exists an infinite trace \( \ell_1 \ell_2 \dots \in \InfTraces(\progqPA) \) such that the unique run of \( \PWA \) over \( \ell_1 \ell_2 \dots \) violates the parity condition.
  Let \( \RTyPath \) be a choice sequence which generates \( \ell_1 \ell_2 \dots \), i.e.~\( \RTyPath \Vdash \mainfun_{\qinit,0} \stackrel{\ell_1}{\red}_E t_1 \stackrel{\ell_2}{\red}_E t_2 \stackrel{\ell_3}{\red_E} \cdots \).
  By Lemma~\ref{lem:liveness:unique-existence-of-call-seq}, there exists an infinite call-sequence \( \RTyPath \Vdash \mainfun_{\qinit,0} \CallSeq_E g_1\,\tilde{u}_1 \CallSeq_E g_2\,\tilde{u}_1 \CallSeq_E \cdots \).
    By Corollary~\ref{cor:liveness:summarising-priority}, there exists \( \{ (\Atype_i, m_i) \}_{i \ge 1} \) such that \( g_i : (\Atype_i, m_i) \in \EffTypeTrans{\TopEnv} \) for every \( i \ge 1 \) and \( \mathbf{max} \mathbf{Inf}(\Omega(R)) = \mathbf{max} \mathbf{Inf}(m_1 m_2 \dots) \).
    Since \( \EffTypeTrans{\TopEnv} \) is simple, there is at most one \( (\Atype_i, m_i) \) such that \( g_i : (\Atype_i, m_i) \in \EffTypeTrans{\TopEnv} \), and by definition, \( m_i = \Pfun_{P,\PWA} \).
    Hence \( g_0 g_1 \dots \) violates the parity condition with respect to \( \Pfun_{P,\PWA} \).
\end{proof}



The next result is the main theorem of this section, which is a consequence of Theorems~\tk{The theorem of 7.1} and \ref{thm:linevess:eff-sel-sound-and-complete} and Lemma~\ref{lem:liveness:eff-sel-effective}.
\begin{theorem}
  Given a program \(P\) and %a deterministic parity word automaton \(\PWA\),
  a parity automaton \( \PWA \),
  %and \(\lts = (\{q_0\}, \emptyset, \emptyset, q_0)\) be an LTS.
  one can effectively construct an HES \( \HES \) such that
  every event sequence generated by \(P\) is accepted by \(\PWA\) if and only if \(\lts_0 \models \HES \).
\end{theorem}

\begin{example}
 Let \(\progqPA\) be the program used in Example~\ref{liveness:example:effective_selection}.
 We construct HES \(\HESf_{\progqPA} = (\HES, X_{\mainfun_{q_0, 0}})\) where \(\HES\) is:
 \begin{align*}
  X_{\funq{f}{1}{2}}\;\funq{k}{5}{0}\;\funq{k}{4}{1}\;\xint &=_{\nu}
  (\xint = 0 \wedge \funq{k}{5}{0}\;0) \vee (\xint \neq 0 \wedge X_{\funq{f}{0}{0}}\;(X_{\funq{g}{2}{0}}\;\funq{k}{4}{1})\;(X_{\funq{g}{3}{1}}\;\funq{k}{4}{1})\;(\xint - 1)) \\
  X_{\funq{g}{3}{1}}\;\funq{k}{4}{1}\;\xint &=_{\mu} X_{\funq{k}{4}{1}}\;(\xint + 1) \\
  X_{\funq{h}{4}{1}}\;\xint &=_{\mu} X_{\funq{f}{1}{2}}\;(X_{\funq{g}{2}{0}}\;X_{\funq{h}{4}{1}})\;(X_{\funq{g}{3}{1}}\;X_{\funq{h}{4}{1}})\;\xint \\
  X_{\funq{f}{0}{0}}\;\funq{k}{5}{0}\;\funq{k}{4}{1}\;\xint &=_{\nu}
  (\xint = 0 \wedge \funq{k}{5}{0}\;0) \vee (\xint \neq 0 \wedge X_{\funq{f}{0}{0}}\;(X_{\funq{g}{2}{0}}\;\funq{k}{4}{1})\;(X_{\funq{g}{3}{1}}\;\funq{k}{4}{1})\;(\xint - 1)) \\
  X_{\funq{g}{2}{0}}\;\funq{k}{4}{1}\;\xint &=_{\nu} \funq{k}{4}{1}\;(\xint + 1) \\
  X_{\mainfun_{q_0, 0}} &=_{\nu} X_{\funq{f}{1}{2}}\;(X_{\funq{g}{2}{0}}\;X_{\funq{h}{4}{1}})\;(X_{\funq{g}{3}{1}}\;X_{\funq{h}{4}{1}})\;0
 \end{align*}
\end{example}





==> memo.tex <==
\begin{lemma}
\label{lem:foo1}
If \(\TopEnv\pInter\prog \ESRel(\prog',\Pfun)\) and \(f\,\seq{s} \CallSeqN{a_1\cdots a_k}_{\prog} g\,\seq{t}\)
and \(\ITE\pInter f\,\seq{s} \COL q_0\ESRel f'\seq{s'}\), and \(q_0q_1\cdots q_k\) is a run of \(A\) from \(q_0\) 
over \(a_1\cdots a_k\), then
\begin{enumerate}[(i)]
\item \(\ITE'\pInter g\,\seq{t}\COL q_k \ESRel g_{\theta,m}\seq{t'}\);
\item \(m = \max(\Omega(q_1),\ldots,\Omega(q_k))\); and
\item \(f'\seq{s'} \CallSeqN{}_{\prog'} g_{\theta,m}\seq{t'}\).
\end{enumerate}
for some \(\ITE', \theta, m, \seq{t'}\).
\end{lemma}
\begin{proof}[sketch]
Let \(m\) be \(\max(\Omega(q_1),\ldots,\Omega(q_k))\).
By the assumptions,
we have:
\[
\begin{array}{l}
f' = f_{\theta',n}\\
f\,\seq{s} \Pred{\epsilon}{\prog} [\seq{s}/\seq{x}]u\\{}
[\seq{s}/\seq{x}][\seq{f}^\#/\seq{f}]u 
\Preds{a_1\cdots a_k}{\prog^\#}g^\#\,\seq{t''}\\
\mathit{Erase}_{\#}(\seq{t''})=\seq{t}
\end{array}
\]
By Lemma~\ref{appx:es:lem:sim1},
\[ [\TopEnv^\#]\cup \ITE \pInter [\seq{s}/\seq{x}][\seq{f}^\#/\seq{f}]u:q_0 \ESRel
   [\seq{s'}/\dup{\seq{x},\seq{\rho}}][\seq{f_{\theta',m'}}^\#/\seq{f_{\theta',m'}}]u'.\]
By repeated applications of Lemma~\ref{appx:es:lem:sim1}, we have:
\[[\seq{s'}/\dup{\seq{x},\seq{\rho}}][\seq{f_{\theta',m'}}^\#/\seq{f_{\theta',m'}}]u' \Preds{a_1\cdots a_k}{\prog'^\#}
   u_1\]
and
\[ [\TopEnv^\#]\RaiseP{m} \cup \ITE' \pInter g^\#\,\seq{t''}\ESRel u_1\]
for some \(u_1\) and \(\ITE'\), where \(\ITE'\) does not contain marked symbols. 
From the latter condition, \(u_1\) must be of the form \(g^\#_{\theta,m}\seq{t'''}\).
Thus, the required conditions hold for \(\seq{t'} = \mathit{Erase}(\seq{t'''})\).
\qed
\end{proof}

\begin{lemma}
\label{lem:foo2}
If \(\TopEnv\pInter\prog \ESRel(\prog',\Pfun)\) and 
\(f'\,\seq{s'} \CallSeqN{a_1\cdots a_k}_{\prog} g_{\theta,m}\,\seq{t'}\)
and \(\ITE\pInter f\,\seq{s} \COL q_0\ESRel f'\,\seq{s'}\), then
\begin{enumerate}[(i)]
\item \(\ITE'\pInter g\,\seq{t}\COL q_k \ESRel g_{\theta,m}\seq{t'}\);
\item \(q_0q_1\cdots q_k\) is a run of \(A\) from \(q_0\) over \(a_1\cdots a_k\);
\item \(m = \max(\Omega(q_1),\ldots,\Omega(q_k))\); and
\item \(f\,\seq{s} \CallSeqN{a_1\cdots a_k}_{\prog'} g\,\seq{t}\).
\end{enumerate}
\end{lemma}

\begin{proof}[sketch]
By the assumptions,
we have:
\[
\begin{array}{l}
f' = f_{\theta',n}\\
f_{\theta',n}\,\seq{s'} \Pred{\epsilon}{\prog'} [\seq{s'}/\dup{\seq{x},\seq{\rho}}]u'\\{}
[\seq{s'}/\dup{\seq{x},\seq{\rho}}][\seq{f_{\theta',m'}}^\#/\seq{f_{\theta',m'}}]u' 
\Preds{a_1\cdots a_k}{\prog'^\#}g^\#_{\theta,m}\,\seq{t''}\\
\mathit{Erase}_{\#}(\seq{t''})=\seq{t'}
\end{array}
\]
By Lemma~\ref{appx:es:lem:sim2}, (where we use, instead of \(\prog\), \(\prog''\) obtained by
marking all the functions on the righthand side of the definition of \(f\)),
\[ [\TopEnv^\#]\cup \ITE \pInter [\seq{s}/\seq{x}][\seq{f}^\#/\seq{f}]u:q_0
 \ESRel [\seq{s'}/\dup{\seq{x},\seq{\rho}}][\seq{f_{\theta',m'}}^\#/\seq{f_{\theta',m'}}]u'.\]
By repeated applicatins of Lemma~\ref{appx:es:lem:sim2}, there exists a run \(R = q_0q_1\cdots q_k\)
over \(a_1\cdots a_k\) such that
\[[\TopEnv^\#]\RaiseP{\mathbf{summ}(R)}\cup \ITE' \pInter g^\#\,\seq{t'''}\ESRel g^\#_{\theta,m}\,\seq{t''}\]
for some \(\ITE'\) (which does not contain marked symbols).
By the transformation rules, it must be the case that \(m=\mathbf{summ}(R) = \max(\Omega(q_1),\ldots,\Omega(q_k))\).
Thus, the required conditions hold for \(\seq{t} = \mathit{Erase}_{\#}(\seq{t'''})\). 
\nk{Here, I ignored the difference between \(\ESRel\) and \(\eESRel\).}
\qed
\end{proof}

\begin{proof}[Theorem 5]
We show the contraposition of each direction.
Suppose \(a_1a_2\cdots \in \InfTraces(P)\cap L\).
Then, there must exist an infinite reduction sequence
\[\textbf{main} \Preds{a_1}{P}\Preds{a_2}{P}\cdots\]
and a run \(q_0q_1q_2\cdots\) over \(a_1a_2\cdots\) that satisfies the parity condition.
By Lemma 26, there exists an infinite call sequence 
\[\textbf{main} \CallSeqN{a_1\cdots a_{k_1}}_{\prog} g_1\seq{u}_1
\CallSeqN{a_{k_1+1}\cdots a_{k_2}}_{\prog} g_2\seq{u}_2\CallSeqN{a_{k_2+1}\cdots a_{k_3}}_{\prog} \cdots\]
By repeated applications of Lemma~\ref{lem:foo1},
we obtain an infinite call sequence
\[\textbf{main}_{q_0,0} \CallSeqN{}_{\prog'} g_{\theta_1,m_1}\seq{u}'_1
\CallSeqN{}_{\prog} g_{\theta_2,m_2}\seq{u}'_2\CallSeqN{}_{\prog'} \cdots\]
such that \(\max(\Omega(a_{k_i+1}),\ldots,\Omega(a_{k_{i+1}})) = m_i\) (where \(k_0=0\)).
Since the largest priority that occurs infinitely often in \(m_1m_2\cdots\) is even,
the largest priority that occurs infinitely often in \(\Pfun(g_{\theta_1,m_1})\Pfun(g_{\theta_2,m_2})\cdots\)
is odd. Therefore, we have \(\not\models_\CSA (P',\Pfun)\).

Conversely, suppose \(\not\models_\CSA (P',\Pfun)\). Then, there must exist an infinite call sequence:
\[\textbf{main}_{q_0,0} \CallSeqN{}_{\prog'} g_{\theta_1,m_1}\seq{u}'_1
\CallSeqN{}_{\prog} g_{\theta_2,m_2}\seq{u}'_2\CallSeqN{}_{\prog'} \cdots\]
where the largest priority that occurs infinitely often in \(m_1m_2\cdots\) is even.
By repeated applications of Lemma~\ref{lem:foo2}, 
we have an infinite call sequence
\[\textbf{main} \CallSeqN{a_1\cdots a_{k_1}}_{\prog} g_1\seq{u}_1
\CallSeqN{a_{k_1+1}\cdots a_{k_2}}_{\prog} g_2\seq{u}_2\CallSeqN{a_{k_2+1}\cdots a_{k_3}}_{\prog} \cdots\]
such that there exists a run \(q_0q_1q_2\cdots\) over \(a_1a_2\cdots\)
and \(\max(\Omega(q_{k_i+1}),\ldots,\Omega(q_{k_{i+1}})) = m_i\).
Since the largest priority that occurs infinitely often in \(m_1m_2\cdots\) is even,
the largest priority that occurs infinitely often in \(\Omega(q_0)\Omega(q_1)\Omega(q_2)\cdots\) must also 
be even. Thus, we have \(a_1a_2\cdots \in \InfTraces(P)\cap L\). \qed
\end{proof}

